Optimization-Driven Adaptive Experimentation

Real-world experiments involve batched & delayed feedback, non-stationarity, multiple objectives & constraints, and (often some) personalization. Tailoring adaptive methods to address these challenges on a per-problem basis is infeasible, and static designs remain the de facto standard. Focusing on short-horizon ($\le 10$) adaptive experiments, we move away from bespoke algorithms and present a mathematical programming formulation that can flexibly incorporate a wide range of objectives, constraints, and statistical procedures. We formulating a dynamic program based on central limit approximations, which enables the use of scalable optimization methods based on auto-differentiation and GPU parallelization. To evaluate our framework, we implement a simple heuristic planning method ("solver") and benchmark it across hundreds of problem instances involving non-stationarity, personalization, and multiple objectives & constraints. Unlike bespoke methods (e.g., Thompson sampling variants), our mathematical programming framework provides consistent gains over static randomized control trials and exhibits robust performance across problem instances.

==> bayesian_model.tex <==
\section{Bayesian Model from Batch Approximations}
\label{section:algorithms}

The validity of the Gaussian batch approximation for large batch sizes
and small treatment effects means that for practical settings,
we can use the standard Bayesian linear regression model for updating posteriors using a Gaussian likelihood
for the aggregated rewards.

As we discuss in this section, the Bayesian linear regression model confers a multitude of capabilities
for adaptive experimentation compared to the raw description of batched adaptive experiment (Definition ~\ref{def:batch_experiment}).
While Bayesian linear regression is a textbook model for inference of linear models, we highlight novel advantages
for designing adaptive experiments.
\begin{enumerate}[itemsep=-2pt, leftmargin=.7cm]
  \item The posterior predictive distribution is Gaussian, which makes it easy to simulate trajectories of the adaptive experiment
  under different sampling policies.
  \item The experimenter can encode their objectives and tractably optimize them with autodifferentation and stochastic gradient descent.
\end{enumerate}

\subsection{Bayesian Markov Decision Process}

Suppose the experimentor has a Gaussian prior over the unknown coefficient vector
$\theta \sim N(\beta_{0}, \Sigma_{0})$, where $\beta_{0}$ describes the mean coefficient vector
under the prior and $\Sigma_{0}$ captures the uncertainty on the components.
This prior can be formed from a reservoir of ppreviously collected data or domain knowledge~\citep{KohaviLoSoHe09,
KohaviDeFrLoWaXu12, KohaviDeFrWaXuPo13}. Using the approximations justified by Theorem~\ref{theorem:limit},
\[
  \Psi_{n,t} = \frac{1}{b_{t}\sqrt{n}}  \Phi_{n,t} R_{n,t} \approx G_{t}
\]
we can update our belief on $\theta$ pretending that $\Psi_{n,t}$ is a draw of the contextual Gaussian sequential experiment.

If we observed draws $G_{0},\ldots,G_{T-1}$ from the Gaussian sequential experiment, 
we could maintain a Gaussian posterior belief on $\theta$ by conjugacy, as $G_{t}$ are all normally distributed conditional on previous observations.
We let $(\beta_{t}, \Sigma_{t})$ be the posterior at epoch $t$ after observing $G_{0},\ldots, G_{t-1}$. 
We refer to this as the asymptotic Bayesian model.
It is a Markov Decision Process, as its dynamics are controlled by the sampling allocations $\pi_{t}$ chosen by the experimenter.

\begin{definition} \label{def:asymptotic_bayes} The {\bf asymptotic Bayesian model} is defined by the following update rule for the Gaussian posterior
  parameters $(\beta_{t}, \Sigma_{t})$, upon observing $G_{t}$ at epoch $t$. Recall that $\bar{\pi}_{t} := \pi_{t} \otimes \mu_{t}$
  is the joint distribution induced by context distribution $\mu_{t}$ and sampling allocation $\pi_{t}(\beta_{t}, \Sigma_{t})$.
\begin{subequations}
  \label{eqn:posterior}
  \begin{align}
    \mbox{Posterior variance:}~~~~ \Sigma_{t+1}^{-1}
    &\defeq \Sigma_{t}^{-1} + b_{t}s^{-2} \E_{\bar{\pi}_{t}}[\phi \phi^{\top}]
      \label{eqn:posterior-var} \\
    \mbox{Posterior mean:}~~~~\beta_{t+1}
    &\defeq \Sigma_{t+1} \left( \Sigma_{t}^{-1}\beta_{t} 
  + (s^2/b_{t}) \E_{\bar{\pi}_{t}}[\phi \phi^{\top}] \E_{\bar{\pi}_{t}}[\phi \phi^{\top}]^{\dagger} G_{t} \right)
      \label{eqn:posterior-mean}
  \end{align}
\end{subequations}
where $\dagger$ denotes the Moore-Penrose pseudoinverse.
\end{definition}
% This leads to the updating rule from Bayes' rule. Starting from a posterior $(\beta_{t}, \Sigma_{t})$,
% the posterior after observing $\Psi_{n,t}$ is:
% \begin{align*}
%   \Sigma_{t+1}^{-1} &= \Sigma_{t}^{-1} + (s^2/b_{t}) \E_{\bar{\pi}_{t}}[\phi \phi^{\top}] \\
%   \beta_{t+1} &= \Sigma_{t+1} \left( \Sigma_{t}^{-1}\beta_{t} 
%   + (s^2/b_{t}) \E_{\bar{\pi}_{t}}[\phi \phi^{\top}] \E_{\bar{\pi}_{t}}[\phi \phi^{\top}]^{\dagger} \Psi_{n,t} \right)
% \end{align*}
\noindent This is almost identical to the standard update rule for Bayesian linear regression with the exception
of the pseudoinverse term, which allows for $\E_{\bar{\pi}_{t}}[\phi \phi^{\top}]$
to be singular. If $\E_{\bar{\pi}_{t}}[\phi \phi^{\top}]$ is invertible, then $\E_{\bar{\pi}_{t}}[\phi \phi^{\top}] \E_{\bar{\pi}_{t}}[\phi \phi^{\top}]^{\dagger} = I$
and this is identical to Bayesian linear regression.

Using standard properties of Gaussian random variables, we can reparameterize
the state transitions~\eqref{eqn:posterior} as a controlled random walk.
\begin{lemma}
  \label{lemma:mdp}
  Let $\theta \sim N(\beta_0, \Sigma_0)$ and
  $Z_0, \ldots, Z_{T-1} \simiid N(0, I_{\numarm})$ be standard normal
  variables. The system governed by the posterior
  updates~\eqref{eqn:posterior} has the same joint distribution as that with
  the following state transitions
  \begin{subequations}
    \label{eqn:dynamics}
    \begin{align}
      \mbox{Posterior variance:}~~~~ \Sigma_{t+1}^{-1}
      & \defeq \Sigma_{t}^{-1} + b_{t}s^{-2} \E_{\bar{\pi}_{t}}[\phi \phi^{\top}]
        \label{eqn:dynamics-var} \\
      \mbox{Posterior mean:}~~~~\beta_{t+1}
      &:= \beta_{t} + (\Sigma_{t} - \Sigma_{t+1})^{1/2} Z_{t}
        \label{eqn:dynamics-mean}
    \end{align}
  \end{subequations}
\end{lemma}
\noindent We defer derivation details to Section~\ref{section:proof-mdp}.

Since the only randomness in this model is from the Gaussian random vectors $Z_{0},\ldots,Z_{T}$,
this representation makes it easy to simulate entire trajectories of the batched adaptive experiment
and understand how the sampling allocations $\pi_{t}$ affect future posterior beliefs.
This capability enables one to be able to \emph{plan} future sampling allocations based on
the current belief on the quality of the treatment arms.
Note that this does require knowledge of the context arrival distributions $\mu_{t}$, 
but this assumption can be replaced by simply being able to sample contexts (e.g. from a historical dataset).
% Cruically, this framework offers a \emph{smoothed} model of partial feedback, 
% in which state transitions are \emph{differentiable} in the sampling allocations.
% This enables the use of autodifferentation frameworks (e.g,.)

\subsection{Bayesian objectives}

The experimenter can encode their objectives within the Bayesian model; in doing so they can guide
the sampling allocations according to their preferences. We consider a Bayesian experimenter whose objective
is to maximize a sum of per-period objective functions $v_{s}$ which depend on the posterior state $(\beta_{s}, \Sigma_{s})$
and the current sampling allocation $\pi_{t}$.
\begin{equation}
  \{ v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) \}_{s=0}^{T} 
\end{equation}

Within this Markov Decision Process, it is natural for the experimenter to use a sampling policy
$\pi = \{\pi(\cdot | \beta_{s}, \Sigma_{s}) \}$ which selects the sampling allocation based on the current posterior state $(\beta_{s}, \Sigma_{s})$.
The value function of the policy at time $t$ is the expectation of the sum of future objective functions.
\begin{equation}
  V^{\pi}_{t}(\beta_{t}, \Sigma_{t}) = \E_{t} \left[ \sum_{s = t}^{T} v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) \right] 
  = \E \left[ \sum_{s = t}^{T} v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) | \beta_{t}, \Sigma_{t}\right]
\end{equation}

To illustrate, we now discuss the Bayesian counterparts of the objectives mentioned in Section~\ref{subsection:objectives},
and how to represent them in this notation.

Bayesian simple regret is defined to be the simple regret, or the sub-optimality of the final arm selection $\pi_{T}\in \Delta_{K}$ at the end of the experiment,
averaged across realizations of $\theta$ distributed from the prior $\theta\sim N(\beta_{0}, \Sigma_{0})$.
\[
  \text{BSR}_{T}(\pi_{T}) 
  = \E_{\theta \sim N(\beta_{0}, \Sigma_{0})}\left[\max_{a} \E_{x\sim \mu}[r(x,a)] - \sum_{a} \pi_{T}(a)\E_{x \sim \mu}\left[r(x,a) \right] \right]
\]
Minimizing $\text{BSR}_{T}$ is equivalent to maximizing the Bayesian reward at the end of the experiment.
\begin{equation}
  \label{eqn:bsr}
  \mbox{Bayes Simple Regret:}~~~~
  \begin{cases}
  v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) = 0, &\forall s<T \\
  v_{T}(\pi_{T}, \beta_{T}, \Sigma_{T}) 
  = \sum_{a} \pi_{T}(a)\E_{x\sim \mu}\left[\phi(x,a)^{\top}\beta_{T} \right] & \text{otherwise}
  \end{cases}
\end{equation}

Alternatively, if the goal is to minimize policy regret, then this is equivalent to maximizing the final Bayesian policy reward
at the end of the experiment.
\begin{equation}
  \mbox{Bayes Policy Regret:}~~~~
  \begin{cases}
    v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) = 0, &\forall s<T \\
    v_{T}(\pi_{T}, \beta_{T}, \Sigma_{T}) 
    = \E_{x\sim \mu}\left[\sum_{a} \pi_{T}(a|x)\phi(x,a)^{\top}\beta_{T} \right] & \text{otherwise}
    \end{cases}
\end{equation}

Finally, if the goal is to minimize cumulative regret, then this is equivalent to maximizing the Bayesian rewards accumulated throughout the experiment
\begin{equation}
  \mbox{Bayes Cumulative Regret:}~~~~
  v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s}) = \sum_{i=1}^{n_{s}} \E_{x\sim \mu_{t}}\left[\sum_{a} \pi_{s}(a|x) \phi(x,a)^{\top}\beta_{s} \right],\quad \forall s\leq T
\end{equation}

By setting an objective within the Markov Decision Process, we can apply modern techniques in Reinforcement Learning (RL)
to optimize for a policy that maximizes the objective. This is feasible since trajectories of the asymptotic Bayesian model
can be easily simulated. Contrast this with the original batched experimental setting, which is very difficult to sample rollouts from 
since the rewards follow unknown distributions.

\paragraph{Pathwise Gradients} Crucially, this framework offers a \emph{smoothed} model of partial feedback,
in which smooth changes to the sampling allocations lead to smooth changes in future posterior beliefs and performance metrics.
Policy optimization is more tractable in this setting
than typical MDPs because state transitions~\eqref{eqn:dynamics}
of the model are \emph{pathwise differentiable} with respect to the sampling allocations $\pi_{t}$. 
As long as the objective functions $v_{s}$ are differentiable 
in their inputs, which they are for the examples described above, then we can compute exact gradients of $\frac{\partial v_{s}}{\partial \pi_{t}}$ for any $s$
with respect to $\pi_{t}$ for any $t\leq s$ along a sample path of sampled $Z_{0},\ldots,Z_{T-1}$ using auto-differentiation
frameworks (e.g. PyTorch~\cite{PyTorch19} or TensorFlow~\cite{TensorFlow16}). If $\pi_{\theta}$ is a parameterized policy
we can then perform stochastic gradient descent of the value function with respect to policy parameters
\[
  \theta \leftarrow \theta - \alpha \nabla_{\theta}  \sum_{s = 0}^{T} v_{s}(\pi^{\theta}_{s}, \beta_{s}, \Sigma_{s})
\]
Pathwise gradients are known to be vastly smaller gradient variance than standard policy gradient methods (e.g. REINFORCE),
which can greatly accelerate optimization.


\subsection{Asymptotic Validity}
Returning back to the original batched adaptive experiment, this model gives a guideline for how to update posterior beliefs
of the unknown coefficient vector. Practically however, the model in Definition~\ref{def:asymptotic_bayes} cannot be used exactly
as is since the population covariance is unknown and the measurement $\Psi_{n,t}$ is used instead of $G_{t}$. So instead, we
can plug-in the empirical counterparts to the asymptotic quantities.
This leads to what we refer to this as the approximate Bayesian model $(\beta_{n,t}, \Sigma_{n,t})$, 
which is compatible with the data obtained from the batched experiment.

\begin{definition} The {\bf approximate Bayesian model} is defined by the following update rule for posterior parameters
  $(\beta_{n,t}, \Sigma_{n,t})$, upon observing aggregated rewards $\Psi_{n,t}$ and contexts $\Phi_{n,t}$:
  \begin{subequations}
    \label{eqn:approx_posterior}
    \begin{align}
      \mbox{Posterior variance:}~~~~ \Sigma_{n,t+1}^{-1}
      &\defeq \Sigma_{n,t}^{-1} + b_{t}s^{-2} \left( \frac{1}{n_{t}}\Phi_{n,t}^{\top}\Phi_{n,t} \right)
        \label{eqn:approx_posterior-var} \\
      \mbox{Posterior mean:}~~~~\beta_{n,t+1}
      &\defeq \Sigma_{n,t+1} \left( \Sigma_{n,t}^{-1}\beta_{t} 
      + (s^2/b_{t})  \left( \frac{1}{n_{t}}\Phi_{n,t}^{\top}\Phi_{n,t} \right)
      \left( \frac{1}{n_{t}}\Phi_{n,t}^{\top}\Phi_{n,t} \right)^{\dagger} \Psi_{n,t} \right)
        \label{eqn:approx_posterior-mean}
    \end{align}
  \end{subequations}
\end{definition}

Using the main asymptotic result in Theorem~\ref{theorem:limit}, we can show that trajectories of the
approximate Bayesian model converge in distribution to trajectories of the asymptotic model as $n\to \infty$,
\begin{corollary}
  \label{cor:trajectory_limit}
  Let $\pi_{t}(\beta_{t}, \Sigma_{t})$ be a policy that is continuous a.s. under $(\beta_{t}, \Sigma_{t})$ drawn from~\eqref{eqn:posterior}.
  Let Assumptions~\ref{assumption:reward} and~\ref{assumption:contexts} hold and consider any fixed $\theta$ and prior $(\beta_{n,0}, \Sigma_{n,0}) = (\beta_{0}, \Sigma_{0})$.
  The posterior states of~\eqref{eqn:approx_posterior} converge in distribution to the states~\eqref{eqn:posterior} as $n\to \infty$,
  \[
    (\beta_{n,1}, \Sigma_{n,1},\ldots, \beta_{n,t}, \Sigma_{n,t}) \cd (\beta_{1}, \Sigma_{1},\ldots, \beta_{t}, \Sigma_{t}).
  \]
\end{corollary}

\noindent This in turn implies convergence of the performance metrics and the value functions. Ultimately, this justifies the use of the asymptotic model
as a guide for evaluating and optimizing performance metrics.
\begin{corollary}
  \label{cor:value_limit}
  If the objective functions $v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s})$ are all continuous in all arguments a.s. under $(\beta_{t}, \Sigma_{t})$ drawn from~\eqref{eqn:posterior},
  then $v_{s}(\pi_{s}, \beta_{n,s}, \Sigma_{n,s})\cd v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s})$ for all $s\leq T$.
  If in addition, $v_{s} = O(\norm{\beta}_{2} + \norm{\Sigma}_{2})$ then we also have convergence of the value functions for all $t=0,...,T-1$
  \[
    \E_{t} \left[ \sum_{s=t}^{T} v_{s}(\pi_{s}, \beta_{n,s}, \Sigma_{n,s})\right] \to \E_{t} \left[ \sum_{s=t}^{T} v_{s}(\pi_{s}, \beta_{s}, \Sigma_{s})  \right]
  \]
\end{corollary}

The exact form of the approximate posterior updates in~\eqref{eqn:approx_posterior} is useful for showing theoretical convergence, but also has 
implications for posterior updates in batched settings.
\paragraph{Implications on practical performance: Scaling the design matrix or prior.} While the covariance update in~\eqref{eqn:approx_posterior} scales the design matrix
by the batch size in order to obtain a sensible limit, we find that this is also practically relevant.
By scaling down the covariance matrix, or alternatively scaling up the prior by $n_{t}$, 
we manage to avoid numerical difficulties that emerge when updating with large batches, especially if the design matrix is singular or low-rank. 
This numerical difficulties emerge when trying to invert $\Sigma_{t+1}^{-1}$, which is going have an extremely small minimum eigenvalue
if the low-rank design matrix dominates the prior.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> deprecated/introduction.tex <==
\section{Introduction}
\label{section:introduction}



Experimentation is fundamental to decision-making in the real world, particularly for businesses 
and large-scale Internet platforms. Due to the cost of running experiments, adaptive experimentation 
has seen increasing adoption amongst practitioners for its ability to efficiently utilize limited experimental resources. 
However, experimentation practitioners often encounter significant practical challenges that standard 
adaptive experimentation (multi-armed bandit) algorithms are not designed to handle. Consider the following applications: 
\begin{itemize}
  \item A fashion retailer carries out a week long experiment 
  comparing multiple layouts for their landing page. The distribution of 
  visiting customers on the weekend is significantly different from a Monday, 
  showing how there can be significant non-stationarity in how users 
  respond to treatments across time.  
  \item A ridesharing platform conducts discount experiments in different regions to optimize region-specific pricing. 
  The platform has region-specific budget constraints that must be satisfied over the course of the experiment. 
\end{itemize} 
Bandit algorithms are typically analyzed and compared based on theoretical regret bounds in ideal settings that assume arm rewards are independently 
and identically distributed (i.i.d.) over time. The fashion retailer example shows the prevalance of naturally occuring non-stationarity, where 
naive applications of standard algorithms have been shown to lead to poor performance \citep{QinRusso2023}. Furthermore, there are many 
constraints that platforms may have to satisfy such as requiring sufficient sample coverage for post-experiment 
inference \citep{OfferWestortCoGr20, ZhangJaMu20}, requiring fairness \citep{chen20a}, ensuring 
safety \citep{amani19}, etc.. Standard algorithms have to be modified in order to satisfy these constraints. 
There are many more challenges that arise in practice including batched/delayed feedback, multiple objectives, and 
personalization. 

As a result, researchers typically develop problem specific algorithms for each possible instance, with a focus on theoretical regret bounds.
However, this approach has several limitations. First, the development of these algorithms is often driven by significant mathematical ingenuity 
and requires great skill in proving their theoretical validity. Due to the countless possible settings that may arise in practice,
it is impractical for practitioners to develop a new algorithm each time they encounter a setting not covered by existing algorithms. Second, 
maintaining a separate problem-specific algorithm for each possible setting that may arise in practice is cumbersome. 
Experimentation scenarios often involve multiple practical challenges at once, and implementing a different algorithm for each combinatorial combination of
objective, constraint, and other concerns like nonstationarity, can lead to fragmentation and difficulty in maintainance. 
Finally, instances involving multiple challenges may simply be complicated, where the development of traditional algorithms 
may be mathematically intractable or yield exceptionally complicated solutions. Practitioners may end up using simpler approximations 
that do not fully capture the complexities of their setting. 

\begin{figure}[t]
  \centering
  \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
  \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
  \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
  Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
  and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
  even under model misspecification, and across a wide range of learning rates.
    \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
    across 241 settings.
    RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
    Contextual TS do so in 95 and 125 instances respectively. 
    In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
    obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
    The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
    relative reward compared to Uniform when it underperforms Uniform.}
  \label{fig:main_plot}
\end{figure}

Consider the application of news feed recommendations on a social media platform like Instagram. Organic content on such platforms 
are often ranked using a \emph{user value model}, a function that scalarizes a set of ML signals into a single 
value for each piece of content (photos, videos, or text posts). More precisely, the scalar value of a post $i$ for user $j$ 
might be defined as $V_{ij} = \sum_{k} w_{k} Y_{ijk}$, where $Y_{ijk}$ is the $k$-th real-time ranking signal 
(e.g., probability of commenting, probability of re-sharing) output by an ML prediction model and $w_{k}$ is the weight 
for that signal. These weights $w_{k}$ are typically selected via online experimentation. During the experiment, 
the experimenter estimates $w_{k}$ by recommending content to users and wishes to minimize \emph{cumulative regret}. At the end of the 
experiment, the experimenter fixes $w_{k}$ and uses the estimated $w_{k}$ to recommend $K$ pieces of content to users, minimizing \emph{simple regret}
in a top-$K$ best arm identification setting. 

While this formulation is a natural objective, we are not aware of any existing algorithm meant to handle such a setting. There exists algorithms 
designed for separately handling the top-$K$ best arm identification setting and trading off between cumulative and simple regret. As a consequence, 
practitioners may either have to develop a new algorithm, potentially complicated algorithm, or use a suboptimal approximation. 

\subsection{Contributions}

To address these issues, we develop a \emph{mathematical-programming} framework
for adaptive experimental design, which tailors the sampling decisions to user-specified
objectives, constraints, and non-stationarity patterns through optimization.
Planning via optimization is the de-facto methodology
for coordinating complex and economically significant decisions across a planning horizon, 
while navigating multiple objectives and constraints,
in widespread settings such as supply-chain optimization, electricity markets, scheduling, etc.

We introduce the \emph{Batched Limit Dynamic Program}, a modeling framework that allows experimenters to write down 
dynamic programs that can flexibly incorporate a wide range of objectives, constraints, models, and plan 
for short time horizons. The \emph{Batched Limit Dynamic Program} is based on the observation that real-world experiments are 
universally conducted in \emph{large batches} and involve only a few reallocation opportunities \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. 
Large batches, often implemented deliberately as a way to reduce operational costs of 
experimentation, result in the asymptotic normality of a wide class of estimators. 
By extending Bayesian statistics to classical m-estimation, 
we allow experimenters to update a flexible and tractable Bayesian model of their uncertainty. 
In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
combinatorial action spaces, the \emph{Batched Limit Dynamic Program} can be 
approximately solved using computational tools. 

In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
the model-predictive control (MPC) design principle to adaptively plan the 
sampling allocations: after observing new samples, re-solve for an optimal 
\emph{non-adaptive} sampling policy to use for the rest of experiment. 
By resolving after every batch, the policy remains adaptive while working flexibly with batched feedback. 
Since the policy is the outcome of an optimization sub-routine, we can flexibly incorporate constraints.
Finally, it allows the experimenter to incorporate predictions of context arrivals, ensuring robustness 
against predictible non-stationarity (e.g. day-of-the-week, seasonality).






As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

... {\color{blue} TODO}

Finally, we release an accompanying software package " " that allows practitioners to easily implement 
our policies and develop new ...  {\color{blue} TODO}









%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> deprecated/introduction_edits.tex <==
\section{Introduction}
\label{section:introduction}


Experimentation is fundamental to decision-making in the real world, particularly for businesses 
and large-scale Internet platforms. Due to the cost of running experiments, adaptive experimentation 
has seen increasing adoption amongst practitioners for its ability to efficiently utilize limited experimental resources. 
However, experimentation practitioners often encounter significant practical challenges that standard 
adaptive experimentation (multi-armed bandit) algorithms are not designed to handle. Consider the following applications: 
\begin{itemize}
  \item A social media platform runs online experiments to tune a machine learning (ML) algorithm for ranking content recommended to the user.
  Each user experiences a personalized ranking.
  \item A fashion retailer carries out a week long experiment 
  comparing multiple layouts for their landing page. The behavior of 
  customers who visit the page on the weekend is different from customers that visit on Monday. 
  This can lead to significant non-stationarity of user responses to treatments across time.  
  \item A ridesharing platform conducts discount experiments in different regions to measure region-specific price elasticities. 
  The platform has an aggregate budget constraint that must be satisfied over the course of the experiment. 
\end{itemize}
These examples illustrate that beyond simply identifying the best treatment,
experimental designs must also be able to handle a variety of practical considerations,
including personalization, non-stationarity, and constraints.
Another complicating factor is that while standard bandit algorithms are designed to be updated
after every sample, experiments are almost always conducted in large batches with infrequent 
updates to the sampling policy
due to operational constraints and delayed feedback \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}.
Experiments may also involve other constraints such as requiring sufficient 
sample coverage for post-experiment inference \citep{OfferWestortCoGr20, ZhangJaMu20}, 
requiring fairness \citep{chen20a}, and ensuring safety \citep{amani19}. 
Experimenters often must balance multiple objectives at once and must 
identify treatments which maximize a primary metric 
without incurring degradations on other, secondary metrics. 

Existing bandit algorithms are usually focused on 
one or at most two of these considerations, and are carefully tailored 
in order to deliver concrete theoretical guarantees for performance. 
However, due to this careful construction, these algorithms can be highly fragile 
when deployed outside of their designated context. In the fashion retailer example,
it is quite commonly known that temporal non-stationarity is widely prevalent in 
user responses to treatments. It has been observed that applying standard bandit algorithms,
which are designed for settings where the arm rewards are independently 
and identically distributed (iid) over time, can lead to substantial degradations in performance
even compared to simple, static A/B testing \citep{QinRusso2023,fiez2024three}.

Even if these challenges are anticipated, it is impractical for practitioners to develop a new algorithm 
each time they encounter a new setting not covered by existing algorithms, which may occur
due to a business or operational need.
Consider the application of news feed recommendations on a social media platform like Instagram. Organic content on such platforms 
are often ranked using a \emph{user value model}, a function that scalarizes a set of ML signals into a single 
value for each piece of content (photos, videos, or text posts) \citep{mahapatra2020insta, lada2021fb}. More precisely, the scalar value of a post $i$ for user $j$ 
might be defined as $V_{ij} = \sum_{k} w_{k} Y_{ijk}$, where $Y_{ijk}$ is the $k$-th real-time ranking signal 
(e.g., probability of commenting, probability of re-sharing) output by an ML prediction model and $w_{k}$ is the weight 
for that signal. These weights $w_{k}$ are typically selected via online experimentation. 

The experimenter estimates $w_{k}$ by recommending content to users and wishes to minimize \emph{cumulative regret} during the experiment. At the end of the 
experiment, the experimenter fixes $w_{k}$ and uses the estimated $w_{k}$ to deliver personalized recommendations of $K$ pieces of 
content to users, minimizing \emph{simple regret} in a top-$K$ best arm identification setting. 
While this formulation is a natural objective, we are not aware of any existing algorithm specifically meant to handle such a setting. There exist algorithms 
designed for separately handling the top-$K$ best arm identification setting \citep{qin2023dual,reda2021topm} and trading off between cumulative and simple regret \citep{krishnamurthy2023prop}. 

This example showcases how practitioners can easily encounter settings not covered by 
existing algorithms due to the need to satisfy multiple platform-specific concerns. 
Due to the complexity of designing new algorithms, practitioners often have to rely on simple but suboptimal approximations 
that capture only part of the challenges of their setting.
In settings involving multiple concerns, designing extensions of traditional algorithms 
may be mathematically intractable or yield exceptionally complicated solutions. Yet, even if it were 
possible to develop a specific algorithm for each combinatorial combination of objective, constraint, and other concerns like non-stationarity, 
maintaining a separate problem-specific algorithm for each possible setting that may arise in practice can lead to 
fragmentation and difficulty in maintainance. 
Therefore, even though adaptive methods are capable of greatly improving sample efficiency of experiments,
given the considerable difficulties of operationalizing adaptive algorithms and tailoring them
to practical circumstances, almost all experiments are non-adaptive A/B tests \citep{SculleyEtAl15, AgarwalEtAl16}.

\begin{figure}[t]
  \centering
  \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
  \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
  \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
  Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
  and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
  even under model misspecification, and across a wide range of learning rates.
    \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
    across 241 settings.
    RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
    Contextual TS do so in 95 and 125 instances respectively. 
    In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
    obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
    The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
    relative reward compared to Uniform when it underperforms Uniform.}
  \label{fig:main_plot}
\end{figure}



\subsection{Contributions}

To address these issues, we develop a \emph{mathematical-programming} framework
for adaptive experimental design, which tailors the sampling decisions to user-specified
objectives, constraints, and non-stationarity patterns through optimization.
Given that experiments are typically carried out in a limited number of large batches,
tools from planning and multi-stage stochastic programming can be applied to obtain treatment allocations
that optimize the user's objective, subject to constraints.
This objective could be a standard one in the bandit literature, such as best arm identification, or complex, 
such as best top-$K$ selection while minimizing cumulative regret as mentioned earlier.
Planning via optimization is a standard methodology
for coordinating complex and economically significant decisions across a time horizon 
while navigating multiple objectives and constraints, with
diverse applications in areas such as supply-chain optimization, electricity markets, job scheduling, etc.
Crucially, optimization provides a clear and interpretable 
language for the experimenter to state their preferences, constraints, and desired outcomes,
and is much more flexible than designing bespoke algorithms for specific problems. 

However, it is challenging to set up an appropriate optimization problem, as this requires understanding
dynamic considerations of how the treatment allocation at each stage affects future treatment allocations and the final performance objective. 
This requires anticipating the value of data collected in future stages. This 
is an especially difficult task when the distribution of the rewards is unknown, as is commonly the case in practice.
It is also difficult to frame the problem as a standard dynamic program, as it is unclear whether there is an appropriate choice
of state space that follows Markovian dynamics in this unstructured environment.
Finally, the action space involves all possible allocations of treatments to users, which 
can be intractably large considering the large sample sizes featured in modern experiments.
At best, this problem is a high-dimensional, partially observable Markov decision process (POMDP) with
a combinatorial action space --  an NP-complete class of problems.

To provide a tractable optimization procedure, 
we introduce the $\modelfull$ ($\model$), a modeling framework that allows experimenters to write down 
dynamic programs that can flexibly incorporate a wide range of objectives, constraints, models, and plan 
across a specified time horizon. The $\modelfull$ is based on the observation that real-world experiments are 
universally conducted in a \emph{few, large batches} \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. 
Large batches, often implemented deliberately as a way to reduce operational costs of 
experimentation, result in the asymptotic normality of a wide class of estimators. 
By extending Bayesian statistics to classical m-estimation, 
we allow experimenters to update a flexible and tractable Bayesian model of their uncertainty. 
In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
combinatorial action spaces, the $\model$ has (1) a simple and interpretable state space, 
(2) has closed-form dynamics making it easy to simulate trajectories and (3)
smooths the partial feedback of sampling, enabling performance metrics such as regret to 
tractably optimized via stochastic gradient descent methods. 

In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
the model-predictive control (MPC) design principle to adaptively plan the 
sampling allocations. Whenever new samples are obtained, which could be from a large batch, 
the policy simulates trajectories from the $\model$ to solve for an optimal 
\emph{static} sequence of treatment allocations to use for the rest of experiment. 
By re-solving this sequence after every batch, the policy remains adaptive while working flexibly with batched feedback. 
The treatment allocation is the solution of an optimization routine, which means we can flexibly incorporate 
user-specified objectives and constraints. It allows the experimenter to also incorporate predictions of context arrivals, 
and by doing so it can ensure robustness against temporal non-stationarity (e.g. day-of-the-week, seasonality).
The model-predictive control principle guarantees that regardless of how complicated
the inputted specifications, objectives, constraints, and non-stationarity patterns are,
the treatment allocations are guaranteed to have a lower Bayesian regret than static A/B testing.
This is a practically useful robustness guarantee since static A/B testing
is the universal baseline for treatment allocation in real-world experiments. It allows the policy to be safely deployed in diverse settings,
including those which have not yet been studied in the multi-armed bandit literature.





As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

... {\color{blue} TODO}

Finally, we release an accompanying software package " " that allows practitioners to easily implement 
our policies and develop new ...  {\color{blue} TODO}









%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



% Experimentation is a core component of the deployment life-cycle of machine learning (ML) models in the real world, 
% particularly for large-scale Internet platforms. Adaptive experimentation offers a powerful methodology for 
% reducing operational costs and increasing statistical power by efficiently allocating sampling effort.  
% {\color{blue} Consider the following applications, motivated by real-world business use cases:
% \begin{itemize}
%   \item Meta example
%   \item A fashion retailer comparing multiple layouts for their landing page in anticipation of a holiday sale.
%   \item A ridesharing platform conducting discount experiments in different regions to optimize region-specific pricing.
% \end{itemize}

% Although superficially these examples may be modeled as instances of a multi-armed bandit problem,
% there are substational practical challenges unique to each setting that preclude a straightforward application
% of standard multi-armed bandit algorithms. These challenges include non-stationarity, constraints, personalization,
% multiple objectives, etc. While there are works dealing individually with each of these issues, 
% currently there is no single framework built to flexibly address all of these issues. Inflexibility of current approaches
% makes it difficult for practitioners to apply adaptive experimentation to their setting, which may involve bespoke considerations
% or even combinations of these challenges.

% partly because
% there is often a disconnect between the practical challenges of conducting modern experiments and the 
% problems that algorithmic researchers attempt to address. 
% }

% To elucidate a few examples: first, adaptive experimentation (bandit) algorithms are typically compared based 
% on their associated regret bounds, almost always in ideal settings that assume arm rewards are independently 
% and identically distributed (i.i.d.) over time. 
% {\color{blue}
% Yet, as in the example of the fashion retailer conducting
% an experiment during the holiday season, there can be significant non-stationarity in how users respond to treatments across time, 
% which can derail adaptive sampling policies \citep{QinRusso2023}}. 
% We conduct a rigorous empirical study across 241 unique settings exhibiting 
% natural non-stationarity based on experiments performed by ASOS.com, a global fashion retailer with 
% over 26 million active customers (as of 2024). Concerningly, we find that popular adaptive experimentation methods
% like Thompson Sampling, even when augmented with contextual information to explicitly account for non-stationary, 
% fail to outperform a simple uniform allocation policy (see Figure \ref{fig:main_plot}) {\color{blue} in more than 48\% of experiments}, 
% showing that theoretical regret bounds may not be indicative of practical performance.
% {\color{blue} Need to be careful, there are bandit papers dealing with non-stationarity.}

% Second, large-scale experiments are increasingly becoming more complicated due to the need to satisfy constraints 
% and optimize multiple objectives directly related to importance and impact on a business platform, usually 
% at the same time. {\color{blue} In the case of the ridesharing platform conducting regional discount experiments,
% often these experiments are conducted with a budget constraint for the total coupon amount across regions.}
% Other examples include requiring sufficient sample coverage for post-experiment 
% inference \citep{OfferWestortCoGr20, ZhangJaMu20}, requiring fairness \citep{chen20a}, and ensuring 
% safety \citep{amani19}. While there are bandit algorithms developed to handle each of these settings individually, 
% these methods are typically developed on a per-problem basis and require significant mathematical insight. There is 
% a lack of a general-purpose framework that allows practitioners to specify platform-specific constraints and 
% objectives in a flexible manner. 

% Third, experimentation is increasingly utilized to optimize policies that assign
% users personalized treatments, such as a slate of content in a social media context~\cite{}.
% Policy regret as an objective

% Finally, in contrast to algorithms designed to achieve strong guarantees as the number of reallocation epochs 
% grows to infinity, real-world experiments are universally conducted in \emph{large batches} with \emph{infrequent updates} to 
% the sampling policy \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. {\color{blue} Experimentation
% with large batches is often implemented deliberately as a way to reduce operational costs of experimentation, with
% the size of the batch typically determined by platform-specific usage (e.g. the batch consists of all users who
% arrive to the platform on a specific day or week).
% Large batches also emerge naturally if the treatment outcomes exhibit delayed feedback. 
% If outcomes can only be collected after a certain period of time,
% rather than waiting sequentially for each individual outcome to be recorded, 
% it is far more efficient to assign treatments to a batch of users in order to obtain a richer sample
% of outcomes at the end of the delay period. This introduces challenges into the mathematical analysis of adaptive experimentation 
% algorithms, which typically rely on martingale arguments that are better suited for algorithms that update frequently}. Much of the literature
% on batched bandit algorithms also require custom batch sizes, which is incompatible with current practices in which batches are determined
% exogenously by platform usage or delays.
% % However, as we will show later, rather than imposing a fundamental
% % algorithmic difficulty, in our proposed framework large batches actually improve our ability to model the information
% % gained by adaptive sampling policies.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
%   \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
%   \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
%   Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
%   and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
%   even under model misspecification, and across a wide range of learning rates.
%     \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
%     across 241 settings.
%     RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
%     Contextual TS do so in 95 and 125 instances respectively. 
%     In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
%     obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
%     The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
%     relative reward compared to Uniform when it underperforms Uniform.}
%   \label{fig:main_plot}
% \end{figure}

% {\color{blue}
% Rather than relying on bespoke algorithms, which are often derived via mathematical insight and cannot easily adapt
% to new settings, we develop a \emph{mathematical-programming} framework
% for adaptive experimental design, which tailors the sampling decisions to user-specified
% objectives, constraints, and non-stationarity patterns through optimization.
% Planning via optimization is the de-facto methodology
% for coordinating complex and economically significant decisions across a planning horizon, 
% while navigating multiple objectives and constraints,
% in widespread settings such as supply-chain optimization, electricity markets, scheduling, etc.
% Considering that modern experiments involve sampling decisions 
% }

% To address these issues, we introduce a modeling methodology called " " that allows experimenters to write down 
% dynamic programs that can flexibly incorporate a wide range of objectives, constraints, and models. 
% " " is based on the observation that batches, which are naturally used in real-world experiments, result in the 
% asymptotic normality of a wide class of estimators. By extending Bayesian statistics to classical m-estimation,
% we allow experimenters to update a tractable Bayesian model of their uncertainty. 
% In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
% combinatorial action spaces, " " dynamic programs can be approximately solved using computational tools. 

% In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
% the model-predictive control (MPC) design principle to adaptively plan the 
% sampling allocations: after observing new samples, re-solve for an optimal 
% \emph{non-adaptive} sampling policy to use for the rest of experiment. 
% By resolving after every batch, the policy remains adaptive while working flexibly with batched feedback. 
% Since the policy is the outcome of an optimization sub-routine, we can flexibly incorporate constraints.
% Finally, it allows the experimenter to incorporate predictions of context arrivals, ensuring robustness 
% against predictible non-stationarity (e.g. day-of-the-week, seasonality).

% As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
% empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

% ... 

% Finally, we release an accompanying software package " " that allows practitioners to easily implement 
% our policies and develop new ...  









% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:



% Experimentation is a core component of the deployment life-cycle of machine learning (ML) models in the real world, 
% particularly for large-scale Internet platforms. Adaptive experimentation offers a powerful methodology for 
% reducing operational costs and increasing statistical power by efficiently allocating sampling effort.  
% {\color{blue} Consider the following applications, motivated by real-world business use cases:
% \begin{itemize}
%   \item Meta example
%   \item A fashion retailer comparing multiple layouts for their landing page in anticipation of a holiday sale.
%   \item A ridesharing platform conducting discount experiments in different regions to optimize region-specific pricing.
% \end{itemize}

% Although superficially these examples may be modeled as instances of a multi-armed bandit problem,
% there are substational practical challenges unique to each setting that preclude a straightforward application
% of standard multi-armed bandit algorithms. These challenges include non-stationarity, constraints, personalization,
% multiple objectives, etc. While there are works dealing individually with each of these issues, 
% currently there is no single framework built to flexibly address all of these issues. Inflexibility of current approaches
% makes it difficult for practitioners to apply adaptive experimentation to their setting, which may involve bespoke considerations
% or even combinations of these challenges.

% partly because
% there is often a disconnect between the practical challenges of conducting modern experiments and the 
% problems that algorithmic researchers attempt to address. 
% }

% To elucidate a few examples: first, adaptive experimentation (bandit) algorithms are typically compared based 
% on their associated regret bounds, almost always in ideal settings that assume arm rewards are independently 
% and identically distributed (i.i.d.) over time. 
% {\color{blue}
% Yet, as in the example of the fashion retailer conducting
% an experiment during the holiday season, there can be significant non-stationarity in how users respond to treatments across time, 
% which can derail adaptive sampling policies \citep{QinRusso2023}}. 
% We conduct a rigorous empirical study across 241 unique settings exhibiting 
% natural non-stationarity based on experiments performed by ASOS.com, a global fashion retailer with 
% over 26 million active customers (as of 2024). Concerningly, we find that popular adaptive experimentation methods
% like Thompson Sampling, even when augmented with contextual information to explicitly account for non-stationary, 
% fail to outperform a simple uniform allocation policy (see Figure \ref{fig:main_plot}) {\color{blue} in more than 48\% of experiments}, 
% showing that theoretical regret bounds may not be indicative of practical performance.
% {\color{blue} Need to be careful, there are bandit papers dealing with non-stationarity.}

% Second, large-scale experiments are increasingly becoming more complicated due to the need to satisfy constraints 
% and optimize multiple objectives directly related to importance and impact on a business platform, usually 
% at the same time. {\color{blue} In the case of the ridesharing platform conducting regional discount experiments,
% often these experiments are conducted with a budget constraint for the total coupon amount across regions.}
% Other examples include requiring sufficient sample coverage for post-experiment 
% inference \citep{OfferWestortCoGr20, ZhangJaMu20}, requiring fairness \citep{chen20a}, and ensuring 
% safety \citep{amani19}. While there are bandit algorithms developed to handle each of these settings individually, 
% these methods are typically developed on a per-problem basis and require significant mathematical insight. There is 
% a lack of a general-purpose framework that allows practitioners to specify platform-specific constraints and 
% objectives in a flexible manner. 

% Third, experimentation is increasingly utilized to optimize policies that assign
% users personalized treatments, such as a slate of content in a social media context~\cite{}.
% Policy regret as an objective

% Finally, in contrast to algorithms designed to achieve strong guarantees as the number of reallocation epochs 
% grows to infinity, real-world experiments are universally conducted in \emph{large batches} with \emph{infrequent updates} to 
% the sampling policy \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. {\color{blue} Experimentation
% with large batches is often implemented deliberately as a way to reduce operational costs of experimentation, with
% the size of the batch typically determined by platform-specific usage (e.g. the batch consists of all users who
% arrive to the platform on a specific day or week).
% Large batches also emerge naturally if the treatment outcomes exhibit delayed feedback. 
% If outcomes can only be collected after a certain period of time,
% rather than waiting sequentially for each individual outcome to be recorded, 
% it is far more efficient to assign treatments to a batch of users in order to obtain a richer sample
% of outcomes at the end of the delay period. This introduces challenges into the mathematical analysis of adaptive experimentation 
% algorithms, which typically rely on martingale arguments that are better suited for algorithms that update frequently}. Much of the literature
% on batched bandit algorithms also require custom batch sizes, which is incompatible with current practices in which batches are determined
% exogenously by platform usage or delays.
% % However, as we will show later, rather than imposing a fundamental
% % algorithmic difficulty, in our proposed framework large batches actually improve our ability to model the information
% % gained by adaptive sampling policies.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
%   \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
%   \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
%   Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
%   and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
%   even under model misspecification, and across a wide range of learning rates.
%     \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
%     across 241 settings.
%     RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
%     Contextual TS do so in 95 and 125 instances respectively. 
%     In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
%     obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
%     The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
%     relative reward compared to Uniform when it underperforms Uniform.}
%   \label{fig:main_plot}
% \end{figure}

% {\color{blue}
% Rather than relying on bespoke algorithms, which are often derived via mathematical insight and cannot easily adapt
% to new settings, we develop a \emph{mathematical-programming} framework
% for adaptive experimental design, which tailors the sampling decisions to user-specified
% objectives, constraints, and non-stationarity patterns through optimization.
% Planning via optimization is the de-facto methodology
% for coordinating complex and economically significant decisions across a planning horizon, 
% while navigating multiple objectives and constraints,
% in widespread settings such as supply-chain optimization, electricity markets, scheduling, etc.
% Considering that modern experiments involve sampling decisions 
% }

% To address these issues, we introduce a modeling methodology called " " that allows experimenters to write down 
% dynamic programs that can flexibly incorporate a wide range of objectives, constraints, and models. 
% " " is based on the observation that batches, which are naturally used in real-world experiments, result in the 
% asymptotic normality of a wide class of estimators. By extending Bayesian statistics to classical m-estimation,
% we allow experimenters to update a tractable Bayesian model of their uncertainty. 
% In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
% combinatorial action spaces, " " dynamic programs can be approximately solved using computational tools. 

% In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
% the model-predictive control (MPC) design principle to adaptively plan the 
% sampling allocations: after observing new samples, re-solve for an optimal 
% \emph{non-adaptive} sampling policy to use for the rest of experiment. 
% By resolving after every batch, the policy remains adaptive while working flexibly with batched feedback. 
% Since the policy is the outcome of an optimization sub-routine, we can flexibly incorporate constraints.
% Finally, it allows the experimenter to incorporate predictions of context arrivals, ensuring robustness 
% against predictible non-stationarity (e.g. day-of-the-week, seasonality).

% As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
% empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

% ... 

% Finally, we release an accompanying software package " " that allows practitioners to easily implement 
% our policies and develop new ...  









% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:


==> extensions.tex <==
\subsection{Extensions}
\label{section:extensions}


In practice, the experimenter often needs to trade multiple objectives and
constraints beyond identifying the treatment with the highest average reward.
For example, the experimenter may want to identify the top two or three
treatments and then later run a static A/B test to obtain statistical
significance.  Alternatively, she may want to minimize the regret incurred
during the experiment and quickly eliminate treatment arms that are
detrimental to sample participants.  In some cases, she may constrain sampling
probabilities to be above a threshold for downstream inferential procedures.
Treatments typically impact multiple rewards/outcomes, in which case there may
no longer be a `best' treatment arm and the experimenter may instead be interested
in identifying treatments that perform well across all dimensions.

Since our framework is optimization-based,
these objectives and constraints can be easily incorporated
into the policy by modifying the planning problem~\eqref{eqn:rho-planning}.
Adding such modifications guarantees that 
performance will always improve over any static design 
across any time horizon as in Proposition~\ref{prop:rho-vs-static}.
One can contrast this with standard adaptive policies such as Thompson Sampling
or Successive Elimination, for which one may have to make
drastic and ad-hoc changes to the policy to accomodate additional features,
without any guarantees of performance.

To illustrate, consider an experimenter 
who wants to minimize a combination of
Bayesian simple regret among the top-5 arms and a negative entropy penalty (to encourage
sampling all arms), while imposing a linear constraint on the sampling probabilities.
For example, in a pricing experiment where each arm corresponds to a different price,
this could be a constraint on the average price shown to users.
Rather than optimizing the value function $\E_{t}[\max_{a}\mu_{T,a}]$,
through similar arguments as in Lemma~\ref{lemma:rho-reduction} one can show that the
$\algo$ problem can be reduced to:
\[
    \maximize_{\bar{\rho} \in \Delta_\numarm}
    \left\{ V^{\bar{\rho}}_{t}(\mu_{t},\sigma_{t})
     = \E_{t}\left[\text{top-}5(\mu_{T}) \right]   + \lambda H(\bar{\rho})
    : r^{\top}\bar{\rho} \leq \bar{r} \right\},
\]
where $r \in \R^{\numarm}$, $\bar{r}\in \R$, $\text{top-}k$ sums the values of the top $k$ entries of an input vector,
$H(\bar{\rho}) = \sum_{a} \bar{\rho}_{a} \log \bar{\rho}_{a}$ is the entropy function,
and $\lambda$ is a parameter calibrating the tradeoff between simple regret and the entropy penalty.
Although $\text{top-}k$ is non-differentiable, there exist reliable differentiable
surrogates~\cite{AmosKoKo19, BlondelTeBeDj20} that allow the use of stochastic gradient methods 
to solve the planning problem. 
The strong empirical performance of our iterative planning approach
suggests that our framework can reliably guide
adaptive experimental design across the varied demands
of modern large-scale experiments.











%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> implementation.tex <==
\section{Implementation Details}
\label{section:implementation}

We first discuss the implementation details for solving the $\algofull$ planning problem \eqref{eqn:rho}.
Recall that the problem involves maximizing the expectation of future posterior means
over constant sampling allocations in the simplex $\Delta_{\numarm}$:
\[
\maximize_{\bar{\rho} \in \Delta_\numarm}
\left\{ V^{\bar{\rho}}_{t}(\mu_{t},\sigma_{t})
  =  \E_{t} \left[ \max_{a} \left\{ \mu_{t,a}
      + \sqrt{\frac{\sigma_{t, a}^4 \bar{\rho}_{a} \bar{b}_{t}}
        {s_a^2 + \sigma_{t, a}^2 \bar{\rho}_{a} \bar{b}_{t}}} Z_{t, a}
    \right\} \right] \right\}.
\]
We approximate the expectation in the objective function by a sample average approximation
with $N$ standard normal random vectors.
\[
    \maximize_{\bar{\rho} \in \Delta_\numarm}
    \left\{
    \frac{1}{N}\sum_{j=1}^{N}
   \max_{a} \left\{ \mu_{t,a}
      + \sqrt{\frac{\sigma_{t, a}^4 \bar{\rho}_{a} \bar{b}_{t}}
        {s_a^2 + \sigma_{t, a}^2 \bar{\rho}_{a} \bar{b}_{t}}} Z_{t, a, j}
    \right\}
    \right\}.
\]
where $Z_{t,a,1},...,Z_{t,a,N}$ are iid draws of $N(0,1)$ random variables. 
We use quasi-Monte Carlo methods for variance reduction and draw
the normal random variables from a Sobol sequence,
which is widely used in practice in Bayesian Optimizaton \cite{BalandatEtAl20}.

There are many methods for solving this constrained optimization problem (e.g. projected gradient descent).
We use a softmax parameterization of the 
simplex $\bar{\rho}_{a} \propto e^{v_{a}}$,
and use unconstrained stochastic gradient methods to optimize over $v$.
We observe that vanilla stochastic gradient descent gets stuck at sub-optimal allocations
that allocate all sampling effort to one treatment arm. We obtain much better performance
from approximate second-order methods such as Adam \cite{KingmaBa15} or L-BFGS \cite{LiuNo89},
and use Adam for the experimental evaluation.

For the policy gradient method, we parameterize the policy as a feed-forward neural network with 
2 hidden layers with 512 units in each layer. The network uses the rectified non-linearity \cite{GlorotBoBe11} for all hidden layers.
We pass the posterior means $\mu \in \R^{\numarm}$, the posterior variances $\sigma^{2} \in \R^{\numarm}$, the current epoch $t \in \N$,
and the measurement variance $s^{2} \in \R^{\numarm}$ as inputs. The output of the network is passed through a softmax layer
and so the final output is a sampling allocation $\bar{\rho}\in \Delta^{\numarm}$. We train the network with the 
Adam optimizer with learning rate $5.0 \times 10^{-6}$ and $(\beta_{1},\beta_{2}) = (0.9, 0.999)$ in minibatches of size $50$.
Minibatches are drawn by randomly generating priors $(\mu_{0}, \sigma_{0})$.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> macros/new_bib <==
@article{WangClLiFr20,
  title={Parallel Bayesian Global Optimization of Expensive Functions},
  author={Jialei Wang and Scott C. Clark and Eric Liu and Peter I. Frazier},
  journal={Operations Research},
  volume=68,
  number=6,
  pages={1850--1865},
  year=2020
}

@inproceedings{Mockus05,
  title={On bayesian methods for seeking the extremum},
  author={Jonas Mo{\v{c}}kus},
  booktitle="Optimization Techniques IFIP Technical Conference Novosibirsk, July 1--7, 1974",
  year = 1975,
  publisher="Springer Berlin Heidelberg",
  address="Berlin, Heidelberg",
  pages="400--404"
}

@techreport{GinsbourgerRiCa08,
  author = {David Ginsbourger and Rodolphe Le Riche and Laurent Carraro},
  title = {A Multi-points Criterion for Deterministic Parallel Global Optimization based on Gaussian Processes},
  year = 2008,
  number = {HAL-00260579},
}

@inproceedings{WuFr16,
  author = {Jian Wu and Peter I. Frazier},
  title = "The Parallel Knowledge Gradient Method for Batch Bayesian Optimization",
  booktitle = nips16,
  year = 2016
}

@inproceedings{GonzalezDaHeLa16,
  author = {Javier Gonzalez and Zhenwen Dai and Philipp Hennig and Neil Lawrence},
  title = "Batch Bayesian Optimization via Local Penalization",
  booktitle = aistat16,
  year = 2016
}

@inproceedings{WuFr19,
  author = {Jian Wu and Peter I. Frazier},
  title = "Practical two-step look-ahead Bayesian optimization",
  booktitle = nips19,
  year = 2019
}

@inproceedings{GonzalezOsLa16,
  author = {Javier Gonzalez and Michael Osborne and Neil Lawrence},
  title = "GLASSES: Relieving The Myopia Of Bayesian Optimisation",
  booktitle = aistat16,
  year = 2016
}

@inproceedings{JiangChGoGa20,
  author = {Shali Jiang and Henry Chai and Javier González and Roman Garnett},
  title = "BINOCULARS for Efficient, Nonmyopic Sequential Experimental Design",
  booktitle = icml20,
  year = 2020
}

@inproceedings{LamWiWo16,
  author = {Remi R. Lam and Karen E. Willcox and David H. Wolpert},
  title = "Bayesian optimization with a finite budget: an approximate dynamic programming approach. ",
  booktitle = nips16,
  year = 2016
}

@inproceedings{YueAl20,
  author = {Xubo Yue and Raed AL Kontar},
  title = "Why Non-myopic Bayesian Optimization is Promising and How Far Should We Look-ahead? A Study via Rollout",
  booktitle = aistat20,
  year = 2020
}

@inproceedings{JiangJiBaKaGaGa19,
  author = {Shali Jiang and Daniel Jiang and Maximilian Balandat and Brian Karrer and Jacob Gardner and Roman Garnett},
  title = "Efficient Nonmyopic Bayesian Optimization via One-Shot Multi-Step Trees",
  booktitle = nips20,
  year = 2020
}




==> oae_dp.tex <==
\section{Optimal Adaptive Experimentation as a Dynamic Program}
\label{section:oae-dp}

% \hn{DJ thought the formulation was bayesian. Say oae dp is really hard both modeling and compute wise, then put the full bayesian version in the appendix.}
The goal of the experimenter is to
select sampling allocations $p_t$ for the batched adaptive experiment to optimize the objective. Importantly, the experimenter adaptively selects $p_t$ based on
observed data during the experiment. This problem can be formulated as a dynamic program 
over policies $\pi = \{\pi_{t} \}_{t=0}^{T}$ which map data to sampling decisions\footnote{Note that it is common that $p_t$ is referred to as a \emph{sampling policy} in the literature. In our case, because of the existence of a ``policy'' $\pi_t$ for selecting $p_t$, it is important to note the crucial distinction between $\pi_t$ and $p_t$.} $p_t$:
\[
  \pi_{t}: \mc{H}_{t} \mapsto p_{t}(\cdot \,|\, x)  \in \Delta_{K}.
\]
Abusing notation, it is convenient to also use $\pi_{t}(\cdot \,|\,x, \mc{H}_{t})$ to describe
the sampling allocation $p_t$ prescribed by the policy $\pi_t$ given the current history:
\[
    \pi_{t}(\cdot \,|\, x, \mc{H}_{t}) \equiv \pi(\mc{H}_{t}) \in \Delta_{K}.
\]
We adopt this notation in contexts when the distinction is clear.

The objective is to minimize a sum of cost functions $c_{t}(p_{t})$ given the sampling allocations $p_{t}$ played by the experimenter. For example, for cumulative regret, the cost function would be:

\vspace{1em}
\begin{example}[Cumulative regret]
To define \emph{cumulative regret}, we consider sampling allocations made \emph{during} the experiment (i.e. $p_{t}$ for $t<T$):
\begin{align}
    \label{eq:cumulative_regret}
    \mathsf{Regret}_{T}(p_{0:T}) 
    & := \E \left[
        \sum\nolimits_{t=0}^{T-1} c_{t}(p_{t}) \right] = \sum_{t=0}^{T-1} n_{t} \, \E_{x\sim\mu_{t}} \left[\max_{a} \, r(x,a) -   \sum\nolimits_{a} p_{t}(a|x)\,r(x,a) \right], 
\end{align} 
where we have defined
$c_t(p_t) = n_{t}\, \E_{x\sim\mu_{t}} \bigl[\max_{a} r(x,a) - \sum\nolimits_{a}
  p_{t}(a|x) \, r(x,a) \bigr]$. Note that the regret of each period is weighted by the size of the batch $n_t$.
\end{example}

Since the cost function may depend on the reward function $r(x,a)$, which is unknown to the experimenter, they must make decisions conditional on the current history of observations thus far:
\[
c_{t}(p_{t}|\mc{H}_{t}) := \E[c_{t}(p_{t})|\mc{H}_{t}]
\]
With this notation, we can describe the optimal adaptive experimentation problem as the following constrained dynamic program, given 

% The dynamic program for optimal adaptive experimental design is as follows,
\begin{definition}
The \textbf{optimal adaptive experimentation dynamic program} $(\origdp)$ is an MDP for which the state at epoch $t$ is the history $\mc{H}_{t}$
and the actions are sampling allocations $p_{t}(\cdot \, |\, x) \in \Delta_{K}$.
The state transition from epoch $t$ to epoch $t+1$, given history $\mc{H}_{t}$ and sampling allocation $p_{t}(\cdot \,|\, x)$ is given by
\begin{subequations}
  % \label{eqn:reward_transition}
  \begin{align*}
    % & \pi(\cdot | X_{t,i}, \mc{H}_{t}) \in \Delta_{K}, && \quad \forall t = 0,...,T,\forall i \in [n_{t}]   \\
      & X_{t,i}  \simiid \mu_{t}, \quad
        A_{t,i}  \simiid p_{t}(\cdot \,|\,X_{t,i}), \quad
        R_{t,i} \simiid \nu(\cdot \,|\, X_{t,i}, A_{t,i}), \quad
        \forall i \in [n_{t}] \\
      & \mc{D}_{t}  = \{ (X_{t,i}, A_{t,i}, R_{t,i}) \}_{i=1}^{n_{t}},
        \quad
        \mc{H}_{t+1} = \mc{H}_{t} \cup \mc{D}_{t}.
  \end{align*}
\end{subequations}
The objective is to minimize cost over policies $\pi_{t}: \mc{H}_{t} \mapsto p_{t}(\cdot \,|\, x)$, subject to constraints:
\begin{align}
  \label{eqn:general-dp}
  \tag{OAE-DP}
  \minimize_{\pi}
  \left\{
  J_{T}(\pi) := \E \left[\sum\nolimits_{t=0}^{T} c_{t}(\pi_{t} | \mc{H}_{t}) \right]
  ~~\Big|~~ 
  \sum\nolimits_{t=0}^{T} g_{t}\left(\pi_{t} \right)\leq B\right\}.
  % \sum\nolimits_{t=0}^{T} g_{t}\left(\pi_{t}, \mc{H}_t, X_{t, \cdot}\right) \leq B\right\}.
\end{align}
\end{definition}
\noindent Here, the transition probabilities are unknown to the experimenter
as the conditional reward distribution $\nu(\cdot \,|\,X_{t,i}, A_{t,i})$ is
unknown (otherwise there is no need to experiment).

% A classical solution to this challenge is to express modeler's epistemic uncertainty on $\nu$---which gets resolved with infinite data---using Bayesian principles. We consider a Bayesian model over $\nu$ such that given the history $\mc{H}_t$, where $\beta_t$ parameterizes the posterior distribution
% $\nu \mid \mc{H}_t$:
% \begin{equation}
%   \label{eqn:bayes-mdp-posterior}
%   \nu \mid \mc{H}_t \sim \P_{\beta_t(\mc{H}_t)}(\nu = \cdot).
% \end{equation}
% \drj{Note that we use $\beta_t$ later as the posterior mean. Might want to change this to something else} If we marginalize out the unobserved $\nu$ according to some prior,
% the~\ref{eqn:general-dp} problem becomes a partially observable MDP (POMDP),
% which is notoriously difficult to estimate and solve. \drj{Usually in POMDP, only the state is unobserved. But here our state is $\mc H_t$, which is fully observed, so I'm unclear on what the POMDP is.} However, if we augment the
% observed states of~\ref{eqn:general-dp} with the posterior states $\beta_t$,
% we arrive at a standard MDP.  In this MDP, the state transitions from $\beta_t$ to
% $\beta_{t+1}$ correspond to posterior updates based on the most recent data
% $\mc{D}_{t+1}$.  \drj{Do we mean state is $(\mc H_t, \beta_t)$? Upon more thought, I'm a little confused about this point because $\beta_t$ is derived from the information content in $\mc H_t$, so I'm not sure the distinction of adding $\beta_t$. Maybe the distinction between OAE-DP vs its Bayesian MDP variant is actually the exact same MDP formulation, but the distinction is just under what lens it is viewed through (ie Bayesian or not) PLUS an assumption on how the posterior is parameterized?}
% \jw{I may be wrong but from my understanding, the Bayesian MDP formulation explicitly specifies a Bayesian model of 
% the environment while the OAE-DP is over the true unknown environment. Additionally, the state 
% $\beta$ is meant to emphasize that compressing the history into $\beta$ is all that is necessary to make decisions.} \drj{In the text it says we are ``augmenting the observed states with posterior states'' suggesting state = $(\mc H_t, \beta_t)$, which was confusing.} \drj{Thanks Jimmy, let's discuss the OAE-DP a bit more in the next meeting. Still a bit confused.}

% We refer to this formulation as the \emph{Bayesian MDP formulation} for~\ref{eqn:general-dp}. Bayesian MDPs have long been used to formalize the exploration
% versus exploitation trade-off~\cite{GhavamzadehMaPiTa15, PengChChFu18}. When the modeler is
% willing to assume a Bayesian model for unit-level rewards, Bayesian adaptive
% experimentation methods~\cite{ChalonerVe95, RyanDrMcPe16, FosterIvMaRa21,
%   JorkeLeBr22} optimize expected information gain, whereas Bayesian bandit
% algorithms consider finite actions and propose one- or two-step lookahead
% policies tailored to specific objectives~\citep{GuptaMi96,ChickIn01, HeChCh07,
%   FrazierPoDa08, ChickBrSc10, FrazierPo10, ChickGaYa22}.
%   There have been attempts in the Bayesian optimization literature to design non-myopic acquisition functions around Bayesian MDPs \citep{gonzalez2016glasses,lam2016bayesian,yue2020non,jiang2020binoculars,lee2020efficient,jiang2020efficient,lee2021nonmyopic,astudillo2021multi}, but the solution methods are often brittle and errors due to model (typically Gaussian procceses) misspecification can easily propagate with longer lookahead horizons \citep{yue2020non}.
  
% While conceptually appealing, the Bayesian MDP reformulation using posterior
% states~\eqref{eqn:bayes-mdp-posterior} has practical drawbacks. It requires
% the modeler to posit a Bayesian model for individual unit-level rewards
% $\nu(\,\cdot \,|\, x, a)$, which is a daunting modeling task that almost always
% leads to misspecified models.  In the ASOS fashion retailer example, this is
% equivalent to positing a Bayesian model for individual user behavior.
% \jw{ I'm a bit confused about the distinction between the "Bayesian MDP" and what 
% we end up solving in the BLDP. The M-estimation formulation still requires that 
% we have a parametric model for the reward function, such as linear or logistic. It seems to 
% me that the main distinction is that the BLDP justifies the Gaussian assumption whereas in 
% other Bayesian formulations they may assume Gaussianeity without justification. I didn't touch 
% this section as a result.} \drj{I tend to agree that this point is confusing. Therefore, I suggest making the OAE-DP Bayesian as well, with $\mc H_t$ as the state along with a ``general'' posterior $\nu | \mc H_t$. And then we only have two concepts, OAE-DP and BLDP. We can thus skip the step to convert to Bayesian MDP, which is confusing.}

==> old_setting.tex <==

\label{section:setting}
 


\section{Batched Experiment Design}
Mirroring current practices for real-world experiments, we consider an experiment composed of $T$ sequential epochs (or ``batches''). 
There are $K$ treatment arms or actions. At each epoch $t$, a batch of $b_t$ sampling units arrive and 
are assigned to treatment arms by the experimenter according to a {\bf sampling allocation} $\pi_{t}\in \Delta_{K}$. 
$\pi_t$ is a probability distribution over treatment arms and is the core decision made by the experimenter. Each 
unit has a context $x\in \mathbb{R}^{p}$ and the expected reward $r(x,a)$ of assigning an action $a\in [K]$ to $x$ is
given by a general parametric model:
\begin{equation}\label{eq:parametric reward model}
r(x,a)=f(x, a; \theta^\ast)
\end{equation}
where  $\theta^\ast \in\mathbb{R}^{d}$ is an unknown
coefficient vector. Common parametric models include the linear contextual bandit model 
\begin{equation}\label{eq:linear reward model}
    r(x,a)=\phi(x,a)^{\top}\theta^\ast,
    \end{equation}
and logistic contextual bandit model 
\begin{equation}\label{eq:logistic reward model}
    r(x,a)=\dfrac{1}{1 + \exp(-\phi(x,a)^{\top}\theta^\ast)},
    \end{equation}
where $\phi(x_{i},a_{i}):\mathcal{X}\times[K]\to\mathbb{R}^{d}$ is a known feature mapping.
Instead of observing the true expected reward, we observe noisy observations $R(x,a)$ where
\begin{equation}\label{eq:parametric reward model}
    R(x,a)=r(x,a) + \varepsilon_{i} = f(x, a; \theta^\ast)+\varepsilon_{i},
    \end{equation}
and $\varepsilon_{i}$ are iid mean zero random variables with a fixed, known measurement variance $\text{Var}(\varepsilon_{i})=s^{2}$.
While the variance is known, all other distributional characteristics (e.g. whether the noise $\varepsilon$ is Gaussian, exponential, or Poisson) are unknown.

Generically, we can allow the sampling allocation to depend on the 
unit context, i.e. the treatment arm assigned to context $x$ is drawn from a
distribution $\pi_{t}(x)$, with probability $\pi_{t}(a|x)$. Examples of contexts include highly user-specific features to 
broader day-of-the-week or geographic fixed effects.
After assigning treatments arms to sampling units, the experimenter observes the reward for each context action pair. 
Using this information, they can update the sampling allocation $\pi_{t+1}$ for the next batch.

\subsection{Experimental Objectives and Constraints}

An experimenter may wish to design adaptive experiments aligned with their preferences by optimizing 
a variety of possible objectives. These objectives can be expressed as  
per-period objective functions $v_t$ that depend on the sampling allocation at each epoch $t$, yielding the dynamic program:  
\begin{align}
    \label{eqn:general-dp}
    \min_{\pi_{0},\ldots,\pi_{T}} \E^{\pi}  \left[
            \sum_{t=0}^{T} v_{t}(\pi_{t})
           \right]
  \end{align}

We illustrate some common examples. For instance, the standard cumulative regret metric can be written as 
\begin{align}
    \label{eq:cumulative_regret}
    \text{CumulativeRegret}(\pi_{0:T}) &= \E^{\pi}  \left[\sum_{t=0}^{T} v_{t}(\pi_{t})\right] \\
    &= \E^{\pi} \left[\sum_{t=0}^{T} \E_{x\sim\mu_{t}} \left[\max_{a} r(x,a) - \sum\nolimits_{a} \pi_{t}(a|x)r(x,a) \right] \right]
\end{align} 
where $v_t(\pi_t) = \E_{x\sim\mu_{t}} \left[\max_{a} r(x,a) - \sum\nolimits_{a} \pi_{t}(a|x)r(x,a) \right]$. This measures 
the regret incurred within an experiment. 

Typically at the end of the experiment, the experimenter will select a treatment arm to deployed
based on the experimental results (or at least selected to be tested further).
We denote $\mu$ as the {\bf reference distribution} over contexts used to evaluate the final performance.
Due to its practical importance, we discuss the {\bf simple regret} metric, 
which measures the sub-optimality of the final arm selection $\pi_{T}\in \Delta_K$ with the treatment arm
with the highest average reward according to $\mu$.
\begin{equation}
    \label{eq:simple_regret}
    \text{SimpleRegret}(\pi_{T}) = \E^{\pi} \left[v_T(\pi_T)\right] = \E^{\pi} \left[\max_{a} \E_{x\sim\mu}[r(x,a)] - \sum\nolimits_{a} \pi_{T}(a) \E_{x\sim\mu}[r(x,a)]\right],
\end{equation}
where $v_t(\pi_t) = 0$ for $t < T$. 
This measures the efficacy of the adaptive experimental design in identifying the treatment arm with the highest expected reward,
rather than minimizing the regret incurred during the experiment.

Another relevant task is identifying the optimal policy for assigning treatment arms to contexts, rather
than identifying a single best arm to be deployed for all contexts. We denote {\bf policy regret} as the regret 
incurred by the experimenter's final policy selection $\pi_{T}$ compared to the optimal policy,
across the reference distribution $\mu$ over contexts.
\begin{equation}
    \label{eq:policy_regret}
    \text{PolicyRegret}(\pi_{T}) = \E^{\pi} \left[v_T(\pi_T)\right] = 
    \E^{\pi} \left[\E_{x\sim\mu}[\max_{a} r(x,a)] - \E_{x\sim\mu}\left[  \sum\nolimits_{a} \pi_{T}(a|x)r(x,a) \right] \right]
\end{equation}
This is relevant for personalization. 

{\color{blue} We could also explain the objectives tied to each of our examples including the Meta example, and ridesharing constraint example. 
Meta example could show a non-standard objective such as top K instead of top 1, and maybe we can also do some sort of 
simple + cumulative regret tradeoff (don't want users leaving platform). The ridesharing example would showcase constraints. }

\subsection{Intractable Dynamic Program} 

Ideally, the experimenter would like to directly solve the dynamic program \eqref{eqn:general-dp} to find the optimal sampling allocation policy. 
However, this is intractable ... 

As a result, policies like Thompsons Sampling and UCB are popular ... 

\section{BLDP: Batched Limit Dynamic Program}

Since the dynamic program \eqref{eqn:general-dp} is intractable due to its high, possibly infinite dimensionality, we need some form 
of structure. Our main observation is that batches, which are used in practice anyways, greatly simplify the problem. When planning 
the experiment, a practitioner may assume that the rewards follow some parametric model as in \eqref{eq:parametric reward model}. Consider a batch 
$b_t$ of samples in the form of context, action, reward pairs $\mc{D}_t := \{x_i, a_i, r_i\}_{i=1}^{b_t}$. To estimate the parameter $\theta^\ast$ 
associated with the reward model, it is natural for an experimenter to use a general m-estimator and compute a 
summary statistic by minimizing some empirical loss function 
\begin{equation}
    \label{eq:m-estimation-loss}
    \hat{\theta}_{t}=\arg\min_{\theta} \frac{1}{b_t} \sum_{i=1}^{b_t }\ell_{\theta}( x_i, a_i).
\end{equation} 
For example, to estimate the linear coefficients in linear regression, one normally solves for 
\begin{equation}
    \hat{\theta}_{t}=\arg\min_{\theta}\frac{1}{b_t} \sum_{i=1}^{b_t }\ell_{\theta} (x_i, a_i) := \frac{1}{b_{t}}\sum_{i=1}^{b_{t}}(r_{i}-\phi(x_{i},a_{i})^{\top}\theta)^{2}. 
\end{equation}
If one wanted to use a robust loss function, one could use the Huber loss or Tukey's Biweight loss. For general maximum likelihood problems, 
one minimizes the negative log likelihood 
\begin{equation}
    \hat{\theta}_{t}=\arg\min_{\theta}\frac{1}{b_t} \sum_{i=1}^{b_t }\ell_{\theta} (x_i, a_i) := -\frac{1}{b_{t}}\sum_{i=1}^{b_{t}}\log p(r_{i}|x_{i},a_{i},\theta).
\end{equation}

As $b_t \to \infty$, under suitable conditions, the estimator in \eqref{eq:m-estimation-loss} is asymptotically distributed as according to a Normal distribution 

\begin{equation}
    b_{t}^{1/2}V(\hat{\theta}_{t}-\theta^\ast) \to N(0, \Gamma)
\end{equation}
where $V = \E^{\pi} [\nabla \ell_{\theta^\ast}(X_{i}, A_{i})]$ is the Hessian of the expected loss function evaluated at $\theta^\ast$ and \\
$\Gamma = \E^{\pi} [\nabla \ell_{\theta^\ast}(X_{i}, A_{i}) \nabla \ell_{\theta^\ast}(X_{i}, A_{i})^\top ]$ is the Fisher information matrix.

\subsection{Bayesian Model and Markov Decision Process}







% \paragraph{Bayesian Linear Model}
% % A standard
% % model for incorporating this information is the Bayesian linear regression
% % model, which maintains a Gaussian posterior distribution over $\beta^{*}$. The asymptotic normality
% % of the OLS estimator computed with batched rewards suggests that this
% % model may be appropriate under batch updates. 
% We consider an experimenter with a prior belief over $\beta^{*}$, $N(\beta_{0},\Sigma_{0})$
% with mean $\beta_{0}\in\mathbb{R}^{d}$ and $\Sigma_{0}\in\mathbb{R}^{d\times d}$, possibly informed
% by a reservoir of previous experiments or domain knowledge. 
% After each epoch $t$, the experimenter updates their posterior beliefs
% $(\beta_{t},\Sigma_{t})$ after assigning actions according to $\pi_{t}$
% and calculating the OLS estimator $\hat{\beta}_{t}$. The experimenter
% updates their posterior using the normal approximation \eqref{eq:normal_approx}, updating 
% $\Sigma_{t+1} =\left(s^{-2}n_{t}\Gamma_{t}(\pi_{t})+\Sigma_{t}^{-1}\right)^{-1}$ and $\beta_{t+1}=\Sigma_{t+1}(\Sigma_{t}^{-1}\beta_{t}+s^{-2}n_{t}\Gamma_{t}(\pi_{t})\hat{\beta}_{t})$.

% We can think of the belief $(\beta_{t},\Sigma_{t})$ as the states
% of a Markov Decision Process (MDP), where states transitions are determined
% by the sampling allocation $\pi_{t}$. We can reparameterize the state
% transition using the posterior predictive distribution of $\hat{\beta}_{t}$
% given $\beta_{t},\Sigma_{t}$. \begin{proposition} \label{prop:state_transition}Let
% $Z_{1},...,Z_{T}$ be standard iid $N(0,I_{d})$ random vectors.
% The system governed by the posterior updates
% has the same joint distribution as that with the following state transition:
% \begin{align}
% \Sigma_{t+1} & =\left(s^{-2}n_{t}\Gamma_{t}(\pi_{t})+\Sigma_{t}^{-1}\right)^{-1}\label{eq:pred_posterior_update}\\
% \beta_{t+1} & =\beta_{t}+\left(\Sigma_{t}-\Sigma_{t+1}\right)^{1/2}Z_{t}
% \end{align}
% \end{proposition} The proof is in Appendix \ref{proof:state_transition}. The state transitions (\ref{eq:pred_posterior_update})
% quantifies the future reduction of uncertainty given a sampling allocation
% $\pi_{t}$, and can be rolled out for several steps.
% % Given this structure, it is natural for the experimenter to consider
% % Markovian sampling allocation policies $\pi_{t}(a|x,\beta_{t},\Sigma_{t})$,
% % which determines the allocation based on the current posterior $(\beta_{t},\Sigma_{t})$
% % as well as the context. 
% % As an example, we can express the standard
% % Gaussian Thompson Sampling policy as:
% % \[
% % \pi^{\text{TS}}(a|x,\beta_{t},\Sigma_{t})=\mathbb{P}\left(a=\arg\max_{a'\in[K]}\phi(x,a')^{\top}(\beta_{t}+\Sigma_{t}^{1/2}Z)\right)
% % \]
% Crucially, this framework offers a \emph{smoothed} model of partial
% feedback, for which state transitions are differentiable in the sampling
% allocation $\pi_{t}$ (as $\Gamma_{t}(\pi)$ is linear in $\pi$).
% This enables the use of autodifferentation frameworks (e.g. PyTorch \citep{PyTorch19}
% or Tensorflow \citep{TensorFlow16}) to calculate gradients of objectives with respect to the sampling
% allocation along a sample path $(Z_{0},...,Z_{T})$, and optimize
% via gradient descent.

% \paragraph{Bayesian Objective}
% The experimenter's objective consists of
% a sum of per-period rewards $v_{s}$, which can depend on the posterior
% state $(\beta_{s},\Sigma_{s})$ and the sampling allocation $\pi_{s}$
% at period $s$. Given a sampling policy $\pi=\{\pi_{t}(\cdot|\beta_{t},\Sigma_{t})\}_{t=0}^{T}$,
% the value function at time $t$ is
% \[
% V_{t}^{\pi}(\beta_{t},\Sigma_{t})=\mathbb{E}\left[\sum_{s=t}^{T}v_{s}(\pi_{s},\beta_{s},\Sigma_{s})\right].
% \]
% % This model can incorporate a variety of different objectives. If the
% % experimenter cares about maximizing cumulative rewards, then $v_{s}$
% % is the total expected reward collected in period $s$:
% % \[
% % v_{s}(\pi_{s},\beta_{s},\Sigma_{s})=\mathbb{E}_{X\sim\mu_{s}}\left[\sum_{a\in[K]}\pi_{s}(a|X)r(X,a)\right]=\mathbb{E}_{X\sim\mu_{s}}\left[\sum_{a\in[K]}\pi_{s}(a|X)\phi(X,a)^{\top}\beta_{s}\right].
% % \]
% If the experimenter is maximizing policy reward or
% minimizing policy regret, then they would only experience a terminal
% reward $v_{T}$ (i.e. $v_{s}=0$ for $s<T$). One can show that minimizing
% Bayesian policy regret is equivalent to maximizing the policy reward
% under the policy that acts greedily according to final posterior ($\beta_{T}, \Sigma_{T})$:
% \[
% v_{T}(\pi_{T},\beta_{T},\Sigma_{T})=\mathbb{E}_{X\sim\mu}\left[\max_{a}\phi(X,a)^{\top}\beta_{T}\right]
% \]

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:


==> overview.tex <==
\section{Overview of the Paper}

In this section, we give a brief overview of the high-level ideas of our paper (with mathematical notation) before moving on to the full exposition. {\color{red}This section uses new notation!}

% We first build the foundations necessary to construct the $\model$. To approximately solve the $\model$, we introduce a simple 
% model-predictive control (MPC) based policy $\algo$. Finally, we highlight strong empirical performance ... 

\subsection{Batched Experiment Setting}
Given the widespread practice of conducting experiments in 
a few, large batches, we consider an experiment composed 
of $T$ sequential epochs (or ``batches'') and $K$ arms. 
At each epoch $t \in \{0, 1, \ldots, T-1\}$, a batch of $n_t$ 
sampling units arrive with contexts $\{X_{t,i}\}_{i=1}^{n_t}$, 
where $X_{t,i}\in \mathbb{R}^{p}$ and is drawn from a context distribution $\mu_t$. 
There is also a \emph{population context distribution} $\mu$, which, 
notably, may differ from $\mu_t$, allowing us to model within-experiment 
context distributions that differ from the population distribution. 

An action $A_{t,i} \in [K]$ is assigned to unit $i$ via an \emph{action selection kernel} $p_t$, where $p_t( \cdot \, | \, x)$ is a probability distribution over $[K]$ for each possible context $x$. After assigning an action $A_{t,i} \sim p_t(\, \cdot \, | X_{t,i})$ to unit $i$, we observe a noisy reward  
\begin{equation}
  R_{t,i} %= R(X_{t,i},A_{t,i}) 
  = r(X_{t,i},A_{t,i};\theta^{*}) + \varepsilon_{t,i},
\end{equation} 
where $\varepsilon_{t, i}$ is a noise term with variance $s^{2}$ and $r(x,a;\theta^{*})$ is a parametric model with unknown parameter $\theta^{*}\in \Theta\subseteq \mathbb{R}^d$. 


We refer to $t \in \{0, 1, \ldots, T-1\}$ as the \emph{within-experiment} phase. During this phase, the experimenter chooses action selection kernels $p_t$ for the purpose of exploration. After the experimentation batch $T-1$ ends, we enter period $T$, which we call the \emph{post-experiment} phase. Here, the experimenter commits to a final action selection kernel $p_T$ (i.e., the ``launch decision''). The quality of $p_T$ is evaluated under the population context distribution $\mu$.

\looseness-1 The experimenter's goal is to accurately estimate $\theta^{*}$, as 
identifying the unknown coefficient is sufficient to identify the optimal action. The parameter $\theta^{*}$ can be expressed in terms of minimizing a loss function $l$ under the population context distribution $\mu$ and a reference action selection kernel $p$:
\begin{align}
  \label{eq:population_loss_intro}
  &\theta^{*} = \arg \min_{\theta \in \Theta} \, \E \bigl [\ell(\theta \, | \, X_i, A_i, R_i) \bigr], 
  \quad X_{i} \sim \mu,\;A_{i} \sim p(\,\cdot\,|\, X_i), \; \text{and} \;  R_i = r(X_{i},A_{i};\theta^{*}) + \varepsilon_{i}
  %, R_{i} \sim p(\cdot | x,a,\theta^{*})
\end{align}
where $\varepsilon_i$ has variance $s^2$. To estimate the unknown $\theta^{*}$ given a batch of context, action, and reward tuples $\{(X_{i}, A_{i}, R_{i})\}_{i=1}^{n}$, it is natural for the experimenter to use an M-estimation procedure and compute the estimator $\hat{\theta}$ that minimizes the empirical counterpart of \eqref{eq:population_loss_intro}:
\begin{equation}
  \label{eq:ERM_intro}
  \hat{\theta} = \arg \min_{\theta \in \Theta} \; \frac{1}{n}\sum_{i=1}^{n} \ell(\theta \,|\, X_{i}, A_{i}, R_{i}).
\end{equation}
Letting $\phi(x,a)\in \R^{d}$ be known feature vector, linear and logistic models can be realized using the following losses: 
\[
  \ell(\theta \, | \, X_{i},A_{i},R_{i}) = \bigl| R_{i} - \phi(X_{i},A_{i})^{\top} \theta \bigr|^{2},
  \quad \ell(\theta | X_{i},A_{i},R_{i}) = \log\left( 1 + e^{-R_{i} \phi(X_{i},A_{i})^{\top} \theta} \right).
\] 
\subsection{Objective of the Experiment}
The action selection kernels $p_t$ are chosen adaptively given the history of observations
\[
\bigl (\{X_{0,i}\}_{i=1}^{n_0}, \{A_{0,i}\}_{i=1}^{n_0}, \{R_{0,i}\}_{i=1}^{n_0}, \ldots, \{X_{t-1,i}\}_{i=1}^{n_{t-1}}, \{A_{t-1,i}\}_{i=1}^{n_{t-1}}, \{R_{t-1,i}\}_{i=1}^{n_{t-1}} \bigr)
\]
The experimenter sets $p_t$ with the intention of minimizing the following objective:
\begin{equation}
  \label{eq:general-dp-intro}
    \underbrace{\sum_{t=0}^{T-1} \E_{x\sim\mu_t} \bigl[ c_{t}(x, p_{t}, \theta^*) \bigr]}_{\text{within-experiment regret/cost}} + \underbrace{ \vphantom{ \sum_{t=0}^{T-1} } \E_{x\sim\mu} \bigl[ c_T(x, p_T, \theta^*) \bigr],}_{\text{post-experiment regret/cost}}
\end{equation}
where $\{c_t\}$ represent the per-period regret (and/or cost) functions. Note that the post-experiment term is evaluated under the population context distribution $\mu$, while the other terms are evaluated under the within-experiment context distributions $\mu_t$.
% At each epoch $t$, the experimenter's core decision is to assign units $x$ to treatment arms $a$ using a sampling policy $\pi_{t}(a|x)\in \Delta_{K}$.
% The experimenter has an objective and sets $\pi_{t}$ with the intention of minimizing this objective. Generally, this can be expressed as the following dynamic program:
% \begin{equation}
%   \label{eq:general-dp-intro}
%   \min_{\pi_{0},\ldots,\pi_{T}} \E^{\pi}  \left[
%           \sum_{t=0}^{T} v_{t}(\pi_{t})
%          \right]
% \end{equation}
The standard cumulative regret metric can be formulated by letting
\[
c_t(x, p_t, \theta^*) = \max_{a} \, r(x,a; \theta^*) - \sum\nolimits_{a} p_{t}(a\,|\,x) \, r(x,a;\theta^*).
\]
At this point, attempting to directly optimizing \eqref{eq:general-dp-intro} to obtain an adaptive policy for selecting $\{p_t\}_{t=0}^T$ is not immediately tractable due to the dependence on the observation history, a high-dimensional and complex object.

% Directly optimizing \eqref{eq:general-dp-intro} is exceptionally difficult outside of trivial settings as it 
% requires understanding dynamic considerations of 
% how the treatment allocation at each stage affects future
% treatment allocations and the final performance objective. To elaborate:  
% \begin{enumerate}
%   \item This requires anticipating the value of
%   data collected in future stages which is an especially difficult task when the distribution of the
%   rewards is unknown, as is commonly the case in practice. 
%   \item It is difficult to frame the problem
%   as a standard dynamic program, as it is unclear whether there is an appropriate choice of state
%   space that follows Markovian dynamics in this unstructured environment.
%   \item The action space
%   involves all possible allocations of treatments to units, which can be intractably large considering the
%   large sample sizes featured in modern experiments. At best, this problem is a high-dimensional,
%   partially observable Markov decision process (POMDP) with a combinatorial action space – an
%   NP-complete class of problems.
% \end{enumerate}

\subsection{Asymptotic Bayesian Model}
{\color{red}TODO} Experimenters often make decisions based on estimates of sufficient statistics (i.e. mean, coefficient, etc.). The 
intuition behind the $\model$ is that one only needs to understand how beliefs about this statistic are 
expected to change upon observing new data, rather than modeling each individual reward. To do so, we construct an asymptotically valid Bayesian model. 
At epoch $t$, the experimenter observes $\mc{D}^{t} := \{X_{i}^{t}, A_{i}^{t}, R_{i}^{t}\}_{i=1}^{n_{t}}$. Under conditions and appropriate scaling specified in Section \ref{section:model}, as the number of samples 
$n\to\infty$, the estimator $\hat{\theta}_{t}$ \eqref{eq:ERM_intro} is approximately normal 
\begin{equation}
  \label{eqn:approx_normality}
    \hat{V}_{t}\hat{\theta}_{t} \sim  
    N \left(V_{\mu_{t}}(\pi_{t})\theta^{*}, \frac{1}{n_{t}}\Gamma_{\mu_{t}}(\pi_{t})  \right).
\end{equation}
where $V_{\mu_{t}}(\pi_{t}) = \E[\nabla^{2} \ell_{\theta^{*}}(\mc{D}^{t}_{i})]$, 
$\hat{V}_{t} = \frac{1}{n_{t}}\sum_{i=1}^{n_{t}} \nabla^{2} \ell_{\hat{\theta}_{t}}(\mc{D}^{t}_{i})$ 
and  $\Gamma_{\mu_{t}}(\pi_{t}) = \E[\nabla \ell_{\theta^{*}}(\mc{D}^{t}_{i}) \nabla \ell_{\theta^{*}}(\mc{D}^{t}_{i})^\top]$.
Instead of "observing" and modeling the entire data $\mc{D}^{t}$, we treat our "observation" at time $t$ 
as the statistic $\hat{\theta}_{t}$. Then, \eqref{eqn:approx_normality} can be 
interpreted as an approximate Gaussian likelihood of the summary statistic $\hat{\theta}_{t}$ under a parameter $\theta$.
This idea naturally suggests a conjugate Gaussian prior. Let $\Lambda_{\mu_{t}}(\pi_{t}) = 
V_{\mu_{t}}(\pi_{t})\Gamma_{\mu_{t}}^{\dagger} (\pi_{t})V_{\mu_{t}}(\pi_{t})$ where $\dagger$ is the pseudo inverse. If the experimenter starts with a prior $N(\theta_{t},\Sigma_{t})$, 
they will approximately update their beliefs according to the posterior update equations 
\begin{equation}
  \label{eqn:posterior_update}
  \theta_{t+1} = \Sigma_{t+1} \left( \Sigma_{t}^{-1}\theta_{t} 
  + \frac{1}{n_{t}} V_{\mu_{t}}(\pi_{t})\Gamma_{\mu_{t}}^{\dagger} (\pi_{t}) \hat{V}_{t}\hat{\theta}_{t} \right),
  \qquad \Sigma_{t+1}^{-1} = \Sigma_{t}^{-1} + n_{t}\Lambda_{\mu_{t}}(\pi_{t}).
\end{equation}
\subsection{Batched Limit Dynamic Program}
Notably, these approximate, asymptotic update equations are directly controlled by the action selection kernels $p_{t}$. If we know (or can approximate) the context distributions $\mu_{t}$, then given an initial belief $(\theta_{t}, \Sigma_{t})$, we have an exact, closed form expression for the posterior belief $(\theta_{t+1}, \Sigma_{t+1})$ by choosing $p_t$.
%The experimenter can easily encode their original objectives within this Bayesian model by 
%specifying ${\{v_{t}(\pi_{t}, \theta_{t}, \Sigma_{t})\}_{t=0}^{T}}$. 
Thus, we can treat each belief $(\theta_{t}, \Sigma_{t})$ as a \emph{state}, forming a Markov decision process (MDP) with an \emph{action space} consisting of action selection kernels $p_t(\cdot \, |\, x) \in \Delta_K$, a \emph{transition function} given by \eqref{eqn:posterior_update}, and a \emph{cost} given by 
\[
c_t(p_t, \theta_t, \Sigma_t) = \E_{x\sim\mu_t} \, \E \bigl[ c_t(x, p_t, \theta^*) \, | \, \theta_t, \Sigma_t \bigr] \quad \text{for} \quad t \in \{0, 1, \ldots, T-1\},
\]
and $c_T(p_T, \theta_T, \Sigma_T)= \E_{x\sim\mu} \, \E \bigl[ c_T(x, p_T, \theta^*) \, | \, \theta_T, \Sigma_T \bigr]$.
% which consists of the following: 
% (1) \textbf{State Space} consisting of beliefs $(\theta_{t}, \Sigma_{t}) \in \mathcal{S}$.
% (2) \textbf{Action Space} consisting of sampling policies $\pi_{t} \in \Delta_{K}$.
% (3) \textbf{Transition Function} $T: \mathcal{S} \times \Delta_{K} \to \mathcal{S}$ given by \eqref{eqn:posterior_update}. 
% (4) \textbf{Reward Function} $R: \mc{S} \times \Delta_{K} \to \mathbb{R}$ given by negative of the objective $v_{t}(\pi_{t}, \theta_{t}, \Sigma_{t})$.
The \emph{batched limit dynamic program}, $\model$, is precisely this MDP. Given a state $(\theta_{t}, \Sigma_{t})$ and potential sampling policies, the experimenter can use closed-form update equations to easily simulate approximate trajectories of how their 
beliefs will change throughout the experiment $(\theta_{t}, \Sigma_{t}) \overset{p_{t}}{\longrightarrow} (\theta_{t+1}, \Sigma_{t+1})\overset{p_{t+1}}{\longrightarrow} \cdots \overset{p_{T-1}}{\longrightarrow} (\theta_{T}, \Sigma_{T})$. Let $\pi_t$ be a policy for the $\model$, which maps from a belief state $(\theta_{t}, \Sigma_{t})$ to an action selection kernel $p_t$. The objective for the $\model$ can therefore be written as:
\[
\min_{\pi_0, \ldots, \pi_T} \E \left[ \sum_{t=0}^T c_t\bigl (\pi_t(\theta_{t}, \Sigma_{t}), \theta_{t}, \Sigma_{t}\bigr) \right].
\]




\vspace{30pt}

{\color{red}TODO}
The $\model$ involves the following process for the experimenter:
\begin{enumerate}
  \item \textbf{Modeling:} The experimenter specifies the model $f(x,a;\theta)$ and the associated 
  M-estimation procedure. They encode their objectives and constraints within the MDP ${\{v_{t}(\pi_{t}, \theta_{t}, \Sigma_{t})\}_{t=0}^{T}}$.
  \item \textbf{Planning via Simulation and Optimization:} At each epoch $t$, the experimenter starts 
  at a belief state $(\theta_{t}, \Sigma_{t})$. Then, they simulate various trajectories by choosing a 
  sequence of policies $(\pi_{t}, \pi_{t+1}, ..., \pi_{T})$ and simulating potential reward trajectories and 
  state transitions: 
  \[
    v(\pi_{t}, \theta_{t}, \Sigma_{t}) \overset{\pi_{t}}{\to} v(\pi_{t+1}, \theta_{t+1}, \Sigma_{t+1}) \overset{\pi_{t+1}}{\to} \dots \overset{\pi_{T-1}}{\to} v(\pi_{T}, \theta_{T}, \Sigma_{T})
  \]  
  If the objectives $v$ are differentiable functions, under common parametric models the objectives $v(\pi_{t}, \theta_{t}, \Sigma_{t})$ are 
  differentiable with respect to the sampling allocation $\pi_{t}$. Therefore, the experimenter can use gradient-based optimization methods 
  to easily solve for the optimal policy $\pi_{t}$. Then, $\pi_{t}$ is implemented and the experimenter updates their belief using real data. 
\end{enumerate}

\subsection{Empirical Results}
We highlight a policy we refer to as $\algofull$ ($\algo$), which uses
the model-predictive control (MPC) design principle to adaptively plan the 
sampling allocations. Whenever new samples are obtained, which could be from a large batch, 
the policy simulates trajectories from the $\model$ to solve for an optimal 
\emph{static} sequence of treatment allocations to use for the rest of experiment. 
By re-solving this sequence after every batch, the policy remains adaptive while working flexibly with batched feedback. 
The model-predictive control principle guarantees that regardless of how complicated
the inputted specifications, objectives, constraints, and non-stationarity patterns are,
the treatment allocations are guaranteed to have a lower Bayesian regret than static A/B testing.








% In particular, 
% The treatment allocation is the solution of an optimization routine, which means we can flexibly incorporate 
% user-specified objectives and constraints. It allows the experimenter to also incorporate predictions of context arrivals, 
% and by doing so it can ensure robustness against temporal non-stationarity (e.g. day-of-the-week, seasonality).
% The model-predictive control principle guarantees that regardless of how complicated
% the inputted specifications, objectives, constraints, and non-stationarity patterns are,
% the treatment allocations are guaranteed to have a lower Bayesian regret than static A/B testing.
% This is a practically useful robustness guarantee since static A/B testing
% is the universal baseline for treatment allocation in real-world experiments. It allows the policy to be safely deployed in diverse settings,
% including those which have not yet been studied in the multi-armed bandit literature.











%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:



% Experimentation is a core component of the deployment life-cycle of machine learning (ML) models in the real world, 
% particularly for large-scale Internet platforms. Adaptive experimentation offers a powerful methodology for 
% reducing operational costs and increasing statistical power by efficiently allocating sampling effort.  
% {\color{blue} Consider the following applications, motivated by real-world business use cases:
% \begin{itemize}
%   \item Meta example
%   \item A fashion retailer comparing multiple layouts for their landing page in anticipation of a holiday sale.
%   \item A ridesharing platform conducting discount experiments in different regions to optimize region-specific pricing.
% \end{itemize}

% Although superficially these examples may be modeled as instances of a multi-armed bandit problem,
% there are substational practical challenges unique to each setting that preclude a straightforward application
% of standard multi-armed bandit algorithms. These challenges include non-stationarity, constraints, personalization,
% multiple objectives, etc. While there are works dealing individually with each of these issues, 
% currently there is no single framework built to flexibly address all of these issues. Inflexibility of current approaches
% makes it difficult for practitioners to apply adaptive experimentation to their setting, which may involve bespoke considerations
% or even combinations of these challenges.

% partly because
% there is often a disconnect between the practical challenges of conducting modern experiments and the 
% problems that algorithmic researchers attempt to address. 
% }

% To elucidate a few examples: first, adaptive experimentation (bandit) algorithms are typically compared based 
% on their associated regret bounds, almost always in ideal settings that assume arm rewards are independently 
% and identically distributed (i.i.d.) over time. 
% {\color{blue}
% Yet, as in the example of the fashion retailer conducting
% an experiment during the holiday season, there can be significant non-stationarity in how users respond to treatments across time, 
% which can derail adaptive sampling policies \citep{QinRusso2023}}. 
% We conduct a rigorous empirical study across 241 unique settings exhibiting 
% natural non-stationarity based on experiments performed by ASOS.com, a global fashion retailer with 
% over 26 million active customers (as of 2024). Concerningly, we find that popular adaptive experimentation methods
% like Thompson Sampling, even when augmented with contextual information to explicitly account for non-stationary, 
% fail to outperform a simple uniform allocation policy (see Figure \ref{fig:main_plot}) {\color{blue} in more than 48\% of experiments}, 
% showing that theoretical regret bounds may not be indicative of practical performance.
% {\color{blue} Need to be careful, there are bandit papers dealing with non-stationarity.}

% Second, large-scale experiments are increasingly becoming more complicated due to the need to satisfy constraints 
% and optimize multiple objectives directly related to importance and impact on a business platform, usually 
% at the same time. {\color{blue} In the case of the ridesharing platform conducting regional discount experiments,
% often these experiments are conducted with a budget constraint for the total coupon amount across regions.}
% Other examples include requiring sufficient sample coverage for post-experiment 
% inference \citep{OfferWestortCoGr20, ZhangJaMu20}, requiring fairness \citep{chen20a}, and ensuring 
% safety \citep{amani19}. While there are bandit algorithms developed to handle each of these settings individually, 
% these methods are typically developed on a per-problem basis and require significant mathematical insight. There is 
% a lack of a general-purpose framework that allows practitioners to specify platform-specific constraints and 
% objectives in a flexible manner. 

% Third, experimentation is increasingly utilized to optimize policies that assign
% users personalized treatments, such as a slate of content in a social media context~\cite{}.
% Policy regret as an objective

% Finally, in contrast to algorithms designed to achieve strong guarantees as the number of reallocation epochs 
% grows to infinity, real-world experiments are universally conducted in \emph{large batches} with \emph{infrequent updates} to 
% the sampling policy \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. {\color{blue} Experimentation
% with large batches is often implemented deliberately as a way to reduce operational costs of experimentation, with
% the size of the batch typically determined by platform-specific usage (e.g. the batch consists of all users who
% arrive to the platform on a specific day or week).
% Large batches also emerge naturally if the treatment outcomes exhibit delayed feedback. 
% If outcomes can only be collected after a certain period of time,
% rather than waiting sequentially for each individual outcome to be recorded, 
% it is far more efficient to assign treatments to a batch of users in order to obtain a richer sample
% of outcomes at the end of the delay period. This introduces challenges into the mathematical analysis of adaptive experimentation 
% algorithms, which typically rely on martingale arguments that are better suited for algorithms that update frequently}. Much of the literature
% on batched bandit algorithms also require custom batch sizes, which is incompatible with current practices in which batches are determined
% exogenously by platform usage or delays.
% % However, as we will show later, rather than imposing a fundamental
% % algorithmic difficulty, in our proposed framework large batches actually improve our ability to model the information
% % gained by adaptive sampling policies.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
%   \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
%   \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
%   Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
%   and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
%   even under model misspecification, and across a wide range of learning rates.
%     \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
%     across 241 settings.
%     RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
%     Contextual TS do so in 95 and 125 instances respectively. 
%     In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
%     obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
%     The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
%     relative reward compared to Uniform when it underperforms Uniform.}
%   \label{fig:main_plot}
% \end{figure}

% {\color{blue}
% Rather than relying on bespoke algorithms, which are often derived via mathematical insight and cannot easily adapt
% to new settings, we develop a \emph{mathematical-programming} framework
% for adaptive experimental design, which tailors the sampling decisions to user-specified
% objectives, constraints, and non-stationarity patterns through optimization.
% Planning via optimization is the de-facto methodology
% for coordinating complex and economically significant decisions across a planning horizon, 
% while navigating multiple objectives and constraints,
% in widespread settings such as supply-chain optimization, electricity markets, scheduling, etc.
% Considering that modern experiments involve sampling decisions 
% }

% To address these issues, we introduce a modeling methodology called " " that allows experimenters to write down 
% dynamic programs that can flexibly incorporate a wide range of objectives, constraints, and models. 
% " " is based on the observation that batches, which are naturally used in real-world experiments, result in the 
% asymptotic normality of a wide class of estimators. By extending Bayesian statistics to classical m-estimation,
% we allow experimenters to update a tractable Bayesian model of their uncertainty. 
% In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
% combinatorial action spaces, " " dynamic programs can be approximately solved using computational tools. 

% In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
% the model-predictive control (MPC) design principle to adaptively plan the 
% sampling allocations: after observing new samples, re-solve for an optimal 
% \emph{non-adaptive} sampling policy to use for the rest of experiment. 
% By resolving after every batch, the policy remains adaptive while working flexibly with batched feedback. 
% Since the policy is the outcome of an optimization sub-routine, we can flexibly incorporate constraints.
% Finally, it allows the experimenter to incorporate predictions of context arrivals, ensuring robustness 
% against predictible non-stationarity (e.g. day-of-the-week, seasonality).

% As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
% empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

% ... 

% Finally, we release an accompanying software package " " that allows practitioners to easily implement 
% our policies and develop new ...  









% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:



% Experimentation is a core component of the deployment life-cycle of machine learning (ML) models in the real world, 
% particularly for large-scale Internet platforms. Adaptive experimentation offers a powerful methodology for 
% reducing operational costs and increasing statistical power by efficiently allocating sampling effort.  
% {\color{blue} Consider the following applications, motivated by real-world business use cases:
% \begin{itemize}
%   \item Meta example
%   \item A fashion retailer comparing multiple layouts for their landing page in anticipation of a holiday sale.
%   \item A ridesharing platform conducting discount experiments in different regions to optimize region-specific pricing.
% \end{itemize}

% Although superficially these examples may be modeled as instances of a multi-armed bandit problem,
% there are substational practical challenges unique to each setting that preclude a straightforward application
% of standard multi-armed bandit algorithms. These challenges include non-stationarity, constraints, personalization,
% multiple objectives, etc. While there are works dealing individually with each of these issues, 
% currently there is no single framework built to flexibly address all of these issues. Inflexibility of current approaches
% makes it difficult for practitioners to apply adaptive experimentation to their setting, which may involve bespoke considerations
% or even combinations of these challenges.

% partly because
% there is often a disconnect between the practical challenges of conducting modern experiments and the 
% problems that algorithmic researchers attempt to address. 
% }

% To elucidate a few examples: first, adaptive experimentation (bandit) algorithms are typically compared based 
% on their associated regret bounds, almost always in ideal settings that assume arm rewards are independently 
% and identically distributed (i.i.d.) over time. 
% {\color{blue}
% Yet, as in the example of the fashion retailer conducting
% an experiment during the holiday season, there can be significant non-stationarity in how users respond to treatments across time, 
% which can derail adaptive sampling policies \citep{QinRusso2023}}. 
% We conduct a rigorous empirical study across 241 unique settings exhibiting 
% natural non-stationarity based on experiments performed by ASOS.com, a global fashion retailer with 
% over 26 million active customers (as of 2024). Concerningly, we find that popular adaptive experimentation methods
% like Thompson Sampling, even when augmented with contextual information to explicitly account for non-stationary, 
% fail to outperform a simple uniform allocation policy (see Figure \ref{fig:main_plot}) {\color{blue} in more than 48\% of experiments}, 
% showing that theoretical regret bounds may not be indicative of practical performance.
% {\color{blue} Need to be careful, there are bandit papers dealing with non-stationarity.}

% Second, large-scale experiments are increasingly becoming more complicated due to the need to satisfy constraints 
% and optimize multiple objectives directly related to importance and impact on a business platform, usually 
% at the same time. {\color{blue} In the case of the ridesharing platform conducting regional discount experiments,
% often these experiments are conducted with a budget constraint for the total coupon amount across regions.}
% Other examples include requiring sufficient sample coverage for post-experiment 
% inference \citep{OfferWestortCoGr20, ZhangJaMu20}, requiring fairness \citep{chen20a}, and ensuring 
% safety \citep{amani19}. While there are bandit algorithms developed to handle each of these settings individually, 
% these methods are typically developed on a per-problem basis and require significant mathematical insight. There is 
% a lack of a general-purpose framework that allows practitioners to specify platform-specific constraints and 
% objectives in a flexible manner. 

% Third, experimentation is increasingly utilized to optimize policies that assign
% users personalized treatments, such as a slate of content in a social media context~\cite{}.
% Policy regret as an objective

% Finally, in contrast to algorithms designed to achieve strong guarantees as the number of reallocation epochs 
% grows to infinity, real-world experiments are universally conducted in \emph{large batches} with \emph{infrequent updates} to 
% the sampling policy \citep{BakshyEtAl18, OfferWestortCoGr20, JobjornssonScMuFr22}. {\color{blue} Experimentation
% with large batches is often implemented deliberately as a way to reduce operational costs of experimentation, with
% the size of the batch typically determined by platform-specific usage (e.g. the batch consists of all users who
% arrive to the platform on a specific day or week).
% Large batches also emerge naturally if the treatment outcomes exhibit delayed feedback. 
% If outcomes can only be collected after a certain period of time,
% rather than waiting sequentially for each individual outcome to be recorded, 
% it is far more efficient to assign treatments to a batch of users in order to obtain a richer sample
% of outcomes at the end of the delay period. This introduces challenges into the mathematical analysis of adaptive experimentation 
% algorithms, which typically rely on martingale arguments that are better suited for algorithms that update frequently}. Much of the literature
% on batched bandit algorithms also require custom batch sizes, which is incompatible with current practices in which batches are determined
% exogenously by platform usage or delays.
% % However, as we will show later, rather than imposing a fundamental
% % algorithmic difficulty, in our proposed framework large batches actually improve our ability to model the information
% % gained by adaptive sampling policies.

% \begin{figure}[t]
%   \centering
%   \includegraphics[width=1.1\textwidth]{fig/main_plots.png}
%   \caption{Benchmarking adaptive experimentation policies on 241 non-stationary settings from the ASOS.com dataset (with a batch size of $n_{t}=100,000$). 
%   \textbf{(Right)} Plot of best-arm identification performance with simple regret for contextual and non-contextual policies.
%   Our proposed policy $\algo$ (star points) is the only adaptive policy to obtain greater average reward
%   and choose the best arm more often compared to uniform sampling. It outperforms other adaptive algorithms
%   even under model misspecification, and across a wide range of learning rates.
%     \textbf{(Left)} Quantile plot of simple regret (normalized by simple regret of the uniform allocation)
%     across 241 settings.
%     RHO outperforms Uniform in 146 instances while Non-Contextual TS and 
%     Contextual TS do so in 95 and 125 instances respectively. 
%     In these instances, Non-Contextual and Contextual TS sometimes do much worse, 
%     obtaining a 24.8\% and 10.7\% decrease in average relative reward compared to uniform. 
%     The performance of RHO is relatively more robust, incurring only a 6.9\% decrease in 
%     relative reward compared to Uniform when it underperforms Uniform.}
%   \label{fig:main_plot}
% \end{figure}

% {\color{blue}
% Rather than relying on bespoke algorithms, which are often derived via mathematical insight and cannot easily adapt
% to new settings, we develop a \emph{mathematical-programming} framework
% for adaptive experimental design, which tailors the sampling decisions to user-specified
% objectives, constraints, and non-stationarity patterns through optimization.
% Planning via optimization is the de-facto methodology
% for coordinating complex and economically significant decisions across a planning horizon, 
% while navigating multiple objectives and constraints,
% in widespread settings such as supply-chain optimization, electricity markets, scheduling, etc.
% Considering that modern experiments involve sampling decisions 
% }

% To address these issues, we introduce a modeling methodology called " " that allows experimenters to write down 
% dynamic programs that can flexibly incorporate a wide range of objectives, constraints, and models. 
% " " is based on the observation that batches, which are naturally used in real-world experiments, result in the 
% asymptotic normality of a wide class of estimators. By extending Bayesian statistics to classical m-estimation,
% we allow experimenters to update a tractable Bayesian model of their uncertainty. 
% In contrast to intractable dynamic programs that attempt to model unit-level rewards resulting in 
% combinatorial action spaces, " " dynamic programs can be approximately solved using computational tools. 

% In particular, we highlight a policy we refer to as $\algofull$ ($\algo$), which uses
% the model-predictive control (MPC) design principle to adaptively plan the 
% sampling allocations: after observing new samples, re-solve for an optimal 
% \emph{non-adaptive} sampling policy to use for the rest of experiment. 
% By resolving after every batch, the policy remains adaptive while working flexibly with batched feedback. 
% Since the policy is the outcome of an optimization sub-routine, we can flexibly incorporate constraints.
% Finally, it allows the experimenter to incorporate predictions of context arrivals, ensuring robustness 
% against predictible non-stationarity (e.g. day-of-the-week, seasonality).

% As our focus is on experimentation settings most representative of naturally occurring practical challenges, we 
% empirically benchmark adaptive experimentation methods on instances based on real-world datasets. 

% ... 

% Finally, we release an accompanying software package " " that allows practitioners to easily implement 
% our policies and develop new ...  









% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:


==> proof-asymptotic.tex <==
\section{Proofs of large horizon results}
\label{section:proof-asymptotic}

\subsection{Proof of Theorem~\ref{theorem:asymptotic-rho}}
\label{section:proof-asymptotic-rho}

The proof of Theorem~\ref{theorem:asymptotic-rho} first relies on a
characterization of the gradient of the objective as $T - t \to \infty$.

\begin{proposition}
  \label{prop:grad-hess}
  Consider any fixed epoch $t$ and state $(\mu, \sigma)$.
  Let $\theta_{a} := \mu_a + \sigma_{a}Z_{a}$ be the random variable
  representing the posterior belief of the average reward for arm $a$,
  and let $\theta_{a}^{*} := \max_{a' \neq a} \theta_{a'}$.
  Suppose that as $T-t$ grows large, 
  the residual sample budget $\bar{b}_{t} = \sum_{s=t}^{T-1} b_{s}\to \infty$.
  Then gradient and Hessian of the planning objective $V^{\bar{\rho}}_{t}(\mu,\sigma)$
  with respect to the allocation $\bar{\rho}$ converge as follows:
    \begin{align*}
    \lim_{T \to \infty} \bar{b}_{t} \nabla V^{\bar{\rho}}_{t}(\mu,\sigma)
     &= \textup{diag} \left( \frac{s_{a}^{2}}{2\bar{\rho}_{a}^{2}}
     \E \left[\frac{1}{\sigma_{a}} \phi \left( \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right] \right) \\
     \lim_{T \to \infty} \bar{b}_{t} \nabla^{2} V^{\bar{\rho}}_{t}(\mu,\sigma)
     &= - \textup{diag} \left(\frac{s_{a}^{2}}{2\bar{\rho}_{a}^{3}}
     \E \left[\frac{1}{\sigma_{a}} \phi \left( \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right] \right)
    \end{align*}
  where $\phi(\cdot)$ is the standard normal density.
\end{proposition}

\begin{proof}
We characterize the asymptotic behavior of the gradient and hessian of
$V_{t}^{\bar{\rho}}(\mu,\sigma) =
\mathbb{E}_{t}\left[\max_{a}\mu_{T,a}\right]$ with respect to $\bar{\rho}$ as
the residual horizon $T-t$ grows large.  The residual horizon affects the
planning problem through the residual batch size $\bar{b}_{t}$, which is
assumed to converge to infinity as $T-t\to \infty$.  Rewrite the planning
objective $V_{t}^{\bar{\rho}}(\mu,\sigma)$ with a rescaled measurement
variance $s_{a}^{2}/\bar{b}_{t}$
\begin{align*}
  V_{t}^{\bar{\rho}}(\mu,\sigma) =\E_{t} \left[ \max_{a} \left\{ \mu_{t,a}
  + \sqrt{\frac{\sigma_{t, a}^4 \bar{\rho}_{a}}
  {s_a^2/\bar{b}_{t} + \sigma_{t, a}^2 \bar{\rho}_{a} }} Z_{t, a}  \right\} \right],
\end{align*}
It is sufficient to understand the behavior of
$V_{t}^{\bar{\rho}}(\mu,\sigma)$ as the measurement variance goes to zero.
For ease of notation we define $\alpha := 1/\bar{b}_{t}$, and consider
$\alpha$ as a scaling parameter of the measurement variance that converges to
zero.

Observe $V_{t}^{\bar{\rho}}(\mu,\sigma)$ can be expressed as the composition
$V_{t}^{\bar{\rho}}(\mu,\sigma)=g\left(\varphi\left(\bar{\rho},\sigma^{2},\alpha
    s^{2} \right)\right)$ where 
\[
\begin{aligned}
  g(v) &\defeq \E[\max_{a}\mu_{a}+v_{a}Z_{a}] \\
  \varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},s_{a}^{2})&\defeq\sigma_{a}\sqrt{\frac{\bar{\rho}_{a}\sigma_{a}^{2}}{s_{a}^{2}+\bar{\rho}_{a}\sigma_{a}^{2}}}
\end{aligned}
\]
and $\varphi, \sigma^{2}, s^{2}$ refer to the vectorized versions. The
function $g(v)$ describes the behavior of the max of Gaussian random variables
under standard deviations $v$, and $\varphi$ characterizes how the standard
deviation of the update changes with the sampling probabilities $\bar{\rho}$.

Through the chain rule, it is sufficient to characterize the gradient and
hessian of $g,\varphi$.  \citet{FrazierPo10} derived expressions for the
gradient and hessian of $g(v)$.
\begin{lemma}[{\citet{FrazierPo10}}]
  \label{lemma:frazier} Letting
  $W_{a}\defeq \max_{a'\neq a}\mu_{a'}+v_{a'}Z_{a'}$,
  \begin{align*}
    \frac{\partial}{\partial v_{a}}g(v)
    & = \mathbb{E}\left[Z_{a}\indic{a=\arg\max_{a'}\mu_{a'}+v_{a'}Z_{a'}}\right]
      = \mathbb{E}\left[\phi\left(\frac{W_{a}-\mu_{a}}{v_{a}}\right)\right] \\
    \frac{\partial^{2}}{\partial v_{a}^{2}}g(v)
    & = \mathbb{E}\left[\left(\frac{W_{a}-\mu_{a}}{v_{a}^{3}}\right)
      \phi\left(\frac{W_{a}-\mu_{a}}{v_{a}}\right)\right] \\
    \frac{\partial^{2}}{\partial v_{a}\partial v_{a'}}g(v)
    & = \mathbb{E}\left[-\left(\frac{W_{a}-\mu_{a}}{v_{a}}\right)
      \phi\left(\frac{W_{a}-\mu_{a}}{v_{a}}\right)Z_{a'}
      \indic{a'=\argmax_{\hat{a}\neq a}
      \mu_{\hat{a}}+v_{\hat{a}}Z_{\hat{a}}}\right]
  \end{align*}
\end{lemma}
\noindent The first and second derivatives of $\varphi$ are given by
\[ \frac{\partial}{\partial\bar{\rho}_{a}}\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},\alpha s_{a}^{2}) 
  = \frac{\alpha s_{a}^{2} \sigma_{a}^{2}}{2\bar{\rho}_{a}^{1/2}(\alpha s_{a}^{2} + \bar{\rho}_{a}\sigma_{a}^{2})^{3/2}},
  \qquad \frac{\partial^{2}}{\partial\bar{\rho}_{a}^{2}}\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},\alpha s_{a}^{2}) = -\frac{\sigma_{a}^{2}(\alpha^2 s_{a}^{4} + 4\bar{\rho}_{a} \alpha s_{a}^{2}\sigma_{a}^{2})}{4\bar{\rho}_{a}^{3/2}(\alpha s_{a}^{2} + \bar{\rho}_{a}\sigma_{a}^{2})^{5/2}}.
\]

We first study the behavior of $\varphi$ and its derivatives as
$\alpha\to0$
\[
\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},\alpha s_{a}^{2}) \to \sigma_{a},
\qquad \frac{\partial}{\partial\bar{\rho}_{a}}\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},\alpha s_{a}^{2})\sim\frac{\alpha s_{a}^{2}}{2\bar{\rho}_{a}^{2}\sigma_{a}},
\qquad \frac{\partial^{2}}{\partial\bar{\rho}_{a}^{2}}\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2}, \alpha s_{a}^{2})\sim-\frac{\alpha s_{a}^{2}}{\bar{\rho}_{a}^{3}\sigma_{a}}.
\]
To analyze $g(\varphi (\bar{\rho},\sigma^{2},\alpha s^{2}))$, recall that
$\theta_{a} = \mu_{a} + \sigma_{a}Z_{a}$ is the random variable representing
the posterior belief of the average reward of arm $a$.  For any realization of
$Z\sim N(0,I)$, we have
\[
  W_{a} = \max_{a'\neq a}\left\{ \mu_{a'}+\varphi_{a'}(\bar{\rho}_{a'},\sigma_{a'}^{2},\alpha s_{a'}^{2})Z_{a'} \right\} \to \theta_{a}^{*},
\]
so dominated convergence implies
\begin{align*}
  \lim_{\alpha \to 0}\frac{\partial}{\partial v_{a}}
  g(\varphi(\bar{\rho}, \sigma^{2}, \alpha s^2))
  & = \E \left[
    \phi\left(\frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}}\right)
    \right] \\
  \lim_{\alpha \to 0}
  \frac{\partial^{2}}{\partial v_{a}^{2}}
  g(\varphi(\bar{\rho}, \sigma^{2}, \alpha s^2))
  & = \E \left[
    \frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}^{3}} 
    \cdot \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)
    \right] \\
  \lim_{\alpha \to 0}
  \frac{\partial^{2}}{\partial v_{a}\partial v_{a'}}
  g(\varphi(\bar{\rho}, \sigma^{2}, \alpha s^2))
  & = \E \left[
    - \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \cdot
    \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)
    Z_{a'} \indic{a'=\arg\max_{\hat{a}\neq a}\theta_{\hat{a}}}
    \right]
\end{align*}


By the chain rule,
$\nabla_{\bar{\rho}} V_{t}^{\bar{\rho}}(\mu, \sigma) =
\nabla_{v}g(\varphi(\mu, \sigma^{2}, \alpha s^{2})) \nabla_{\bar{\rho}}
\varphi (\bar{\rho},\sigma^{2},\alpha s^{2}) $ where the Jacobian
$\nabla_{\bar{\rho}} \varphi$ is
\[
  \nabla_{\bar{\rho}} \varphi (\bar{\rho},\sigma^{2},\alpha s^{2}) := \text{diag} \left( \frac{\partial}{\partial\bar{\rho}_{a}}\varphi_{a}(\bar{\rho}_{a},\sigma_{a}^{2},\alpha s_{a}^{2}) \right).
\]
Rescaling the planning objective $V_{t}^{\bar{\rho}}$ by $1/\alpha$, we obtain
the following limit
\[
  \lim_{\alpha \to \infty}  \alpha^{-1}
  \nabla_{\bar{\rho}} V^{\bar{\rho}}_{t}(\mu, \sigma)
  = \frac{s_{a}^{2}}{2\bar{\rho}_{a}^{2}\sigma_{a}}
  \E \left[\phi\left(\frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}}\right)\right]
\]
As for the Hessian, the chain rule implies
\begin{align*}
  \frac{\partial^{2} V_{t}^{\bar{\rho}}}{\partial \bar{\rho}_{a}\partial \bar{\rho}_{a'}}
  &= \sum_{i} \frac{\partial g(\varphi(\bar{\rho}))}{\partial v_{i}}
    \frac{\partial^{2} \varphi_{i}}{\partial \bar{\rho}_{a} \partial \bar{\rho}_{a'}}
    + \sum_{i,j} \frac{\partial g(\varphi(\bar{\rho})) }{\partial v_{i}\partial v_{j}} 
    \frac{\partial \varphi_{i}}{\partial \bar{\rho}_{a}}
    \frac{\partial \varphi_{j}}{\partial \bar{\rho}_{a'}} \\
  &= \frac{\partial g(\varphi(\bar{\rho}))}{\partial v_{a}}
    \frac{\partial^{2} \varphi_{a}}{\partial \bar{\rho}_{a}^{2}} 1\{ a = a' \}
    + \frac{\partial g(\varphi(\bar{\rho})) }{\partial v_{a}\partial v_{a'}} 
    \frac{\partial \varphi_{a}}{\partial \bar{\rho}_{a}}
    \frac{\partial \varphi_{a'}}{\partial \bar{\rho}_{a'}},
\end{align*}
where we suppress the dependence of $\varphi$ on other arguments for
succinctness. Rewriting this using
$\nabla_{\bar{\rho}}^{2}\varphi := \diag \left( \frac{\partial^{2}
    \varphi_{a}}{\partial \bar{\rho}_{a}^{2}} \right)$, we get
\[  
  \nabla_{\bar{\rho}}^{2}V^{\bar{\rho}}_{t}(\mu,\sigma)
 = \text{diag}(\nabla_{v} g(\varphi(\bar{\rho}))) \nabla_{\bar{\rho}}^{2}\varphi + \nabla_{\bar{\rho}}\varphi \nabla_{v}^{2}g(\varphi(\bar{\rho}))\nabla_{\bar{\rho}}\varphi.
\]
Collecting the above results, we have
\begin{align*}
  \lim_{\alpha \to 0} \alpha^{-1} 
  \text{diag}(\nabla_{v} g(\varphi(\bar{\rho}))) \nabla_{\bar{\rho}}^{2}\varphi
  &= -\text{diag} \left( \frac{ s_{a}^{2}}{\bar{\rho}_{a}^{3}\sigma_{a}} 
      \E \left[\phi\left(\frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}}\right)\right] \right)\\
  \lim_{\alpha \to 0} \alpha^{-1}  \nabla_{\bar{\rho}}\varphi \nabla_{v}^{2}g(\varphi(\bar{\rho}))\nabla_{\bar{\rho}}\varphi
  &= \lim_{\alpha \to 0} \alpha^{-1}
  \text{diag} \left(  \frac{\alpha s_{a}^{2}}{2 \bar{\rho_{a}}^{2} \sigma_{a}} \right)
  \nabla_{v}^{2} g(\varphi(\bar{\rho}))
  \text{diag} \left( \frac{ \alpha s_{a}^{2}}{2 \bar{\rho_{a}}^{2} \sigma_{a}} \right)
  = 0,
\end{align*}
which gives the final result.

\end{proof}

This leads us to the following corollary, which uses the characterization of the Hessian to show that 
the objective becomes strongly concave as $T-t \to \infty$.

\begin{corollary}
  \label{cor:strong-concavity}
  Let $\Delta_K^\epsilon = \Delta_K \cap \{p: p \ge \epsilon\}$ be the
  truncated simplex. For a fixed epoch $t$ and state $(\mu, \sigma)$, there
  exists $T_0(\epsilon) > 0$ such that $\forall T - t > T_0$,
  $\bar{\rho} \mapsto \bar{b}_{t}V^{\bar{\rho}}_{t}(\mu,\sigma)$ is strongly
  concave on $\Delta_K^\epsilon$.
\end{corollary}

% \subsection{Proof of Corollary~\ref{cor:strong-concavity}}
% \label{section:proof-strong-concavity}

\begin{proof}
In the proof of Proposition~\ref{prop:grad-hess}, we showed that as the
(scaled) measurement variance $\alpha s_{a}^{2}$ converges to zero, the
Hessian $\alpha^{-1} \nabla_{\bar{\rho}}^{2}V^{\bar{\rho}}_{t}(\mu,\sigma)$
can be expressed as a negative-definite diagonal matrix plus a matrix that
converges to zero. As long as the sampling probabilities are bounded below, the
convergence is uniform. We have the following bound for the largest eigenvalue
of the Hessian
\begin{align*}
  \lambda_{\max}\left(
  \nabla_{\bar{\rho}}^{2} \alpha^{-1}
  V^{\bar{\rho}}_{t}(\mu,\sigma) \right)
  & \leq \lambda_{\max}\left( \alpha^{-1}
    \text{diag}(\nabla_{v} g(\varphi(\bar{\rho})))
    \nabla_{\bar{\rho}}^{2}\varphi \right)
    +\lambda_{\max}\left(\alpha^{-1} \nabla_{\bar{\rho}}\varphi
    \nabla_{v}^{2}g(\varphi(\bar{\rho}))\nabla_{\bar{\rho}}\varphi
    \right) \\
  & \leq -\min_{a} \frac{s_{a}^{2}}{2\sigma_{a}\epsilon^3}
    \E \left[\phi\left(\frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}}\right)\right]
    + \alpha C/\epsilon^{4},
\end{align*}
where $C$ is a constant that depends only on $\mu,\sigma,s$. So as
$\alpha \to 0$, the Hessian will be negative-definite for all
$\bar{\rho}\in \Delta_{K}^{\epsilon}$. Thus, for a large enough residual batch
size $\bar{b}_{t}$ the planning objective will be strongly concave on the
truncated simplex $\Delta_{K}^{\epsilon}$ for some threshold $\epsilon$.
\end{proof}

% \hn{I think the final bound be something like
% $-\min_{a} \frac{s_{a}^{2}}{\epsilon^3 \sigma_{a}}
%     \E \left[\phi\left(\frac{\theta_{a}^{*} - \mu_{a}}{\sigma_{a}}\right)\right]
%     + \alpha C/\epsilon^{4}$?}

% \subsection{Proof of Proposition~\ref{prop:dts}}
% \label{section:proof-dts}

% By assumption, there exists some threshold $\epsilon > 0$ so that
% for $T-t$ large enough, the solution to $\max_{\rho\in\Delta_{K}^{\epsilon}} V^{\bar{\rho}}_{t}(\mu,\sigma)$
% is unique and the solution is in the interior of $\Delta_{K}^{\epsilon}$.
% We require this assumption as we prove convergence of the solutions through the
% KKT conditions, but we only obtain strong concavity, which guarantees uniqueness
% of solutions, on the truncated simplex
% $\Delta_{K}^{\epsilon}$ rather than the entire simplex. 
% However, this is not a strong assumption,
% as we are free to choose the threshold $\epsilon$.
% Although there are other techniques for proving the convergence of maxima
% without this assumption
% (e.g. Berge's Maximum Principle), a technical difficulty is that while
% the gradient and hessian of the rescaled objective $\alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma)$
% have well-defined limits, the function itself blows up as $\alpha \to 0$.

Finally, by strong concavity, the KKT conditions of the planning problem have a unique solution.
By the implicit function theorem, we can characterize the limit of this solution.

\begin{proposition}
  \label{prop:dts}
  Consider a fixed epoch $t$ and state $(\mu, \sigma)$. Suppose there exists
  $T_1$ such that for $\forall T - t > T_1$, the $\algo$ allocation satisfies
  $\rho_{t,a}(\mu,\sigma) > \epsilon$. Then as $T-t \to \infty$,
  \begin{equation*}
    \rho_{t,a}(\mu,\sigma) \to \pi_{a}^{\textup{DTS}}(\mu, \sigma),~\mbox{where}~
    \pi^{\rm DTS}_a(\mu, \sigma) \propto s_a \left[ \frac{\partial}{\partial
        \mu_a}\pi_{a}^{\textup{TS}}(\mu,\sigma) \right]^{1/2}
  \end{equation*}
  %if $\pi^{\rm DTS}_a (\mu_t,\sigma_t) > \epsilon$.
\end{proposition}

\begin{proof}
As in the proof of Proposition~\ref{prop:grad-hess}, we let
$\alpha = \bar{b}_{t}^{-1}$. Let $\alpha_{0}$ to be the threshold such that
for $\alpha < \alpha_{0}$ the objective is strongly concave (such a threshold
exists from Corollary~\ref{cor:strong-concavity}), and let
$\alpha_{1} < \alpha_{0}$ to be the threshold such that for
$\alpha < \alpha_{1}$ the unique solution is in the interior of
$\Delta_{K}^{\epsilon}$ (such a threshold exists by hypothesis).

For $\alpha$ small enough, the (scaled) KKT conditions give
\begin{equation}
  \label{eqn:opt_foc}
  \alpha^{-1} \nabla_{\bar{\rho}} V^{\bar{\rho}}_{t}(\mu,\sigma)
  - \lambda \onevec = 0, \quad \onevec^\top \rho_t = 1,
\end{equation}
where $\lambda$ is the optimal dual variable for the equality constraint.  The
Jacobian of this equation with respect to $(\bar{\rho}, \lambda)$ is the
following block matrix
\[
\begin{bmatrix}
  \nabla^{2}_{\bar{\rho}} \alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma) & -\onevec\\
  \onevec^{\top} & 0
\end{bmatrix}
\]
Since $\alpha < \alpha_{0}$, the Hessian of
$\alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma)$ is negative definite and
invertible in a neighborhood of $\alpha = 0$.  The Jacobian is also invertible
since the Schur complement
\begin{equation*}
  0 - \onevec^\top \alpha^{-1} \nabla^{2}_{\bar{\rho}}\E\left[\max_{a}\mu_{T,a}\right] (-\onevec) < 0
\end{equation*}
is invertible.  Moreover,
$\alpha^{-1} \nabla_{\bar{\rho}} V^{\bar{\rho}}_{t}(\mu,\sigma)$ is
continuously differentiable in $\alpha$ at $\alpha = 0$.  So by the Implicit
Function Theorem, there exists a $\alpha_2$ such that for all
$\alpha < \alpha_2$, the solution satisfying the KKT
conditions~\eqref{eqn:opt_foc}, $\bar{\rho}(\alpha)$ and $\lambda(\alpha))$,
is continuous in $\alpha$.  Thus, as $\alpha \to 0$, the unique maximizer of
$\alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma)$ converges to $\bar{\rho}\opt$
satisfying the limiting version of the KKT conditions~\eqref{eqn:opt_foc}.
Using the explicit expression for
$\alpha^{-1} \nabla_{\bar{\rho}} V^{\bar{\rho}}_{t}(\mu,\sigma)$ obtained in
Proposition~\ref{prop:grad-hess}, we conclude
\begin{equation}
  \label{eqn:kkt_dts}
  \bar{\rho}_{a}\opt \propto s_{a} \E \left[\frac{1}{\sigma_{a}}
    \phi \left( \frac{\theta_{a}\opt-\mu_{a}}{\sigma_{a}} \right)
  \right]^{1/2}
\end{equation}



% Using the expression for the gradient in the proof of
% Proposition~\ref{prop:grad-hess}, we have that the following expression for
% the KKT conditions of the rescaled objective
% $\alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma)$ for $\alpha < \alpha_{1}$.  We can
% omit the inequality constraints $\bar{\rho} > \epsilon$ as by assumption at
% the solution the inequality constraints do not bind:
% At $\alpha = 0$, using the limit of $\nabla_{\bar{\rho}} \alpha^{-1}V^{\bar{\rho}}_{t}(\mu,\sigma)$
% obtained in Proposition~\ref{prop:grad-hess}, we have that the solution to the KKT conditions is:
% \begin{equation} \label{eqn:kkt_dts}
%   \bar{\rho}_{a}^{*} \propto s_{a} \E \left[\frac{1}{\sigma_{a}} \phi \left( \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right]^{1/2},
%   \quad \lambda^{*} = \sum_{a} 2\bar{\rho}_{a}^{*}
% \end{equation}



To show the equivalence with the partial derivatives of the Thompson sampling probabilities, observe
\begin{align*}
  \pi_{a}^{\text{TS}}(\mu,\sigma)
  & =\mathbb{P}(\theta_{a}>\theta_{a}^{*})
    =\mathbb{P}\left(Z_{a}>\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right) \\
  & = \E\left[\mathbb{P}\left(
    Z_{a}>\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}
    \mid \theta_{a}^{*} \right) \right] 
   = \E\left[1-\Phi\left(
    \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right],
\end{align*}
where the final equality is a result of the independence prior and posterior
distributions across the treatment arms. Interchanging the derivative
and expectation, 
\[ \frac{\partial}{\partial\mu_{a}}
  \pi_{a}^{\text{TS}}(\mu,\sigma)
  = \frac{\partial}{\partial\mu_{a}}
  \E\left[
    1-\Phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)
  \right]
  = \E\left[\frac{1}{\sigma_{a}}
    \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right].
\]
\end{proof}

\subsection{More details on Density Thompson Sampling}
\label{section:proof-log-dts}

Similar to TS, DTS samples from the posterior distribution; while TS
asymptotically assigns all sampling effort to the best arm, DTS does not
oversample the best arm, as it is based on the gap between the second best
arm. Concretely, the relative sampling proportions
$\pi^{\text{DTS}}_{a}/\pi^{\text{DTS}}_{a'}$ can be expressed as ratios of the
`index'
$\E \left[\frac{1}{\sigma_{a}} \phi \left(
    \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right]^{1/2}$; the
higher the index, the more sampling effort allocated to that arm during the
epoch.  This index decreases at an exponential rate for \emph{all} arms as the
experiment progresses and the posterior uncertainty shrinks
$\sigma_{a} \to 0$.  
\begin{proposition}
  \label{prop:log-dts}
  Consider a fixed state $(\mu, \sigma)$ and suppose arms are sorted in decreasing order of their means $\mu_{1} > \mu_{2} > \ldots > \mu_{K}$.
  Then we have that:
  \[
    \begin{cases}
      -\frac{(\mu_{1}-\mu_{2})^{2}}{2(\sigma_{1}^{2}+\sigma_{2}^{2})}
      & ~~\mbox{top two arms}~~a\in{1,2} \\
      -\frac{(\mu_{1}-\mu_{a})^{2}}{2\sigma_{a}^{2}}
      & ~~\mbox{otherwise} \\
    \end{cases}
  \lesssim \log \E \left[\frac{1}{\sigma_{a}} \phi \left( \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right]
  \lesssim -\min_{a'\neq a}\frac{(\mu_{a'}-\mu_{a})^{2}}{2(\sigma_{a}^{2}+\sigma_{a'}^{2})}
  \]
  where $\lesssim$ contains additive terms that are logarithmic in $\min_{a} \sigma_{a}$.
  % For the remaining arms:
  % \[
  % -\frac{(\mu_{1}-\mu_{a})^{2}}{2(\sigma_{a}^{2})}
  % \leq \log \E \left[\frac{1}{\sigma_{a}} \phi \left( \frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}} \right) \right]
  % \leq -\min_{a'\neq a}-\frac{(\mu_{a'}-\mu_{a})^{2}}{2(\sigma_{a}^{2}+\sigma_{a'}^{2})}
  % \]
\end{proposition}
%\noindent See Section~\ref{section:proof-log-dts} for a proof. 
If an arm is excessively under-sampled, its index will eventually be larger than others and
so sampling effort will be spread out across arms rather than concentrating on
the best one.  This makes DTS better suited for best-arm identification and
closer to Top-Two Thompson Sampling~\citep{Russo20}.

\begin{proof}
Suppose that the arms are sorted so that $\mu_{1}>...>\mu_{K}$. Since
$\theta_{a}^{*}$ is the max of independent random variables, $\mathbb{P}(\theta_{a}^{*}\leq x)=\prod_{a'\neq a}\mathbb{P}(\theta_{a'}\leq x)=\prod_{a'\neq a}\Phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)$.
This means that the density of $\theta_{a}^{*}$ , denoted as $f_{a}^{*}(x)$,
can be expressed as (by the Leibniz product rule)
\begin{align*}
  f_{a}^{*}(x)
  & =\frac{d}{dx}\prod_{a'\neq a}\Phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)\\
  & =\sum_{a'\neq a}
    \left[\frac{d}{dx}\Phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)\right]
    \prod_{\hat{a}\notin\{a,a'\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)\\
  & =\sum_{a'\neq a}\left[\frac{1}{\sigma_{a'}}
    \phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)\right]
    \prod_{\hat{a}\notin\{a,a'\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right).
\end{align*}
Thus, we can write the expectation as
\begin{align*}
  \mathbb{E}\left[\frac{1}{\sigma_{a}}\phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  & =\int_{-\infty}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)f_{a}^{*}(x)dx\\
  & =\int_{-\infty}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)\sum_{a'\neq a}
    \left[\frac{1}{\sigma_{a'}}
    \phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)\prod_{\hat{a}\notin\{a,a'\}}
    \Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)\right]dx\\
  & =\sum_{a'\neq a}\int_{-\infty}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{a'}}\phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)
    \prod_{\hat{a}\notin\{a,a'\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx.
\end{align*}

For any arm $a$, we can obtain an upper bound for each term in the
sum by bounding $\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)\leq1$
and directly integrating
\begin{align*}
  & \int_{-\infty}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{a'}}\phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)
    \prod_{\hat{a}\notin\{a,a'\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx\\
  & \leq\int_{-\infty}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{a'}}\phi\left(\frac{x-\mu_{a'}}{\sigma_{a'}}\right)dx\\
  & =\frac{1}{\sqrt{2\pi(\sigma_{a'}^{2}+\sigma_{a}^{2})}}
    e^{-\frac{(\mu_{a'}-\mu_{a})^{2}}{2(\sigma_{a'}^{2}+\sigma_{a}^{2})}}.
\end{align*}
Finally, taking a max and summing up the terms gives
\[
  \mathbb{E}\left[\frac{1}{\sigma_{a}}
    \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  \leq(K-1)\max_{a'\neq a}\frac{1}{\sqrt{2\pi(\sigma_{a'}^{2}+\sigma_{a}^{2})}}
  e^{-\frac{(\mu_{a'}-\mu_{a})^{2}}{2(\sigma_{a'}^{2}+\sigma_{a}^{2})}}
\]

To get the lower bound, it suffices to lower bound a single $a'$ term in the
sum, since all terms are positive. We select the term involving $a'=1$ ($a'=2$
if $a=1$). Since the integrand is positive, we obtain a further lower bound by
truncating the integration from $\mu_{1}$ to $\infty$
\begin{align*}
  \mathbb{E}\left[\frac{1}{\sigma_{a}}\phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  & \geq\int_{-\infty}^{\infty}
    \frac{1}{\sigma_{a}}\phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)
    \prod_{\hat{a}\notin\{a,1\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx \\
  & \geq\int_{\mu_{1}}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)
    \prod_{\hat{a}\notin\{a,1\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx.
\end{align*}
On the domain of integration, $x\geq\mu_{1}$, so
$\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)\geq\frac{1}{2}$ for
all $\hat{a}\notin\{a,1\}$. Conclude
\begin{align*}
  & \int_{\mu_{1}}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)
    \prod_{\hat{a}\notin\{a,1\}}\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx\\
  & \geq\left(\frac{1}{2}\right)^{K-2}
    \int_{\mu_{1}}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)dx.
\end{align*}
Evaluating the integral explicitly gives
\begin{align*}
   \int_{\mu_{1}}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)dx
  = \frac{e^{-\frac{(\mu_{a}-\mu_{1})^{2}}{2(\sigma_{a}^{2}+\sigma_{1}^{2})}}}{\sqrt{2\pi (\sigma_{a}^{2}+ \sigma_{1}^{2})}}
    \bar{\Phi} \left( \frac{\sigma_{1}}{\sigma_{a}}\frac{\mu_{1} - \mu_{a}}{\sqrt{\sigma_{a}^{2}+ \sigma_{1}^{2}}} \right)
  % & =\frac{1}{\sigma_{a}\sigma_{1}}
  %   e^{-\frac{(\mu_{a}-\mu_{1})^{2}}{2(\sigma_{a}^{2}+\sigma_{1}^{2})}}
  %   \int_{\mu_{1}}^{\infty}e^{-\frac{1}{2}\left(\sigma_{1}^{-2}+\sigma_{a}^{-2}\right)
  %   \left(x-\frac{\sigma_{1}^{-2}\mu_{1}+\sigma_{a}^{-2}\mu_{a}}{\sigma_{1}^{-2}+\sigma_{a}^{-2}}
  %   \right)^{2}}dx\\
  % & =\frac{1}{\sigma_{a}\sigma_{1}}
  %   e^{-\frac{(\mu_{a}-\mu_{1})^{2}}{2(\sigma_{a}^{2}+\sigma_{1}^{2})}}
  %   \sqrt{2\pi(\sigma_{1}^{-2}+\sigma_{a}^{-2})^{-1}}
  %   \bar{\Phi}\left(\frac{(\mu_{1}-\mu_{a})}
  %   {\sigma_{a}^{2}\sqrt{\sigma_{1}^{-2}+\sigma_{a}^{-2}}}\right).
\end{align*}
Using the Gaussian tail bound $\bar{\Phi}(x)\geq\frac{\phi(x)}{2x}$ for
$x > 0$, 
\begin{align*}
  \mathbb{E}\left[\frac{1}{\sigma_{a}}
  \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  & \geq\left(\frac{1}{2}\right)^{K-2}
    \int_{\mu_{1}}^{\infty}\frac{1}{\sigma_{a}}
    \phi\left(\frac{x-\mu_{a}}{\sigma_{a}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)dx\\
  & \geq\frac{1}{\sqrt{2\pi(\sigma_{a}^{2}+\sigma_{1}^{2})}}
    e^{-\frac{(\mu_{a}-\mu_{1})^{2}}{2(\sigma_{a}^{2}+\sigma_{1}^{2})}}
    \frac{1}{2\left(\frac{\sigma_{1}}{\sigma_{a}}\frac{(\mu_{1}-\mu_{a})}{\sqrt{\sigma_{1}^{2}+\sigma_{a}^{2}}}\right)}
    e^{-\frac{(\mu_{1}-\mu_{a})^{2}}{2\sigma_{a}^{4}(\sigma_{1}^{-2}+\sigma_{a}^{-2})}}\\
  & =\frac{\sigma_{a}}{2\sigma_{1}\sqrt{2\pi}(\mu_{1}-\mu_{a})}
    e^{-\frac{1}{2}\frac{(\mu_{a}-\mu_{1})^{2}}{\sigma_{a}^{2}}}.
\end{align*}

We can get tighter lower bounds for the top two arms $a\in\{1,2\}$.  As in the
above lower bound, we focus on lower bounding the term corresponding with
$a'=1$ if $a=2$ or $a'=2$ if $a=1$ (for both we obtain the same lower bound).
But instead of integrating from $\mu_{1}$, we integrate from $\mu_{2}$.  For
illustration, we focus on $a=2$
\begin{align*}
  \mathbb{E}\left[\frac{1}{\sigma_{2}}
  \phi\left(\frac{\theta_{2}^{*}-\mu_{2}}{\sigma_{2}}\right)\right]
  & \geq\int_{-\infty}^{\infty}\frac{1}{\sigma_{2}}
    \phi\left(\frac{x-\mu_{2}}{\sigma_{2}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)
    \prod_{\hat{a}\notin\{a,1\}}
    \Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx\\
  & \geq\int_{\mu_{2}}^{\infty}\frac{1}{\sigma_{2}}
    \phi\left(\frac{x-\mu_{2}}{\sigma_{2}}\right)
    \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)
    \prod_{\hat{a}\notin\{a,1\}}
    \Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)dx.
\end{align*}
On this range, we have $x\geq\mu_{2}$. This implies that for every
$\hat{a}\neq\{1,2\}$, $x-\mu_{\hat{a}}\geq\mu_{2}-\mu_{\hat{a}}\geq0$. In
turn, this means
$\Phi\left(\frac{x-\mu_{\hat{a}}}{\sigma_{\hat{a}}}\right)\geq\frac{1}{2}$ as
we had before
\[
  \mathbb{E}\left[\frac{1}{\sigma_{a}}
    \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  \geq\left(\frac{1}{2}\right)^{K-2}
  \int_{\mu_{2}}^{\infty}\frac{1}{\sigma_{2}}
  \phi\left(\frac{x-\mu_{2}}{\sigma_{2}}\right)
  \frac{1}{\sigma_{1}}\phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)dx
\]
For $a=2$, we can evaluate this integral explicitly
\begin{align*}
  & \int_{\mu_{2}}^{\infty}\frac{1}{\sigma_{2}}
    \phi\left(\frac{x-\mu_{2}}{\sigma_{2}}\right)\frac{1}{\sigma_{1}}
    \phi\left(\frac{x-\mu_{1}}{\sigma_{1}}\right)dx\\
  & =\frac{1}{2\sqrt{2\pi(\sigma_{1}^{2}+\sigma_{2}^{2})}}
    e^{-\frac{(\mu_{1}-\mu_{2})^{2}}{2(\sigma_{1}^{2}+\sigma_{2}^{2})}}
    \left(1+\text{erf}\left(\frac{(\mu_{1}-\mu_{2})\sigma_{2}}
    {\sqrt{2}\sigma_{1}\sqrt{\sigma_{1}^{2}+\sigma_{2}^{2}}}
    \right)\right).
\end{align*}
Note that for positive values of the error function it is bounded below by zero. This gives 
\[
  \mathbb{E}\left[\frac{1}{\sigma_{a}}
    \phi\left(\frac{\theta_{a}^{*}-\mu_{a}}{\sigma_{a}}\right)\right]
  \geq\left(\frac{1}{2}\right)^{K-2}
  \frac{1}{2\sqrt{2\pi(\sigma_{1}^{2}+\sigma_{2}^{2})}}
  e^{-\frac{(\mu_{1}-\mu_{2})^{2}}{2(\sigma_{1}^{2}+\sigma_{2}^{2})}}.
\]
Repeating these steps for $a=1$ (taking $a'=2$) results in the same lower
bound.
\end{proof}


%\subsection{Proof of Theorem~\ref{theorem:dts-asymptotic}}
%\label{section:proof-dts-asymptotic}
%
%We consider the improper prior setting, in which the experimenter begins with a flat prior $\mu_{a}=0, \sigma_{a}=\infty$. 
%Recall that the Density Thompson Sampling at state $(\mu_{t},\sigma_{t})$ samples arms with probabilities:
%\[
%\pi_{a}^{\text{DTS}}(\mu_{t},\sigma_{t})=
%\frac{s_{a}\left(\E \left[\frac{1}{\sigma_{t,a}}\phi\left(\frac{\theta_{t,a}^{*}-\mu_{t,a}}{\sigma_{t,a}}\right)\right]\right)^{1/2}}
%{\sum_{b}s_{b}\left(\E\left[\frac{1}{\sigma_{t,b}}\phi\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{\sigma_{t,b}}\right)\right]\right)^{1/2}}
%\]
%where $\theta_{t,a}^{*}=\max_{a'\neq a}\mu_{'t,a}+\sigma_{t,a'}Z_{a'}$.
%As a shorthand, let $\pi_{t,a} := \pi^{\text{DTS}}(\mu_{t}, \sigma_{t})$, 
%and let $\Psi_{t,a}=\sum_{s=1}^{t}\pi_{s,a}$ be the total sampling effort allocated to arm $a$ by time $t$.
%
%By the Gumbel-max trick, the sampling policy is equivalent to:
%\[
%\pi_{a}^{\text{DTS}}(\mu_{t},\sigma_{t})=\mathbb{P}\left(a=\arg\max_{b}\left\{ \log s_{b}\left(\mathbb{E}\left[\frac{1}{\sigma_{t,b}}\phi\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{\sigma_{t,b}}\right)\right]\right)^{1/2}+\xi_{b}\right\} \right)
%\]
%where $\xi_{b}$ are independent $Gumbel(0,1)$ random variables. 
%Now, we consider the modified DTS policy that randomly draws an arm from $\pi^{\text{DTS}}$ and assigns all sampling effort
%to that arm.
%\[
%I_{a}^{\text{DTS}}(\mu,\sigma)=1\left\{ a=\arg\max_{b}\left\{ \log s_{b}\left(\mathbb{E}\left[\frac{1}{\sigma_{t,b}}\phi\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{\sigma_{t,b}}\right)\right]\right)^{1/2}+\xi_{b}\right\} \right\}.
%\]
%As a shorthand let $I_{t,a} := I_{a}^{\text{DTS}}(\mu_{t}, \sigma_{t})$, 
%and we denote $N_{t,a}=\sum_{s=1}^{t}I_{s,a}$ as the realized total sampling effort to arm $a$ by time $t$
%under this alternative policy. Under this policy, we have by Bayes rule:
%\[
%\mu_{t,a}=\frac{1}{N_{t,a}}\sum_{s=1}^{t}I_{s,a}X_{s,a},\quad\sigma_{t,a}^{2}=\frac{s_{a}^{2}}{N_{t,a}}
%\]
%where $X_{s,a} \sim N(h_{a}, s_{a}^{2})$.
%
%We use a key result from~\citet{Russo20}, which establishes appropriate law of large numbers for martingale sums.
%Crucially, it implies that  $N_{t,a}$ and $\Psi_{t,a}$ will be close together as long as $\Psi_{t,a}\to\infty$. 
%For concreteness, let $\mathcal{F}_{t} = \sigma(\mu_{t}, \sigma_{t}, I_{t-1}, \ldots, \mu_{0}, \sigma_{0})$
%denote the filtration up to $t$.
%
%\begin{lemma}[\citet{Russo20}]
%  \label{lemma:mrtngle-conv}
%Let $Y_{t}$ be an iid sequence of real-valued random variables with finite variance 
%and let $\{X_{t}\}$ be a sequence of binary random variables with 
%$\E[X_{t}]=Z_{t}$. 
%If conditioning on the filtration $\mathcal{F}_{t-1}$, each $Y_{t}$ is independent from $X_{t}$, then with probability 1:
%\[
%  \begin{aligned}
%\lim_{t\to\infty}\sum_{s=1}^{t}Z_{s}	&=\infty\implies\lim_{t\to\infty}\frac{\sum_{s=1}^{t}X_{s}Y_{s}}{\sum_{s=1}^{t}Z_{s}}=\mathbb{E}[Y_{1}] \\
%\lim_{t\to\infty}\sum_{s=1}^{t}Z_{s}	&<\infty\implies\sup_{t\in\mathbb{N}}\left|\sum_{s=1}^{t}X_{s}Y_{s}\right|<\infty
%  \end{aligned}
%\]
%\end{lemma}
%
%Notably this implies that:
%\[
%  \begin{aligned}
%  \lim_{t\to \infty} \Psi_{t,a} = \infty &\implies \lim_{t\to \infty} N_{t,a} = \infty 
%  \text{ and } \lim_{t\to \infty} \frac{N_{t,a}}{\Psi_{t,a}} = 1 \\
%  \lim_{t\to \infty} \Psi_{t,a} < \infty &\implies \sup_{t,a} N_{t,a} < \infty 
%  \text{ and } \sup_{t,a}|\mu_{t,a}| < \infty \\
%  \end{aligned}
%\]
%
%We can use this to prove the following:
%\begin{lemma}
%  For all arms $a$, $\lim_{t\to\infty} \Psi_{t,a} = \infty$.
%\end{lemma}
%
%\begin{proof-of-lemma}
%Consider a sample path $\omega$, and suppose this does not hold for some $a$. 
%  Since $\Psi_{t,a}(\omega)$ is monotonic, there exists a limit $\Psi_{\infty,a}(\omega)=\lim_{t\to\infty}\Psi_{t,a}$.
%  By the pigeonhole principle, since $\sum_{a}\Psi_{t,a}=1$ at every $t$, 
%  there must be at least 1 arm $b$ such that $\Psi_{t,b}\to\infty$. Note that
%\[
%\frac{\pi_{t,a}}{\pi_{t,b}}=\frac{s_{a}\left(\mathbb{E}\left[\frac{1}{\sigma_{t,a}}\phi\left(\frac{\theta_{t,a}^{*}-\mu_{t,a}}{\sigma_{t,a}}\right)\right]\right)^{1/2}}
%{s_{b}\left(\mathbb{E}\left[\frac{1}{\sigma_{t,b}}\phi\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{\sigma_{t,b}}\right)\right]\right)^{1/2}}
%\]
%Lemma~\ref{lemma:mrtngle-conv} implies that as $t\to\infty, \mu_{t,b}\to h_{b}$ almost surely, which implies 
%$\theta_{t,b}^{*}\to h_{b}^{*}$. Since $\Psi_{t,b}\to\infty$, $N_{t,b}\to\infty$. 
%Thus,
%\[
%s_{b}\left(\mathbb{E}\left[\frac{1}{\sigma_{t,b}}\phi\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{\sigma_{t,b}}\right)\right]\right)^{1/2}=s_{b}\left(\mathbb{E}\left[\sqrt{N_{t,b}}e^{-N_{t,b}\left(\frac{\theta_{t,b}^{*}-\mu_{t,b}}{s_{b}}\right)^{2}}\right]\right)^{1/2}\to0
%\]
%almost surely as well. 
%On the other hand, since $\lim_{t\to\infty}\Psi_{t,a}<\infty$, then Lemma~\ref{lemma:mrtngle-conv} implies that 
%$N_{t,a},\mu_{t,a}$ and $\theta_{t,a}^{*}$ will be bounded for all $t$ almost surely, which means that for $\omega$, there exists $\epsilon$ such that:
%
%\[
%\inf_{t \in \mathbb{N}}s_{a}\left(\mathbb{E}\left[\sqrt{N_{t,a}}e^{-N_{t,a}\left(\frac{\theta_{t,a}^{*}-\mu_{t,a}}{s_{a}}\right)^{2}}\right]\right)^{1/2}
%>\epsilon
%\]
%This means there exists $T_{M}$ large enough such that for all $t>T_{M}$, $\frac{\pi_{t,a}}{\pi_{t,a'}}>M$, which is a contradiction of $\lim_{t\to\infty}\Psi_{t,a}<\infty$.
%\end{proof-of-lemma}
%
%This implies that it is sufficient to track 
%$N_{t,a}$ in order to measure $\Psi_{t,a}$. 
%We define the index  $\nu_{t,a}:=\nu_{a}(N_{t,a})$ to be the quantity
%$I_{t,a} := 1\{a = \argmax_{b} \nu_{b}(N_{t,b})\}$.
%
%\[
%\nu_{a}(N_{t,a})=\log s_{a}+\frac{1}{4}\log N_{t,a}+\frac{1}{2}\log\mathbb{E}\left[e^{-N_{t,a}\left(\frac{\theta_{t,a}^{*}-\mu_{t,a}}{s_{a}}\right)^{2}}\right]+\xi_{a}
%\]



% %%% Local Variables:
% %%% mode: latex
% %%% TeX-master: "main"
% %%% End:


==> tv-bounds.tex <==
\subsection{Proof of Corollary~\ref{cor:proof-tv-rate}}
\label{section:proof-tv-rate}

For TV distance
\[
  \norm{f * \phi_{t} - \phi_{t}}_{1} \leq \sqrt{2t} \norm{\nabla f}_{1}
\]
and moreover
\[
  \begin{aligned}
  \norm{\nabla f}_{1} 
  &= \int_{\R^{K}} |\nabla f(x)| dx \\
  &= \int_{\R^{K}} |f(x) \nabla \log f(x)| dx \\
  &= \int_{\R^{K}} f(x) |\nabla \sum_{a} \log f_{a}(x_{a})| dx \\
  &\leq \int_{\R^{K}} f(x) \sum_{a}|\nabla  \log f_{a}(x_{a})| dx \\
  &\leq \sum_{a} \int_{\R^{K}} f(x) |\frac{\partial}{\partial x_{a}} \log f_{a}(x_{a})| dx \\
  & = \sum_{a} \int_{\R} f_{a}(x_{a}) |\frac{\partial}{\partial x_{a}} \log f_{a}(x_{a})| dx \\
  & = \sum_{a} \int_{\R} |f'_{a}(x_{a})| dx
  \end{aligned}
\]




While one would
expect pointwise convergence of $g_n(r_{0:t})$ to $g(r_{0:t})$ by the CLT,
proving the above requires controlling the convergence across random
realizations of the propensity score
$\pi_{t+1,a}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})$.  
This is complicated by the fact that we allow the propensity scores to be zero,
in which case we would not expect the CLT to hold. 
To handle this, we set a threshold $\epsilon$ and split the arms into those
with propensity scores larger than $\epsilon$  and those with scores less than $\epsilon$.
For the arms with large enough propensity scores, we use quantitative rates for the CLT
to bound the the discrepancy with its limiting Gaussian.
For the arms with small propensity scores, we show that both the aggregated rewards
$\sqrt{n}\bar{R}^{n}_{t+1}$ and the target Gaussian are close to zero.
We then scale $\epsilon$ with $n$ in order to ensure that the sample mean estimators
for all arms converges.
Although the set of arms in each group will change according to the random realizations
of the propensity scores, we provide uniform bounds of convergence for both groups.

We first define some new notation. In order to use quantify convergence of the CLT, we
use the bounded Lipschitz distance $d_{\text{BL}}$ to metrize weak convergence
\begin{equation*}
  d_{\text{BL}}(\mu, \nu) \defeq \sup\left\{
    |\mathbb{E}_{R \sim \mu}\bar{f}(R)-\mathbb{E}_{R \sim \nu}\bar{f}(R)|:
    \bar{f}\in\text{Lip}(\mathbb{R}^{\numarm}),
    \sup_{x,y\in\mathbb{R}^{\numarm}}|\bar{f}(x)-\bar{f}(y)|\leq1\right\}.
\end{equation*}
For $\epsilon >0$, let the set $I_{\epsilon}(\pstate_{0:t})$ be defined as the set of arms
whose propensity scores (given state $\pstate_{0:t}$) are bigger than $\epsilon$.
\[
I_{\epsilon}(\pstate_{0:t}) \defeq \{ a \in [\numarm]: \pi_{t+1,a}(\pstate_{0:t}) > \epsilon \}
\]
Let $\projeps(r_{0:t})$ and $\projepsc(r_{0:t})$
denote the projection operators of a vector in $\mathbb{R}^{\numarm}$
to a lower-dimensional vector containing only the coordinates corresponding to the arms
in $I_{\epsilon}(\pstate_{0:t})$ and its complement
$I_{\epsilon}(\pstate_{0:t})^{c}$ respectively. We use the shorthand $\projeps$, $\projepsc$
omitting dependence on $r_{0:t}$ whenever clear.
We use the notation $||\cdot||_{2,I^{c}_{\epsilon}} \defeq ||\projepsc \cdot ||_{2}$ to denote
the $2$-norm only among arms in $I^{c}_{\epsilon}$, and
$d_{\text{BL},\epsilon}(\cdot, \cdot) \defeq d_{\text{BL}}(\projeps \cdot, \projeps \cdot)$ 
to denote bounded Lipschitz distance only among arms in $I_\epsilon$.

We have the following bound for the difference in $g_n$ and $g$ in terms of bounded Lipschitz distance.

\[
  \begin{aligned}
    &|\E[g_{n}(\Pstate_{0},\ldots,\Pstate_{t})]-\mathbb{E}[g(\Pstate_{0},\ldots,\Pstate_{t})]| \\
    &=|\E[\E\left[f(\pstate_{0:t},\Pstate_{t+1})-f(\pstate_{0:t}, \Sigma_{t+1}^{1/2}(r_{0:t})Z + h\pi_{t+1}(r_{0:t}))|\Pstate_{0},\ldots \Pstate_{t}=\pstate_{0:t}\right]]| \\
    &\leq \E[\E\left[d_{\text{BL}}(\Pstate_{t+1}, \Sigma_{t+1}^{1/2}(r_{0:t})Z + h\pi_{t+1}(r_{0:t}))||\Pstate_{0},\ldots \Pstate_{t}=\pstate_{0:t}\right]] \\
  \end{aligned}
\]

We can then show that the bounded Lipschitz distance can be bounded by
the bounded Lipschitz distance between arms in $I_{\epsilon}(r_{0:t})$ and the 2-norm
between arms in $I_{\epsilon}(r_{0:t})^{c}$.

\begin{equation}
  \label{eqn:bl-props-ge-eps}
  \begin{aligned}
    &\E[\E_{\pstate_{0:t}} \left[d_{\text{BL}}(\Pstate_{t+1}, \Sigma_{t+1}^{1/2}(r_{0:t})Z + h\pi_{t+1}(r_{0:t}))\right]] \\
    &\leq \E[\E_{\pstate_{0:t}} \left[d_{\text{BL}, \epsilon}(\Pstate_{t+1},\Sigma_{t+1}^{1/2}(r_{0:t})Z + h\pi_{t+1}(r_{0:t}))\right]] \\
    & \qquad+\E [ \E_{\pstate_{0:t}} [ || \Pstate_{t+1} - \Sigma_{t+1}^{1/2}(r_{0:t})Z - h\pi_{t+1}(r_{0:t}) ||_{2,I_{\epsilon}^{c}}] ]
    \end{aligned}
\end{equation}

Since for any bounded 1-Lipschitz function $f$ and projection operators $\proj$, $\proj^{c}$
that project into mutually exclusive coordinates we have for any random vectors $A, B \in \R^{\numarm}$:
\[
  \begin{aligned}
  |\E f(A) - \E f(B)| &= |\E f(\proj A,\proj^{c} A) - \E f(\proj B, \proj^{c}B)| \\
                      &= |\E f(\proj A,\proj^{c} A) - \E f(\proj B, \proj^{c} A)|
                       + |\E f(\proj B, \proj^{c} A) - \E f(\proj B, \proj^{c} B)| \\
                            &\leq d_{\text{BL}}((\proj A,\proj^{c} A), (\proj B, \proj^{c} A))
                            + \E \ltwo{(\proj B, \proj^{c} A) - (\proj B, \proj^{c} B)} \\
                            & = d_{\text{BL}}(\proj A, \proj B) +  \E \ltwo{ \proj^{c} A, \proj^{c} B}
  \end{aligned}
\]

To bound the second part of the inequality (\ref{eqn:bl-props-ge-eps}),
we will show that for the arms whose propensity scores are less than $\epsilon$, 
both the sample mean estimators and the target Gaussian will be close to zero:

\[
  \begin{aligned}
  & \E \left[ \E_{\pstate_{0:t}} \left[ || \Pstate_{t+1} - \Sigma_{t+1}^{1/2}(r_{0:t})Z - h\pi_{t+1}(r_{0:t}) ||_{2, I_{\epsilon}^{c}}  \right] \right] \\
  &\leq \E \left[ \E_{\pstate_{0:t}} \left[ || \Pstate_{t+1} - \pi_{t+1}(\pstate_{0:t})h ||_{2, I_{\epsilon}^{c}} 
       +  || \Sigma^{1/2}_{t+1}(\pstate_{0:t})Z  ||_{2, I_{\epsilon}^{c}}  \right] \right] \\
  &\leq \epsilon^{1/2} \left( \sum_{a} \frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}} \right)^{1/2} + \epsilon^{1/2} (\max_{a} s_{t+1,a}) \numarm
\end{aligned}
\]

The last line uses the fact that:

\[
\begin{split}
  &\E \left[ \E_{\pstate_{0:t}} \left[  || \Pstate_{t+1} - \pi_{t+1}(\pstate_{0:t})h||_{2, I_{\epsilon}^{c}}   \right] \right] \\
  &  \leq \sqrt{n} \E \left[ \E_{\pstate_{0:t}} \left[ \sum_{a\in I_{\epsilon}^{c}(\pstate_{0:t})} 
  \left( \frac{1}{b_{t+1}n} \sum_{j=1}^{b_{t+1}n} \xi_{a,j}^{t+1} R_{a,j}^{t+1} - \pi_{t+1,a}(\pstate_{0:t})\frac{h}{\sqrt{n}} \right)^{2}
    \right] \right]^{1/2} \\
  & = \sqrt{n} \E \left[ \E_{\pstate_{0:t}} \left[  
    \sum_{a\in I_{\epsilon}^{c}(\pstate_{0:t})} \text{Var} \left( \frac{1}{b_{t+1}n} \sum_{j=1}^{b_{t+1}n} \xi_{a,j}^{t+1} R_{a,j}^{t+1} \right)
    \right] \right]^{1/2}\\
  & \leq \sqrt{n} \E \left[ \E_{\pstate_{0:t}} \left[  \sum_{a\in I_{\epsilon}^{c}(\pstate_{0:t})} \frac{\pi_{t+1,a}(\pstate_{0:t}) (s_{a}^{2} + h_{a}^{2})}{b_{t+1}n} \right] \right]^{1/2} \\
  &\leq \epsilon^{1/2} \left( \sum_{a} \frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}} \right)^{1/2}
\end{split}
\]
where the first inequality uses Jensen's inequality, and the second inequality uses the fact that 
$\text{Var}(\xi_{a,j}^{t+1}R_{a,j}^{t+1}) = \pi_{t+1,a}(\pstate_{0:t}) s_{t+1,a}^{2} + \pi_{t+1,a}(\pstate_{0:t})(1-\pi_{t+1,a}(\pstate_{0:t}))h_{a}^{2}$.

It remains then to bound the first part of the inequality \eqref{eqn:bl-props-ge-eps}, which
measures the distance between the sample mean estimator and its limiting Gaussian for the arms
with propensity scores greater than $\epsilon$.

First, if $I_{\epsilon}(\pstate_{0:t})$ is empty, then the distance is automatically zero. Moreover,
for $\epsilon < 1/\numarm$ there will always be at least 1 arm in $I_{\epsilon}(\pstate_{0:t})$, so without loss we assume that
$|I_{\epsilon}(\pstate_{0:t})| = m > 0$ for some $m$. We can observe the following decomposition:

\begin{align}
  & \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}, \epsilon}(\Pstate_{t+1},\Sigma_{t+1}^{1/2}(r_{0:t})Z + h\pi_{t+1}(r_{0:t})) \right]] \nonumber \\
  & \leq \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}, \epsilon} (\Pstate_{t+1} - \pi_{t+1}(\pstate_{0:t})h, \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z ) \right]] \nonumber \\
  & \qquad+ \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}, \epsilon} (\Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z, \Sigma^{1/2}_{t+1}(\pstate_{0:t})Z ) \right]]
    \label{eqn:bl-triangle}
\end{align}

The first part of the preceding inequality~\eqref{eqn:bl-triangle} measures
the distance between $\sqrt{n}\bar{R}^{n}_{t+1}$ and its Gaussian limit
$\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h\pi_{t+1}(r_{0:t})$ under the CLT. For any finite $n$, the
covariance of this Gaussian $\Sigma_{n,t+1}$ not only includes the variance of
the arm rewards but also correlations that emerge from sampling arms according
to a random multinomial vector (rather than a deterministic allocation).
However, these effects vanish as $n\to\infty$ and the covariance matrix
converges to the diagonal covariance matrix
$\Sigma_{t+1}(r_{0:t})$~\eqref{eqn:cov}. The distance between these two
Gaussians is captured by the second part of the preceding
inequality~\eqref{eqn:bl-triangle}.

We proceed to bound the first term in \eqref{eqn:bl-triangle}.
First we define some new notation. Let $Q_{n}^{t+1}(\pstate_{0:t})$ be the vector of
normalized sample mean estimators, projected to the arms in $I_{\epsilon}$:

\begin{equation*}
  \begin{split}
  Q_{n}^{t+1}(\pstate_{0:t}) &\defeq
  \left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{-1/2}\projeps(\Pstate_{t+1} - \pi_{t}(\pstate_{0:t})h) \\
  &= \left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{-1/2} \frac{1}{\sqrt{b_{t+1}n}}\sum_{j=1}^{b_{t+1}n} 
  \left(
    \projeps \left( \xi_{j}^{t}R_{j}^{t} -\frac{\pi_{t+1}(\pstate_{0:t})h}{\sqrt{n}} \right)
  \right)
  \end{split}
\end{equation*}
where the conditional covariance $\Sigma_{n,t+1}(\pstate_{0:t})$ is:

\[
  \Sigma_{n,t+1}(\pstate_{0:t}) \defeq \text{Cov} \left(\frac{\xi_{j}^{t+1}R_{j}^{t+1}}{b_{t+1}}\right) = \Sigma_{t+1}(\pstate_{0:t}) 
  + \frac{1}{b_{t+1}n}\text{diag}(\pi_{t+1,a}(\pstate_{0:t})h_{a}^{2}) - \frac{1}{b_{t+1}n}(\pi_{t+1}(\pstate_{0:t})h)(\pi_{t+1}(\pstate_{0:t})h)^{\top}
\]

Note that conditional on $\pstate_{0:t}$, $Q^{t+1}_{n}$ is a normalized sum of independent random vectors since
$\text{Cov}\left(\projeps ( \xi_{j}^{t}R_{j}^{t}) \right)= \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top}$.
It is useful to state the following bounds for the maximum and minimum
eigenvalues of $\projeps \Sigma_{n,t+1} \projeps^{\top}$.

\begin{lemma} \label{lemma:min-max-eig} 
  Suppose that $|I_{\epsilon}(\pstate_{0:t})|> 0$. Let $\lambda_{\max}(\cdot)$ and $\lambda_{\min}(\cdot)$ denote
  the maximum and minimum eigenvalues respectively. For any realization of $\pstate_{0:t}$, we have that:
  \[
    \begin{aligned}
    \lambda_{\max} (\projeps \Sigma_{n,t+1} \projeps^{\top}) &\leq \lambda_{\max}
    \left( \projeps\Sigma_{t+1} \projeps^{\top}
    +\frac{1}{b_{t+1}n} \projeps \text{diag} \left( \pi_{t+1,a}h_{a}^{2} \right) \projeps^{\top}\right)
    \leq \max_{a}\left( \frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}} \right) \\
    \lambda_{\min} (\projeps \Sigma_{n,t+1} \projeps^{\top}) 
    & \geq \lambda_{\min}(\projeps  \Sigma_{t+1} \projeps^{\top})
    +\frac{1}{b_{t+1}n}  \lambda_{\min}\left( \projeps \left( \text{diag}(\pi_{t+1,a}h_{a}^{2})
    -  (\pi_{t+1}h)(\pi_{t+1}h)^{\top} \right)  \projeps^{\top} \right)\\
    &\geq \epsilon \left( \min_{a}s_{t+1,a}^{2}  \right) \\
    \end{aligned}
  \]
\end{lemma}

\begin{proof-of-lemma}
  The first inequality follows since
  $\lambda_{\max}(A + B) \le \lambda_{\max}(A) + \lambda_{\max}(B)$ for
  symmetric matrices $A,B \in \R^{m\times m}$. The second inequality uses
  $\lambda_{\min}(A + B) \geq \lambda_{\min}(A) + \lambda_{\min}(B)$.
  Moreover, for any $b\in \R^{m}$
  \[
  \begin{split}
  & b^{\top} \projeps \left( \text{diag}(\pi_{t+1,a}(\pstate_{0:t})h_{a}^{2}) - (\pi_{t+1}(\pstate_{0:t})h)(\pi_{t+1}(\pstate_{0:t})h)^{\top} \right)\projeps^{\top} b \\
  &= \sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t})h_{a}^{2}b_{a}^{2} - \left( \sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t})h_{a}b_{a} \right)^{2} \geq 0
  \end{split}
  \]
  as by Cauchy-Schwartz:
  \[
   \left( \sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t})h_{a}b_{a} \right)^{2} \leq \left(\sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t}) \right)
   \left(\sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t})h_{a}^{2}b_{a}^{2} \right) \leq \left(\sum_{a\in I_{\epsilon}(\pstate_{0:t})} \pi_{t+1,a}(\pstate_{0:t})h_{a}^{2}b_{a}^{2} \right)
  \]
so the matrix is positive semi-definite
\end{proof-of-lemma}
We begin with bounding the first term in \eqref{eqn:bl-triangle}. Since for any $1$-Lipschitz function $f$,
the Lipschitz constant of $v \mapsto f(\left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{1/2} v)$ is 
$\lambda_{\max} \left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{1/2} $,

\[
  \begin{split}
  & \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}, \epsilon} (\projeps \left( \Pstate_{t+1} - \pi_{t+1}(\pstate_{0:t})h \right), \projeps \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z ) \right]] \\
  & \leq \lambda_{\max} \left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{1/2} 
  \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}}  \left( Q_{n}^{t+1}(\pstate_{0:t}) ,
\left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{-1/2} 
  \projeps \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z \right) \right]] \\
  & \leq \max_{a} \left(\frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}}\right)^{1/2} \E[\E_{\pstate_{0:t}} 
  \left[ d_{\text{BL}} (Q_{n}^{t+1}(\pstate_{0:t}),  Z) \right]]
  \end{split}
\]
\noindent using the upper bound for the max eigenvalue in Lemma \ref{lemma:bayes-min-max-eig}, and the fact that

\[
  \left( \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \right)^{-1/2} \projeps \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z \sim N(0, I_{m})
\]

Under the assumption  via a classical result, which is a corollary
of~\citet[Theorem 1]{Bhattacharya70}.  The following result explicitly
quantifies how the rate of convergence depends on the propensity scores,
allowing us to guarantee uniform convergence.
\begin{lemma}[{\citet[Theorem 1]{Bhattacharya70}}]. 
  \label{lemma:clt-rate}
  Let $\{X_i\}_{i =1}^n$ be a sequence of $n$ independent random vectors
  taking values in $\R^{\numarm}$ with covariance matrix $\Sigma_n$. Assume
  that for some $\delta > 0$
  \begin{equation*}
    M \defeq \sup_{n} \frac{1}{n} \sum_{i=1}^{n}
    \E \ltwo{\Sigma_{n}^{-1/2} X_{i}}^{3+\delta} < \infty.
  \end{equation*}
  Then, the normalized partial sum
  $\bar{Z}_{n} = \frac{1}{\sqrt{n}} \sum_{i=1}^{n} \Sigma_{n}^{-1/2} X_{i}$
  satisfies
  \begin{equation*}
    d_{\text{BL}}(\bar{Z}_n, N(0, I))
    \leq A_{K,\delta} M^{\frac{3+3\delta}{3+\delta}}n^{-1/2} + B_{K,\delta} M^{\frac{3}{3+\delta}}n^{-1/2}
  \end{equation*}
  where $A_{K,\delta}, B_{K,\delta}$ are constants that only depends on $K$ and
  $\delta$. 
\end{lemma}
\noindent  In order to guarantee uniform convergence over $r_{0:t}$ using
Lemma~\ref{lemma:clt-rate}, we use
Assumptions~\ref{assumption:reward}\ref{item:moment}
to control the moment term $M$.
Using $C_{\numarm, \delta}$ to denote a constant that only depends on
$\numarm$ and $\delta$ (that may differ line by line), use lower bound on the
minimum eigenvalue of $\Sigma_{n,t+1}$ given in Lemma~\ref{lemma:min-max-eig}
to get

\begin{equation*}
  \begin{split}
  M(\pstate_{0:t})
  & \defeq \sup_{n} \frac{1}{b_{t+1}n}\sum_{j=1}^{b_{t+1}n} \mathbb{E}
    \ltwo{\Sigma_{n,t+1}(\pstate_{0:t})^{-1/2} 
   \left(
      \xi_{j}^{t+1}R_{j}^{t+1} -\frac{\pi_{t+1,a}(\pstate_{0:t})h_{a}}{\sqrt{n}}
    \right)}^{3+\delta} \\
  & \leq \left( \epsilon \min_{a} s_{t+1,a}^{2} \right)^{-\frac{3+\delta}{2}} 
  \sup_{n} \frac{1}{b_{t+1}n}\sum_{j=1}^{b_{t+1}n} \mathbb{E}
  \ltwo{\projeps \left( \xi_{j}^{t+1}R_{j}^{t+1} -\frac{\pi_{t+1}(\pstate_{0:t})h}{\sqrt{n}}\right)}^{3+\delta} \\
      &\leq C_{k,\delta} \left( \epsilon \min_{a} s_{t+1,a}^{2} \right)^{-\frac{3+\delta}{2}}
      \max_{a} \E \left|\xi_{a,j}^{t+1}R_{a,j} - \frac{\pi_{t+1,a}(\pstate_{0:t})h_{a}}{\sqrt{n}}\right|^{3+\delta} < \infty\\
  \end{split}
\end{equation*}

Using Assumption~\ref{assumption:reward}\ref{item:moment}, conclude

\[
  M(\pstate_{0:t})\leq C_{k,\delta} \left( \epsilon \min_{a} s_{t+1,a}^{2} \right)^{-\frac{3+\delta}{2}} 
  \left( C + \left(\frac{\max_{a} |h_{a}|}{\sqrt{n}} \right)^{3+\delta} \right) < \infty 
\]
where $C$ is the moment bound in $\epsilon_{a}$ given in Assumption~\ref{assumption:reward}\ref{item:moment}.

Apply Lemma~\ref{lemma:clt-rate} to get

\[
  \begin{split}
  &\E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}} ( Q_{n}^{t+1}, \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z )\right]] \\
  & \leq \max_{a} \left(\frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}}\right)^{1/2} \cdot \E[\E_{\pstate_{0:t}} 
  \left[ A_{m,\delta} M(\pstate_{0:t})^{\frac{3+3\delta}{3+\delta}} (b_{t+1}n)^{-1/2}
  + B_{m,\delta} M(\pstate_{0:t})^{\frac{3}{3+\delta}} (b_{t+1}n)^{-1/2} \right]]
  \end{split}
\]


Taking expectation over $\pstate_{0:t}$ and using the preceding bound on $M(\pstate_{0:t})$, we have that
\[
  \begin{split}
  & \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}} (Q_{n}^{t+1}, \Sigma^{1/2}_{n,t+1}(\pstate_{0:t})Z )\right]] \\
  & \leq \max_{a} \left(\frac{s_{a}^{2} + h_{a}^{2}}{b_{t+1}}\right)^{1/2} \cdot 
  \E[\E_{\pstate_{0:t}} \left[ A_{m,\delta} M(\pstate_{0:t})^{\frac{3+3\delta}{3+\delta}} (b_{t+1}n)^{-1/2}
  + B_{m,\delta} M(\pstate_{0:t})^{\frac{3}{3+\delta}} (b_{t+1}n)^{-1/2}
   \right]] \\
  & \leq n^{-1/2} \cdot C_{k,\delta,s,b_{t}} \epsilon^{-\frac{3+3\delta}{2}} 
  \left( C^{\frac{3+3\delta}{3+\delta}} + \frac{\max_{a} \{|h_{a}|^{4+3\delta} + |h_{a}|^{3+3\delta} \}}{n^{\frac{3+3\delta}{2}}} \right) \\
  &+n^{-1/2} \cdot B_{k,\delta,s,b_{t}} \epsilon^{-\frac{3}{2}}
  \left( C^{\frac{3}{3+\delta}} + \frac{3}{(3+\delta)C^{\frac{\delta}{3+\delta}}}\frac{\max_{a} \{|h_{a}|^{4 + \delta} + |h_{a}|^{3 + \delta} \}}{n^{\frac{3+\delta}{2}}} \right)
  \end{split}
\]
where $C_{k,\delta,s,b_{t}}, B_{k,\delta,s,b_{t}}$ are constants that only depend on $K,\delta$, measurement noise $s^{2}$,
and batch scale $b_{t}$. Note that this bound holds regardless of the realization of $\pstate_{0:t}$.

Finally, we show uniform convergence of the second term in the
bound~\eqref{eqn:bl-triangle}, that the limiting Gaussian
$N(0, \Sigma_{n,t+1}^{1/2}(r_{0:t}))$ converges uniformly to
$N(0, \Sigma_{t+1}^{1/2}(r_{0:t}))$ as $n\to \infty$
\begin{equation*}
  \E\left[\E_{r_{0:t}}\left[d_{\text{BL}, \epsilon}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z,
        \Sigma_{t+1}^{1/2}(r_{0:t})Z\right) \right]\right] \to 0
\end{equation*}
First, for any two measures $(\mu,\nu)$, $d_{\text{BL}}(\mu,\nu)$ is upper
bounded by the total variation distnace $2d_{\text{TV}}(\mu,\nu)$, which is in
turn bounded above by KL divergence $\sqrt{\frac{1}{2}d_{\text{KL}}(\mu,\nu)}$
by Pinsker's inequality. We derive the following concrete bound on the KL
divergence, whose proof we defer to Section~\ref{section:proof-kl-cov}.

\begin{lemma}\label{lemma:kl-cov} The KL-divergence between $N(0, \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top})$ and
  $N(0, \projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top})$
  is bounded above as follows:
\[
 \dkl{N \left( 0,\projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top}) \right)}{N \left( 0, \projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top} \right)}
  \leq \frac{1}{b_{t+1}n} \left[\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right]
\]
\end{lemma}

This guarantees that:
\[
  \begin{split}
  &\E\left[\E_{r_{0:t}}\left[d_{\text{BL}, \epsilon}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z,
  \Sigma_{t+1}^{1/2}(r_{0:t})Z\right) \right]\right] \\
  &\leq (b_{t+1}n)^{-1/2} \sqrt{2}\left(\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right)^{1/2}
  \end{split}
\]

Altogether, we have shown that
\[
  |\E[g_{n}(\Pstate_{0},\ldots,\Pstate_{t})]-\mathbb{E}[g(\Pstate_{0},\ldots,\Pstate_{t})]|
  \leq A\epsilon^{1/2} + B\epsilon^{-\frac{3+3\delta}{2}}n^{-1/2} + C\epsilon^{-\frac{3}{2}}n^{-1/2} + Dn^{-1/2}
\]
where $A,B,C,D$ are constants that do not depend on $\epsilon$ or $n$, but may depend on $h,s,\delta,K,b_{t+1}$. Since the choice of threshold $\epsilon$ was arbitrary,
we can set $\epsilon = n^{-\frac{1}{4+3\delta}}$ and obtain a rate of convergence of $n^{-\frac{1}{8 + 6\delta}}$.

Thus, this shows that $\E[f(\Pstate_{0},\ldots,\Pstate_{t+1})] \to \E[f(G_{0},\ldots,G_{t+1})]$ as $n\to \infty$ 
for any bounded Lipschitz function $f$, which implies the desired weak convergence.

\subsubsection{Proof of Lemma~\ref{lemma:kl-cov} \label{section:proof-kl-cov}}

We use the expression for the KL-divergence between two multivariate normal distributions:

\[
  \begin{aligned}
	& \dkl{N(0, \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top})}{N(0, \projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top})} \\
	&=\text{tr}\left((\projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top})^{-1} \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top}\right)
   - m +\log\frac{\det\projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top}}{\det\projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top}} \\
  &=\sum_{a \in I_{\epsilon}(\pstate_{0:t})} \left( s_{t+1,a}^{2}\pi_{t+1,a}(\pstate_{0:t}) \right)^{-1} 
  \left(s_{t+1,a}^{2}\pi_{t+1,a}(\pstate_{0:t}) + \pi_{t+1,a}(\pstate_{0:t}) (1 - \pi_{t+1,a}(\pstate_{0:t})) \frac{h_{a}^{2}}{b_{t+1}n} \right)-m \\
  &\qquad +\log\det \projeps \Sigma_{t+1}(\pstate_{0:t}) \projeps^{\top} -\log\det \projeps \Sigma_{n,t+1}(\pstate_{0:t}) \projeps^{\top} \\
	&\leq \sum_{a \in I_{\epsilon}(\pstate_{0:t})} \frac{1}{b_{t+1}n} \frac{\left(1-\pi_{t+1,a}(\pstate_{0:t})\right)h_{a}^{2}}{s_{t+1, a}^{2}}
  +\sum_{a \in I_{\epsilon}(\pstate_{0:t})} \log\left( s_{t+1,a}^{2}\pi_{t+1,a}(\pstate_{0:t}) \right) \\
  & \qquad-\sum_{a \in I_{\epsilon}(\pstate_{0:t})}\log\left(s_{t+1,a}^{2}\pi_{t+1,a}(\pstate_{0:t})+\frac{1}{b_{t+1}n}h_{a}^{2}\pi_{t+1,a}(\pstate_{0:t})\right) 
  + \left(\frac{1}{b_{t+1}n}\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})} \right) \\
	&\leq\frac{1}{b_{t+1}n}\left[\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right) + \frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{a}^{2}+h_{a}^{2})}\right]
\end{aligned}
\]

We obtain $\det{\projeps\Sigma_{n,t+1}(\pstate_{0:t})\projeps^{\top}}$ using the fact that $\Sigma_{n,t+1}(\pstate_{0:t})$ is a rank-one perturbation of a diagonal matrix:

\[
  \begin{aligned}
  &\log\det \projeps\Sigma_{n,t+1}\projeps^{\top}	\\
  &=\log\det\left(\projeps \left( \Sigma_{t+1}+\frac{1}{b_{t+1}n}\text{diag}\left(\pi_{t+1,a}h_{a}^{2}\right)\right) \projeps^{\top}\right) \\
  &\qquad+\log\det\Bigl(I + \left( \projeps \left(\Sigma_{\epsilon,t}+\frac{1}{b_{t+1}n}\text{diag}\left(\pi_{t+1,a}h_{a}^{2}\right)\right)\projeps^{\top}\right)^{-1}
   \left(-\frac{1}{b_{t+1}n}\projeps(\pi_{t+1}h)(\pi_{t+1}h)^{\top}\projeps^{\top}\right)\Bigr) \\
	&=\sum_{a \in I_{\epsilon}} \log\left(s_{t+1,a}^{2}\pi_{t+1,a}+\frac{1}{b_{t+1}n}h_{a}^{2}\pi_{t+1,a}\right)  \\
  &\qquad+\log\det\left(I-\frac{1}{b_{t+1}n}(\projeps \pi_{t+1}h)^{\top}\left(\projeps \left(\Sigma_{t+1}
  +\frac{1}{b_{t+1}n}\text{diag}\left(\pi_{t+1,a}h_{a}^{2}\right)\right)\projeps^{\top}\right)^{-1}(\projeps\pi_{t+1}h)\right) \\
	&=\sum_{a \in I_{\epsilon}} \log\left(\pi_{t+1,a}s_{t,a}^{2}+\frac{1}{b_{t+1}n}\pi_{t+1,a}h_{a}^{2}\right)
  +\log\left(1-\frac{1}{b_{t+1}n} \sum_{a \in I_{\epsilon}} \pi_{t+1,a}\frac{h_{a}^{2}}{s_{t+1,a}^{2}+(1/n)h_{a}^{2}}\right) \\
  &\geq \sum_{a \in I_{\epsilon}} \log\left(\pi_{t+1,a}s_{t,a}^{2}+\frac{1}{b_{t+1}n}\pi_{t+1,a}h_{a}^{2}\right)
   + \log\left(1- \frac{1}{b_{t+1}n}\max_{a} \frac{h_{a}^{2}}{s_{t,a}^{2}+(1/b_{t+1}n)h_{a}^{2}}\right)
  \end{aligned}
\]

Finally, we use the bound $\log(1-x)\geq \frac{-x}{1-x}$ to obtain

\[
  \begin{aligned}
    \log\det\Sigma_{n,t+1}&\geq \sum_{a \in I_{\epsilon}} 
    \log\left(\pi_{t+1,a}s_{t+1,a}^{2}+\frac{1}{b_{t+1}n}\pi_{t+1,a}h_{a}^{2}\right)
    -  \frac{1}{b_{t+1}n}\frac{\max_{a} \frac{h_{a}^{2}}{s_{t+1,a}^{2}+(1/b_{t+1}n)h_{a}^{2}}}{1 - \max_{a} \frac{h_{a}^{2}}{b_{t+1}ns_{t+1,a}^{2}+h_{a}^{2}}} \\
  &\geq \sum_{a \in I_{\epsilon}} \log\left(\pi_{t+1,a}s_{t+1,a}^{2}+\frac{1}{b_{t+1}n}\pi_{t+1,a}h_{a}^{2}\right)
   -  \frac{1}{b_{t+1}n}\frac{\max_{a} h_{a}^{2}/s_{t,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{a}^{2}+h_{a}^{2})} \\
  \end{aligned}
\]



\subsection{Proof of Theorem \ref{theorem:limit}}
\label{section:proof-limit}

Let $s_{t, a}^{2} \defeq s_a^{2}/b_{t}$ be the rescaled measurement variance.
Recall the Gaussian sequential experiment given in Definition~\ref{def:gse}:
for all $0< t \le T-1$
\begin{equation*}
  G_{0}\sim N(h,\Sigma_{0}),
  ~~G_{t}|G_{t-1},\ldots,G_{0} \sim N(h,\Sigma_{t})
\end{equation*}
where $\Sigma_{t}=\text{diag}(s_{t}^{2}/\pi_{t}(G_{1},...,G_{t-1}))$ and
$\Sigma_{0}=\text{diag}(s_{t}^{2}/\pi_{0})$.


We use an inductive argument to prove the weak
convergence~\eqref{eqn:weak-convergence} for a policy $\pi$ and reward process
$R_{a,t}$ satisfying
Assumptions~\ref{assumption:reward},~\ref{assumption:policy}.  For the base
case, since $\pi _{0}$ is a fixed vector, Lindeberg CLT gives
$\sqrt{n} \bar{R}^{n}_{0} \cd N(h,\Sigma_0)$.  Next, suppose
\begin{equation}
  \label{eqn:inductive-hypothesis}
  (\sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t})
  \cd (G_{0},...,G_{t}).
\end{equation}
To show weak convergence to $G_{t+1}$, it is sufficient to show 
\begin{equation}
  \label{eqn:inductive-weak-convergence}
  \E[f(\sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t+1})] \to
  \E[f(G_{0},...,G_{t+1})]~~\mbox{for any
bounded Lipschitz function}~f
\end{equation}
Fixing a bounded Lipschitz $f$, assume without loss of generality that
\begin{equation*}
  \sup_{x,y\in\mathbb{R}^{(t+1)\times k}}|f(x)-f(y)|\leq 1
  ~~~\mbox{and}~~~f\in\text{Lip}(\mathbb{R}^{(t+1)\times K}).
\end{equation*}


We first set up some basic notation. For any
$r_{0:t} \in \R^{(t+1) \times \numarm}$, define the conditional expectation
operator on a random variable $W$
\begin{equation*}
  \E_{r_{0:t}}[W] \defeq \E\left[ W \Bigg| \sqrt{n} \left\{\bar{R}^n_s\right\}_{s=0}^t = r_{0:t}\right].
\end{equation*}
Then, conditional on realizations of previous importance sampling estimators
up to time $t$, let $g_{n},g:\R^{t\times K} \to \R$ be the conditional
expectation of $f$ and its limiting counterpart
\begin{align*}
  g_{n}(r_{0:t}) &\defeq
             \E_{r_{0:t}}\left[f\left(\sqrt{n}\bar{R}_{0}^{n}, \ldots,
             \sqrt{n}\bar{R}_{t}^{n},\sqrt{n}\bar{R}_{t+1}^{n}\right)\right]
             = \E\left[f\left(r_{0:t}, \sqrt{n}\bar{R}_{t+1}^{n}\right)\right] \\
  g(r_{0:t}) & \defeq \E_{r_{0:t}}\left[f\left(\sqrt{n}\bar{R}_{0}^{n}, \ldots,
         \sqrt{n}\bar{R}_{t}^{n},\Sigma_{t+1}^{1/2}(r_{0:t})Z + h\right)\right]
         = \E\left[f\left(r_{0:t}, \Sigma_{t+1}^{1/2}(r_{0:t})Z + h\right)\right]
\end{align*}
where $Z\sim N(0,I)$ and the covariance at history $r_{0:t}$ is determined by the
propensity scores $\pi_{t+1,a}(r_{0:t})$
\begin{equation}
  \label{eqn:cov}
  \Sigma_{t+1}(r_{0:t}) \defeq \text{diag}\left(\frac{s_{t+1}^{2}}{\pi_{t+1}(r_{0:t})}\right).
\end{equation}
Conditional on the history $r_{0:t}$, $\sqrt{n}\bar{R}_{t+1}^{n}$ depends on
$r_{0:t}$ only through the propensity scores $\pi_{t+1,a}(r_{0:t})$.


To show the weak convergence~\eqref{eqn:inductive-weak-convergence}, decompose the
difference between
$\E[f(\sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t})]$ and
$\E[f(G_{0},\ldots,G_{t})]$ in terms of $g_{n}$ and $g$
\begin{align}
  &|\mathbb{E}[f(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t+1}^{n})]
     - \mathbb{E}[f(G_{0},...,G_{t+1})]| \label{eqn:start} \\ 
  & =|\mathbb{E}[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]
    -\mathbb{E}[g(G_{0},...,G_{t})]|  \nonumber  \\
  & =|\mathbb{E}[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]
    -\mathbb{E}[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]|
    +|\E[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]-\mathbb{E}[g(G_{0},...,G_{t})]| \nonumber
\end{align}
By Assumption~\ref{assumption:policy}\ref{item:continuity} and dominated
convergence, $g$ is continuous almost surely under $(G_0, \ldots, G_{t})$.
From the inductive hypothesis~\eqref{eqn:inductive-hypothesis}, the continuous mapping theorem implies
\begin{equation*}
  \E[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})] \to \mathbb{E}[g(G_{1},...,G_{t})].
\end{equation*}

It remains to show the convergence
$\E[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})] \to
\E[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]$.  While one would
expect pointwise convergence of $g_n(r_{0:t})$ to $g(r_{0:t})$ by the CLT,
proving the above requires controlling the convergence across random
realizations of the propensity score
$\pi_{t+1,a}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})$.  Toward
this goal, we metrize the weak convergence in the central limit theorem
conditional on the history $r_{0:t}$, and quantify the convergence rate
depends on $r_{0:t}$. We show that given sufficient overlap in the propensity
scores (Assumption~\ref{assumption:policy}\ref{item:overlap}), we have
appropriate uniform convergence of $g_n$ to $g$ over values of $r_{0:t}$.  We
use the bounded Lipschitz distance $d_{BL}$ to metrize weak convergence
\begin{equation*}
  d_{\text{BL}}(\mu, \nu) \defeq \sup\left\{
    |\mathbb{E}_{R \sim \mu}\bar{f}(R)-\mathbb{E}_{R \sim \nu}\bar{f}(R)|:
    \bar{f}\in\text{Lip}(\mathbb{R}^{\numarm}),
    \sup_{x,y\in\mathbb{R}^{\numarm}}|\bar{f}(x)-\bar{f}(y)|\leq1\right\}.
\end{equation*}

We can observe that bounded Lipschitz distance controls the convergence of
$g_n(r_{0:t})$ to $g(r_{0:t})$
\begin{align*}
  &\left|\E\left[g_{n}\left(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}\right)\right]
    -\mathbb{E}\left[g\left(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}\right)\right]\right| \\
  &=\E\left[\mathbb{E}\left[f\left(r_{0:t},\sqrt{n}\bar{R}_{t+1}^{n}\right)
    -f\left(r_{0:t},\Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right) \mid
    \sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right] \\
  &\le \E\left[\E\left[d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n}, \Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right)
    \mid\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right] \\
  &\le \E\left[\E\left[d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n}, \Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h\right)
    \mid \sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right] \\
  & \qquad + \E\left[\E\left[d_{\text{BL}}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h,
    \Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right)
    \mid \sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right]
\end{align*}

The first part of the last inequality measures the distance between $\sqrt{n}\bar{R}^{n}_{t+1}$
and its Gaussian limit $\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h$ under the CLT, where $\Sigma_{n,t+1}$
denotes the conditional covariance:
\begin{equation*}
  \Sigma_{n,t+1}(r_{0:t}) \defeq
  \text{Cov}\left(\frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(r_{0:t})}\right)
  = \Sigma_{t+1}(r_{0:t})+\frac{1}{n} \text{diag} \left( \frac{h^2}{\pi_{t+1}(r_{0:t})} \right)- \frac{1}{n}hh^{\top}
\end{equation*}
so that $\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h$ is the Gaussian limit of
$\sqrt{n}\bar{R}^{n}_{t+1}$ by the CLT.
Use the triangle inequality to arrive at
\begin{align}
  & |\E[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]
    - \mathbb{E}[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]| \nonumber \\
  & \le \E\left[\E\left[d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n},
    \Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h\right)
    \mid \sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right] \nonumber \\
  &\qquad + \E\left[\E\left[d_{\text{BL}}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h,
    \Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right)
    \mid \sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=r_{0:t}\right]\right].
    \label{eqn:bl-triangle}
\end{align}
The first part of the preceding inequality~\eqref{eqn:bl-triangle} measures
the distance between $\sqrt{n}\bar{R}^{n}_{t+1}$ and its Gaussian limit
$\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h$ under the CLT. For any finite $n$, the
covariance of this Gaussian $\Sigma_{n,t+1}$ not only includes the variance of
the arm rewards but also correlations that emerge from sampling arms according
to a random multinomial vector (rather than a deterministic allocation).
However, these effects vanish as $n\to\infty$ and the covariance matrix
converges to the diagonal covariance matrix
$\Sigma_{t+1}(r_{0:t})$~\eqref{eqn:cov}. The distance between these two
Gaussians is captured by the second part of the preceding
inequality~\eqref{eqn:bl-triangle}.

% Let $\sqrt{n}\widehat{R}_{t+1}^{n}\equiv\sqrt{n}\bar{R}_{t+1}^{n}-h$ be the
% demeaned estimator \hn{This notation is only used a couple times. Let's not
% introduce unnecessary notation.} and define

To show the uniform convergence of the first term in the
bound~\eqref{eqn:bl-triangle}, we first set up some requisite notation.  Let
$Q_{n}^{t+1}(y)$ be the demeaned, normalized importance sampling estimator
\begin{equation*}
  Q_{n}^{t+1}(r_{0:t}) \defeq
  \Sigma_{n,t+1}^{-1/2}(r_{0:t})(\sqrt{n}\bar{R}_{t+1}^{n} - h)
  = \frac{1}{\sqrt{n}}\sum_{j=1}^{n} \Sigma_{n,t+1}^{-1/2}(r_{0:t})
  \left(
    \frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(r_{0:t})} -\frac{h}{\sqrt{n}}
  \right).
\end{equation*}
The terms in the preceding sum are i.i.d. across $j$ and have mean zero and
identity covariance. Since for any 1-Lipschitz function $f$, the Lipschitz constant of
$v \mapsto f\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})v\right)$ is
$\lambda_{\max}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})\right)$,
\begin{align*}
  d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n},\Sigma_{t+1}^{1/2}(r_{0:t})Z + h\right)
  & \le d_{\text{BL}}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Q_{n}^{t+1}(r_{0:t}),
    \Sigma_{n,t+1}^{1/2}(r_{0:t})Z\right) \\
  & \le \lambda_{\max}(\Sigma_{n,t+1}^{1/2}(r_{0:t})) d_{\text{BL}}\left(Q_{n}^{t+1}(r_{0:t}),Z\right)
\end{align*}



A key observation is that $\Sigma_{n,t+1}(r_{0:t})$ is a rank-one perturbation
of a diagonal matrix, which allows us to use standard results to bound its
minimum and maximum eigenvalues.
\begin{lemma}[{\citet[Section 5]{Golub73}}]
  \label{lemma:min-max-eig}
  Let $\lambda_{\max}(\cdot)$ and $\lambda_{\min}(\cdot)$ denote the maximum
  and minimum eigenvalues respectively. We have
  \begin{align*}
    \lambda_{\max} (\Sigma_{n,t+1}(r_{0:t}))
    &\leq \lambda_{\max}
      \left( \Sigma_{t+1}(r_{0:t})+\frac{1}{n}
      \diag \left( \frac{h_{a}^2}{\pi_{t+1,a}(r_{0:t})} \right) \right) 
    \leq \max_{a}\left(\frac{s_{t+1,a}^{2} + h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right) \\
    \lambda_{\min} (\Sigma_{n,t+1}(r_{0:t}))
    & \geq \lambda_{\min}(\Sigma_{t+1}(r_{0:t}))
      + \frac{1}{n} \lambda_{\min}
      \left( \diag \left( \frac{h_{a}^2}{\pi_{t+1,a}(r_{0:t})} \right) - hh^{\top} \right)
      \geq \min_{a}\left( \frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})} \right) 
  \end{align*}
\end{lemma}
\begin{proof-of-lemma}
  The first inequality follows since
  $\lambda_{\max}(A + B) \le \lambda_{\max}(A) + \lambda_{\max}(B)$ for
  symmetric matrices $A,B \in \R^{K\times K}$. The second inequality uses
  $\lambda_{\min}(A + b) \geq \lambda_{\min}(A) + \lambda_{\min}(B)$ and the
  fact that
  $\text{Cov}\left(\frac{\xi_{j}^{t+1} h }{\pi_{t+1}(r_{0:t})}\right) =
  \text{diag} \left( \frac{h^2}{\pi_{t+1}(r_{0:t})}\right) - hh^{\top} \succeq
  0$.
\end{proof-of-lemma}
\noindent Using Lemma \ref{lemma:min-max-eig}, we arrive at a bound on the
first part of the inequality~\eqref{eqn:bl-triangle}
\begin{align*}
  d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n},\Sigma_{t+1}^{1/2}(r_{0:t})Z + h\right)
  \le \max_{a}\left(\frac{s_{t+1,a}^{2} + h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)^{1/2} d_{\text{BL}}\left(Q_{n}^{t+1}(r_{0:t}),Z\right)
\end{align*}
since for any 1-Lipschitz function $f$, the Lipschitz constant of $f(\Sigma_{n,t+1}^{1/2}(r_{0:t})\cdot)$ is $\lambda_{\max}(\Sigma_{n,t+1}^{1/2}(r_{0:t}))$.

Next, we show convergence of $Q_{n}^{t+1}(r_{0:t})$ to a standard normal
random vector $Z \sim N(0,I)$ via a classical result. which is a corollary
of~\citet[Theorem 1]{Bhattacharya70}.  The following result explicitly
quantifies how the rate of convergence depends on the propensity scores,
allowing us to guarantee uniform convergence.
\begin{lemma}[{\citet[Theorem 1]{Bhattacharya70}}]. 
  \label{lemma:clt-rate}
  Let $\{X_i\}_{i =1}^n$ be a sequence of $n$ independent random vectors
  taking values in $\R^{\numarm}$ with covariance matrix $\Sigma_n$. Assume
  that for some $\delta > 0$
  \begin{equation*}
    M \defeq \sup_{n} \frac{1}{n} \sum_{i=1}^{n}
    \E \ltwo{\Sigma_{n}^{-1/2} X_{i}}^{3+\delta} < \infty.
  \end{equation*}
  Then, the normalized partial sum
  $\bar{Z}_{n} = \frac{1}{\sqrt{n}} \sum_{i=1}^{n} \Sigma_{n}^{-1/2} X_{i}$
  satisfies
  \begin{equation*}
    d_{\text{BL}}(\bar{Z}_n, N(0, I))
    \leq A_{K,\delta} M^{\frac{3+3\delta}{3+\delta}}n^{-1/2} + B_{K,\delta} M^{\frac{3}{3+\delta}}n^{-1/2}
  \end{equation*}
  where $A_{K,\delta}, B_{K,\delta}$ are constants that only depends on $K$ and
  $\delta$. 
\end{lemma}
\noindent In order to guarantee uniform convergence over $r_{0:t}$ using
Lemma~\ref{lemma:clt-rate}, we use
Assumptions~\ref{assumption:reward}\ref{item:moment}
and~\ref{assumption:policy}\ref{item:overlap} to control the moment term $M$.
Using $C_{\numarm, \delta}$ to denote a constant that only depends on
$\numarm$ and $\delta$ (that may differ line by line), use lower bound on the
minimum eigenvalue of $\Sigma_{n,t+1}$ given in Lemma~\ref{lemma:min-max-eig}
to get
\begin{align*}
  M(r_{0:t})
  & \defeq \sup_{n} \frac{1}{n}\sum_{j=1}^{n} \mathbb{E}
    \ltwo{\Sigma_{n,t+1}^{-1/2}(r_{0:t})
    \left( \frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(r_{0:t})} - \frac{h}{\sqrt{n}}\right)}^{3+\delta} \\
  &\le \left( \max_a\frac{\pi_{t+1, a}(r_{0:t})}{s_{t+1,a}^{2}} \right)^{\frac{3+\delta}{2}}
  \sup_{n} \frac{1}{n}\sum_{j=1}^{n} \mathbb{E}
    \ltwo{\frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(r_{0:t})} - \frac{h}{\sqrt{n}}}^{3+\delta} \\
  & \le C_{\numarm, \delta}
   \max_a s_{t+1,a}^{-(3+\delta)}
    \max_a ~\E
    \left|\frac{\xi_{j, a}^{t+1}R_{j,a}}{\pi_{t+1, a}(r_{0:t})} - \frac{h_a}{\sqrt{n}}\right|^{3+\delta}
\end{align*}
Using Assumptions~\ref{assumption:reward}\ref{item:moment}
and~\ref{assumption:policy}\ref{item:overlap}, conclude
\begin{align}
  \label{eqn:m-bound}
  M(r_{0:t})
  \le C_{\numarm, \delta} \max_a s_{t+1,a}^{-(3+\delta)}
    \cdot \left(\frac{1}{\min_{a} \pi_{t+1, a}(r_{0:t})}  \right)^{3+\delta}
    \left( C + \left(\frac{\max_a |h_a|}{\sqrt{n}}\right)^{3+\delta}\right),
\end{align}
where $C$ is the moment bound on $\epsilon_a$ given in
Assumption~\ref{assumption:reward}\ref{item:moment}.

Apply Lemma~\ref{lemma:clt-rate} to get
\begin{equation*}
  d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n},\Sigma_{t+1}^{1/2}(r_{0:t})Z\right)	
  \leq \max_{a}\left(\frac{s_{t+1,a}^{2} + h_{a}^{2}}
    {\pi_{t+1,a}(r_{0:t})}\right)^{1/2}
  \cdot \left( A_{K,\delta} M(r_{0:t})^{\frac{3+3\delta}{3+\delta}} 
  + B_{K,\delta} M(r_{0:t})^{\frac{3}{3+\delta}} \right)n^{-1/2} 
\end{equation*}
Taking expectation over $r_{0:t}$ on both sides and using the preceding bound
on $M(r_{0:t})$~\eqref{eqn:m-bound}
\begin{align*}
  & \E\left[\E_{r_{0:t}}\left[d_{\text{BL}}\left(\sqrt{n}\bar{R}_{t+1}^{n},
    \Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h\right)
    \right]\right] \\
  & \leq \E \Biggl[ \max_{a}\left(\frac{s_{t+1,a}^{2} + h_{a}^{2}} 
    {\pi_{t+1,a}\left(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}\right)}\right)^{1/2} \\
   &\qquad \times \Biggl(  A_{K,\delta} M\left(\sqrt{n}\bar{R}_{0}^{n},...,
    \sqrt{n}\bar{R}_{t}^{n}\right)^{\frac{3+3\delta}{3+\delta}}
    + B_{K,\delta} M\left(\sqrt{n}\bar{R}_{0}^{n},...,
  \sqrt{n}\bar{R}_{t}^{n}\right)^{\frac{3}{3+\delta}} \Biggr)n^{-1/2} \Biggr] \\
  & \le n^{-1/2} \cdot C_{\numarm, \delta, s, b_{t+1}}
    \E\left[\left(\frac{1}{\min_a \pi_{t+1, a}\left(\sqrt{n}\bar{R}_{0}^{n},...,
    \sqrt{n}\bar{R}_{t}^{n}\right) }\right)^{\frac{7}{2}+3\delta} \right]
    \left( C^{\frac{3+3\delta}{3+\delta}}
    + \frac{\max_a \{ |h_a|^{4+3\delta} + |h_a|^{3+3\delta} \}}{n^{\frac{3+3\delta}{2}}} \right) \\
  & \qquad + n^{-1/2} \cdot B_{\numarm, \delta, s, b_{t+1}}
  \E\left[\left(\frac{1}{\min_a \pi_{t+1, a}\left(\sqrt{n}\bar{R}_{0}^{n},...,
  \sqrt{n}\bar{R}_{t}^{n}\right) }\right)^{\frac{7}{2}} \right]
  \left( C^{\frac{3}{3+\delta}}
  + \frac{3}{(3+\delta)C^{\frac{\delta}{3+\delta}}} \frac{\max_a \{ |h_a|^{4 + \delta} + |h_a|^{3 + \delta} \}}{n^{\frac{3+\delta}{2}}} \right),
\end{align*}
where $C_{\numarm, \delta, s, b_{t+1}}, B_{\numarm, \delta, s, b_{t+1}}$ are constants that only depends on
$\numarm$, $\delta$, measurement noise $s^2$, and batch scale $b_t$.

Finally, we show uniform convergence of the second term in the
bound~\eqref{eqn:bl-triangle}, that the limiting Gaussian
$N(h, \Sigma_{n,t+1}^{1/2}(r_{0:t}))$ converges uniformly to
$N(h, \Sigma_{t+1}^{1/2}(r_{0:t}))$ as $n\to \infty$
\begin{equation*}
  \E\left[\E_{r_{0:t}}\left[d_{\text{BL}}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h,
        \Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right) \right]\right] \to 0
\end{equation*}
First, for any two measures $(\mu,\nu)$, $d_{\text{BL}}(\mu,\nu)$ is upper
bounded by the total variation distnace $2d_{\text{TV}(\mu,\nu)}$, which is in
turn bounded above by KL divergence $\sqrt{\frac{1}{2}d_{\text{KL}}(\mu,\nu)}$
by Pinsker's inequality. We derive the following concrete bound on the KL
divergence, whose proof we defer to Section~\ref{section:proof-kl-cov}.
\begin{lemma}
  \label{lemma:kl-cov}
  \begin{equation*}
    \dkl{N\left(h, \Sigma_{n,t+1}(r_{0:t})\right)}
      {N\left(h, \Sigma_{t+1}(r_{0:t})\right)}
    \leq \frac{1}{n} \left[\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right]
  \end{equation*}
\end{lemma}
\noindent Therefore,
\begin{align*}
  &\E \left[ \E_{r_{0:t}}\left[ d_{\text{BL}}\left(\Sigma_{n,t+1}^{1/2}(r_{0:t})Z+h,
    \Sigma_{t+1}^{1/2}(r_{0:t})Z+h\right) \right] \right] \\
  &\leq n^{-1/2} \sqrt{2}\left(\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right)^{1/2}
\end{align*}

Altogether, we have shown that
\[
  |\E[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})] - \E[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]| = O(n^{-1/2})
\]
which implies weak convergence $(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t+1}^{n}) \cd (G_{0},...,G_{t+1})$.

\subsubsection{Proof of Lemma \ref{lemma:kl-cov}}
\label{section:proof-kl-cov}

We use the expression for the KL-divergence between two multivariate normal
distributions
\begin{align*}
  &\dkl{N(h,\Sigma_{n,t+1}(r_{0:t}))}{N(h,\Sigma_{t+1}(r_{0:t}))} \\
  &=\text{tr}\left(\Sigma_{t+1}(r_{0:t})^{-1}\Sigma_{n,t+1}(r_{0:t})\right)
    -k+\log\frac{\det\Sigma_{t+1}(r_{0:t})}{\det\Sigma_{n,t+1}(r_{0:t})} \\
  & =\sum_{a}\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)^{-1}
    \left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}
    +\left(\frac{1}{\pi_{t+1,a}(r_{0:t})}-1\right)
    \frac{h_{a}^{2}}{n}\right)-k+\log\det\Sigma_{t+1}(r_{0:t})-\log\det\Sigma_{n,t+1}(r_{0:t}) \\
  & \leq\sum_{a}\frac{\left(1-\pi_{t+1,a}(r_{0:t})\right)}{s_{t+1, a}^{2}}
    \frac{h_{a}^{2}}{n}+\sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right) \\
  & \qquad-\sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}
    +\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)
    + \left(\frac{1}{n}\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}
    {1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})} \right) \\
  &\leq\frac{1}{n}\left[\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}
    {1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}
    +\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right]
\end{align*}


We obtain $\det{\Sigma_{n,t+1}(r_{0:t})}$ using the fact that $\Sigma_{n,t+1}(r_{0:t})$ is a rank-one perturbation of a diagonal matrix
\begin{equation*}
  \Sigma_{n,t+1} =\Sigma_{t+1}
  +\frac{1}{n}\text{diag}\left(\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)-\frac{1}{n}hh^{\top}
\end{equation*}
It follows that
\begin{align*}
  \log\det\Sigma_{n,t+1}(r_{0:t})	&=\log\det\left(\Sigma_{t+1}(r_{0:t})+\frac{1}{n}\text{diag}\left(h_{a}^{2}/\pi_{t+1,a}(r_{0:t})\right)\right) \\
                                        &\qquad +\log\det\left(I+\left(\Sigma_{t+1}(r_{0:t})+\frac{1}{n}\text{diag}\left(h_{a}^{2}/\pi_{t+1,a}(r_{0:t})\right)\right)^{-1}\left(-\frac{1}{n}hh^{\top}\right)\right) \\
                                        &=\sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right) \\
                                        &\qquad+\log\det\left(I-\frac{1}{n}h^{\top}\left(\Sigma_{t+1}(r_{0:t})+\frac{1}{n}\text{diag}\left(h^{2}/\pi_{t+1}(r_{0:t})\right)\right)^{-1}h\right) \\
                                        &=\sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)+\log\left(1-\frac{1}{n}\sum_{a}\pi_{t+1,a}(r_{0:t})\frac{h_{a}^{2}}{s_{t+1,a}^{2}+(1/n)h_{a}^{2}}\right) \\
                                        &\geq \sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right) + \log\left(1- \frac{1}{n}\max_{a} \frac{h_{a}^{2}}{s_{t+1,a}^{2}+(1/n)h_{a}^{2}}\right)
\end{align*}
Finally, we use the bound $\log(1-x)\geq \frac{-x}{1-x}$ to obtain
\begin{align*}
  \log\det\Sigma_{n,t+1}(r_{0:t})
  & \geq \sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}
    +\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)
    -  \frac{1}{n}\frac{\max_{a} \frac{h_{a}^{2}}{s_{t+1,a}^{2}+(1/n)h_{a}^{2}}}
    {1 - \max_{a} \frac{h_{a}^{2}}{ns_{t+1,a}^{2}+h_{a}^{2}}} \\
  &\geq \sum_{a}\log\left(\frac{s_{t+1,a}^{2}}{\pi_{t+1,a}(r_{0:t})}
    +\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(r_{0:t})}\right)
    - \frac{1}{n}\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}
    {1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}.
\end{align*}

\subsection{Proof of Corollary~\ref{cor:bsr-limit}}
\label{section:proof-bsr-limit}

From the proof of Theorem~\ref{theorem:limit}, the convergence of the Bayes
simple regret immediately follows from the fact that the weak
convergence~\eqref{eqn:weak-convergence} is uniform in $h$ under the
hypothesized moment condition on $h$.  The discontinuity points of $\pi_T$ are
of measure zero with respect to $(G_0,\dots,G_{T-1})$, the
convergence~\eqref{eqn:weak-convergence} and the Portmanteau theorem implies
that for any fixed $h$, as $n \to \infty$
\begin{equation*}
  \E[\pi_{T}(\sqrt{n}\bar{R}_{0}^{n},\ldots,\sqrt{n}\bar{R}_{T-1}^{n})|h] \to
  \E[\pi_{T}(G_{0},\ldots,G_{T-1})|h]
\end{equation*}
For any prior distribution $\nu$ over $h$ such that $\E_{\nu}||h|| < \infty$,
dominated convergence gives 
\begin{align*}
  \bsr_{T}(\pi, \nu, \sqrt{n}\bar{R}^{n})
  &= \E_{h\sim\nu}[h^{\top}\pi_{T}(\sqrt{n}\bar{R}_{0}^{n},\ldots,\sqrt{n}\bar{R}_{t+1}^{n})] 
  = \E_{h\sim\nu}[h^{\top}\E[\pi_{T}(\sqrt{n}\bar{R}_{0}^{n},\ldots,\sqrt{n}\bar{R}_{t+1}^{n})|h]] \\
  &\to \E_{h\sim\mu}[h^{\top}\E[\pi_{T}(G_{0},\ldots,G_{T-1})|h]] 
  = \bsr_{T}(\pi, \nu, V).
\end{align*}


\subsection{Proof of Theorem \ref{theorem:bayes-limit}}
\label{section:proof-limit-bayes}

We can show that for Bayesian policies, which update posterior beliefs as if the measurements were Gaussian, convergence of Bayes simple regret
occurs even without overlap. This explains why the Gaussian sequential approximation serves as a useful approximation for Bayesian policies
even when the propensity scores can be very small.

Suppose the experimenter selects the sampling allocation based on a Gaussian posterior state. That is, the sampling policy 
at period $t$ is of the form $\pi_{t}(\mu_{n,t}, \sigma_{n,t})$, where the posterior state $\Pstate_{n,t}\defeq(\mu_{n,t}, \sigma_{n,t})$ is defined recursively As

\begin{equation}
  \label{eqn:pre-limit-bayes-cond}
\begin{split}
  \sigma_{n,t+1,a}^{-2}|\mu_{n,t}, \sigma_{n,t} &= \sigma_{t,a}^{-2} + s_{t,a}^{-2}b_{t}\pi_{t,a}(\mu_{n,t}, \sigma_{n,t}) \\
  \mu_{n,t+1,a}|\mu_{n,t}, \sigma_{n,t} &= \sigma_{t+1,a}^{2}(\sigma_{t,a}^{-2}\mu_{t,a} + s_{t,a}^{-2}b_{t}\pi_{t,a}(\mu_{n,t}, \sigma_{n,t})\cdot\sqrt{n}\bar{R}_{t,a}^{n})
\end{split}
\end{equation}
starting from a deterministic prior $x_{0} = (\mu_{0}, \sigma_{0})$.

These are the posterior beliefs as if the estimates $\sqrt{n}\bar{R}_{t}^{n}$ were truly Gaussian,
and we expect that as $n \to \infty$, these beliefs converge to $\Pstate_{t} = (\mu_{t}, \sigma_{t})$, the trajectory of posterior beliefs
in the Gaussian Sequential Experiment:

\begin{equation}
  \label{eqn:limit-bayes-cond}
  \begin{split}
    \sigma_{t+1}^{-2} | \mu_{t}, \sigma_{t} &= \sigma_{t}^{-2} + s^{-2}b_{t}\pi_{t}(\mu_{t}, \sigma_{t}) \\
    \mu_{t+1} | \mu_{t}, \sigma_{t} &= \sigma_{t+1}^{2} \left( \sigma_{t}^{-2}\mu_{t} + s^{-2}b_{t}\pi_{t}(\mu_{t}, \sigma_{t})h + s^{-2}b_{t}\widetilde{\Sigma}_{t}^{-1/2}Z \right)
  \end{split}
\end{equation}
where $Z \sim N(0,I)$, addition and multiplication are element-wise, and 
\[
  \widetilde{\Sigma}_{t} \defeq \text{diag}(\pi_{t,a}s_{t,a}^{2})
\]

We say that a policy $\pi$ is a Gaussian Bayesian policy if the policy depends on the importance sampling estimators through Gaussian posterior beliefs.
That is, if there exists functions $\tilde{\pi}$ such that for all $t,a$
\[
  \pi_{t,a}(\sqrt{n} \bar{R}_{0}^{n}, \ldots, \sqrt{n} \bar{R}_{t-1}^{n}) = \tilde{\pi}_{t,a} (\mu_{n,t}, \sigma_{n,t})
\]

Note that for fixed local parameters $h$ and policy $\pi$, the pre-limit states $\Pstate_{n,t}\defeq(\mu_{n,t}, \sigma_{n,t})$
and the states in the Gaussian sequential experiment $\Pstate_{t}\defeq(\mu_{t}, \sigma_{t})$
evolve as Markov chains.

To formalize this, we consider alternative assumptions for the policy:

\begin{assumption}
  \label{assumption:bayes-policy}
  \begin{enumerate}
  \item \label{item:bayes-sufficiency}
    \emph{Bayesian Sufficiency}: the policy $\pi$ depends on
    the data only through the posterior states, i.e.,
    $\pi_{t}=\pi_{t}(\mu_{n,t}, \sigma_{n,t})$ for all $t$.
  \item \label{item:bayes-continuity} \emph{Continuity}: for all $t$, the
    discontinuity points of $\tilde{\pi}_{t}$ are of measure zero with respect to
    $X_{t} = (\mu_{t}, \sigma_{t})$.
  \end{enumerate}
\end{assumption}

Critically, we no longer need the overlap assumption. The reason is that Gaussian Bayesian policies do not directly reliably
on the importance sampling estimators, which will blow up as the propensity scores tend to zero, but rather the modified estimators:

\[
  \sqrt{n}\widetilde{R}_{t,a}^{n} \defeq \pi_{t,a}\sqrt{n}\bar{R}_{t,a}^{n} = \frac{1}{b_{t}\sqrt{n}} \sum_{j=1}^{b_{t}n}\xi_{a,j}^{t} R^{t}_{a,j}
\]

\begin{theorem}
  \label{theorem:bayes-limit}
  Let Assumptions~\ref{assumption:reward},\ref{assumption:bayes-policy} hold. Then the pre-limit posterior states 
  converge to the posterior states under the Gaussian Sequential Experiment as $n\to\infty$:
  \[
    (\mu_{n,0}, \sigma_{n,0},\ldots,\mu_{n,T-1}, \sigma_{n,T-1}) \cd (\mu_{0}, \sigma_{0},\ldots,\mu_{T-1}, \sigma_{T-1})
  \]
\end{theorem}

The proof proceeds similarly as with the proof of Theorem \ref{theorem:limit}.

Let $s_{t, a}^{2} \defeq s_a^{2}/b_{t}$ be the rescaled measurement variance. Recall the pre-limit posterior state trajectory $\Pstate_{n,t} = (\mu_{n,t}, \sigma_{n,t})$:

\begin{equation*}
\begin{split}
  \sigma_{n,t+1}^{-2}|\mu_{n,t}, \sigma_{n,t} &= \sigma_{t}^{-2} + s_{t}^{-2}\pi_{t}(\mu_{n,t}, \sigma_{n,t}) \\
  \mu_{n,t+1}|\mu_{n,t}, \sigma_{n,t} &= \sigma_{t+1,a}^{2}(\sigma_{t}^{-2}\mu_{t} + s_{t}^{-2}\cdot\sqrt{n}\widetilde{R}_{t}^{n})
\end{split}
\end{equation*}
and the posterior state trajectory under the Gaussian sequential experiment $\Pstate_{t} = (\mu_{t}, \sigma_{t})$:

\begin{equation*}
  \begin{split}
    \sigma_{t+1}^{-2} | \mu_{t}, \sigma_{t} &= \sigma_{t}^{-2} + s_{t}^{-2}\pi_{t}(\mu_{t}, \sigma_{t}) \\
    \mu_{t+1} | \mu_{t}, \sigma_{t} &= \sigma_{t+1}^{2} \left( \sigma_{t}^{-2}\mu_{t} + s^{-2}b_{t}\pi_{t}(\mu_{t}, \sigma_{t})h + s^{-2}b_{t}\widetilde{\Sigma}_{t}^{-1/2}Z \right)
  \end{split}
\end{equation*}
where $\widetilde{\Sigma}_{t} = \text{diag}(\pi_{t,a} s_{t,a}^{2})$.

We prove weak convergence by an induction argument. To fix the base cases, we can first observe that
 $(\mu_{n,0}, \sigma_{n,0}) = (\mu_{0}, \sigma_{0})$ since this is the prior posterior state.
Next, $\sigma_{n,1}^{-2} = \sigma_{0}^{-2} + s_{0}^{-2}\pi_{0}(\mu_{0}, \sigma_{0}) = \sigma_{1}^{-2}$ since 
$\pi_{0}(\mu_{0}, \sigma_{0})$ is deterministic.

Before we show weak convergence for the mean, it is worth mentioning that since we do not assume any overlap condition
(allowing propensity scores to even be zero), showing that the central limit theorem holds is trickier.
Our strategy is to split the arms between those whose propensity scores are larger than some threshold $\epsilon >0$
and those whose propensity scores aren't and use the central limit theorem for the former.

Let $I(0, \mu_0, \sigma_0) \defeq \{ a \in [K]: \pi_{0,a}(\mu_{0}, \sigma_{0}) > 0 \}$. Since $\pi_{0}$ and $(\mu_0, \sigma_0)$
are deterministic, this is a deterministic set. For the arms not in $I(0, \mu_0, \sigma_0)$, $\mu_{n, 1,a} = \mu_{0,a}$, which
coincides with $\mu_{1,a}$ in the Gaussian sequential limit. For the remaining arms, by the Lindeberg CLT,
we have that $\sqrt{n}\widetilde{R}_{1}^{n} \cd N(\pi_{0}h, \widetilde{\Sigma}_{0})$. By the continuous mapping theorem,
this implies weak convergence of $\mu_{n,1} \cd \mu_{1}$.
% \[
% \begin{aligned}  
% \mu_{n,1} &= \sigma_{1}^{2}\left( \sigma_{0}^{-2} \mu_{0} + s_{0}^{-2}\cdot \sqrt{n}\widetilde{R}_{t}^{n} \right)
%           \cd \sigma_{1}^{2}(\sigma_{0}^{-2} \mu_{0} + s_{0}^{-2} \pi_{0}h) +  \sigma_{1}^{2}s_{0}^{-2}\widetilde{\Sigma}_{0}^{-1/2}Z
% \end{aligned}
% \]

We proceed with the induction argument. Suppose that as $n\to \infty$
\[
  (\mu_{n,0}, \sigma_{n,0},\ldots,\mu_{n,t}, \sigma_{n,t}) \cd (\mu_{0}, \sigma_{0},\ldots,\mu_{t}, \sigma_{t})
\]

Note that joint weak convergence with $\sigma_{n,t+1}$ immediately follows
since by Assumption \ref{assumption:bayes-policy}\ref{item:bayes-continuity}
$\sigma_{n,t+1}$ is a deterministic, continuous function of $(\mu_{n,t}, \sigma_{n,t})$.

To show joint weak convergence it is sufficient to show 
\begin{equation}
  \label{eqn:bayes-inductive-weak-convergence}
  \E[f(\mu_{n,0}, \sigma_{n,0},\ldots,\mu_{n,t+1}, \sigma_{n,t+1})] \to
  \E[f(\mu_{0}, \sigma_{0},\ldots,\mu_{t+1}, \sigma_{t+1})]~~\mbox{for any
bounded Lipschitz function}~f
\end{equation}
Fixing a bounded Lipschitz $f$, assume without loss of generality that
\begin{equation*}
  \sup_{x,y\in\mathbb{R}^{(t+1)\times k}}|f(x)-f(y)|\leq 1
  ~~~\mbox{and}~~~f\in\text{Lip}(\mathbb{R}^{(t+1)\times K}).
\end{equation*}

We proceed with the same decomposition as in Theorem \ref{theorem:limit}.
We first set up some basic notation. We define the conditional expectation operator on a random variable $W$
\begin{equation*}
  \begin{split}
  \E_{\pstate_{t}}[W] &\defeq \E\left[ W \Bigg| \Pstate_{n,t} = \pstate_{t}\right]. \\
  \E_{\pstate_{0:t}}[W] &\defeq \E\left[ W \Bigg| \Pstate_{0,t} = \pstate_{0},\ldots,\Pstate_{n,t} = \pstate_{t}\right].
  \end{split}
\end{equation*}
Then, conditional on realizations of previous importance sampling estimators
up to time $t$, let $g_{n},g:\R^{t\times K} \to \R$ be the conditional
expectation of $f$ and its limiting counterpart
\begin{align*}
  g_{n}(\pstate_{0:t}) &\defeq
             \E_{\pstate_{0:t}}\left[f\left( \Pstate_{n,0}, \ldots, \Pstate_{n,t}, \Pstate_{n,t+1} \right) \right]
             = \E\left[f\left(\pstate_{0:t}, \mu_{n,t+1}(\pstate_{t}), \sigma_{t+1}^{2}(\pstate_{t})\right)\right] \\
  g(s_{0:t}) & \defeq \E_{s_{0:t}}\left[f\left(\Pstate_{n,0}, \ldots, \Pstate_{n,t}, \Pstate_{t+1}\right)\right]
         =\E\left[f\left(\pstate_{0:t}, \mu_{t+1}(\pstate_{t}), \sigma_{t+1}^{2}(\pstate_{t}) \right)\right]
\end{align*}

Sufficiency of conditioning by $\Pstate_{n,t}$ follows from
the Markovian assumption for the propensity scores (Assumption \ref{assumption:bayes-policy}\ref{item:bayes-sufficiency}). 
The functions $\mu_{n,t+1}(\cdot), \mu_{t+1}(\cdot), \sigma^{2}(\cdot)$ are defined for a fixed state
$\pstate_{t} = (\bar{\mu}_{t}, \bar{\sigma}_{t})$ to be
\[
  \begin{aligned}
    \sigma_{t+1}^{-2}(\pstate_{t}) &= \bar{\sigma}_{t}^{-2} + s_{t}^{-2}\pi_{t}(\pstate_{t}) \\
    \mu_{t+1}(\pstate_{t}) &= \sigma_{t+1}^{2}(\pstate_{t})(\bar{\sigma}_{t}^{-2}\bar{\mu}_{t} + s_{t}^{-2}\pi_{t}(\pstate_{t})h) +  \sigma_{t+1}^{2}s_{t}^{-2}\widetilde{\Sigma}^{1/2}_{t+1}(\pstate_{t})Z \\
    \mu_{n,t+1}(\pstate_{t}) &= \sigma_{t+1}^{2}(\pstate_{t})(\bar{\sigma}_{t}^{-2}\bar{\mu}_{t} + s_{t}^{-2} \sqrt{n}\tilde{R}_{t}^{n})
  \end{aligned}
\]
and $Z\sim N(0,I)$ and $\widetilde{\Sigma_{t}}(\pstate_{t})$ depends on the state $\pstate_{t}$ through the propensity scores
$\pi_{t,a}(\pstate_{t})$.
\[
  \widetilde{\Sigma_{t}}(\pstate_{t}) = \text{diag}(\pi_{t,a}(\pstate_{t}) s_{t,a}^{2}).
\]
Conditional on the state $\pstate_{t}$, $\sqrt{n}\tilde{R}_{t}^{n}$ depends on $x_{t}$ only through the propensity scores
$\pi_{t,a}(\pstate_{t})$. Moreover, note that conditional on $\pstate_{t}$, $\sigma_{n,t+1} = \sigma_{t+1}(\pstate_{t})$, so the only difference between $g_n$ and $g$
is between $\mu_{n,t+1}$ and $\mu_{t+1}$.

% The conditional distribution of $S_{n,t+1}|S_{n,t} = s_t$ is specified in (\ref{eqn:pre-limit-bayes-cond});
% the conditional distribution of $S_{t+1}|S_{n,t} = s_t$ is specified in (\ref{eqn:limit-bayes-cond}).

As in Theorem \ref{theorem:limit}, to show the weak convergence we decompose the
difference between
$\E[f(\Pstate_{n,0},\ldots,\Pstate_{n,t+1})]$ and
$\E[f(\Pstate_{0},\ldots,\Pstate_{t+1})]$ in terms of $g_{n}$ and $g$
\begin{align}
  &|\mathbb{E}[f(\Pstate_{n,0},\ldots,\Pstate_{n,t+1})]
     - \mathbb{E}[f(\Pstate_{0},...,\Pstate_{t+1})]| \label{eqn:bayes-start} \\ 
  & =|\mathbb{E}[g_{n}(\Pstate_{n,0},\ldots,\Pstate_{n,t})]
    -\mathbb{E}[g(\Pstate_{0},...,\Pstate_{t})]|  \nonumber  \\
  & =|\mathbb{E}[g_{n}(\Pstate_{n,0},\ldots,\Pstate_{n,t})]
    -\mathbb{E}[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})]|
    +|\E[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})]-\mathbb{E}[g(\Pstate_{0},\ldots,\Pstate_{t})]| \nonumber
\end{align}
By Assumption~\ref{assumption:bayes-policy}\ref{item:bayes-continuity} and dominated
convergence, $g$ is continuous almost surely under $(\Pstate_{0}, \ldots, \Pstate_{t})$.
From the inductive hypothesis~\eqref{eqn:inductive-hypothesis}, the continuous mapping theorem implies
\begin{equation*}
  \E[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})] \to \mathbb{E}[g(\Pstate_{0},\ldots, \Pstate_{t})].
\end{equation*}

It remains to show the convergence
$\E[g_{n}(\Pstate_{n,0},\ldots,\Pstate_{n,t})] \to
\E[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})]$. As in Theorem \ref{theorem:limit}, we require
Lemma \ref{lemma:clt-rate} to provide a quantitative rate of convergence.
However, without an overlap condition, we have to carefully apply the CLT
for the arms with large enough propensity scores, and show for the remaining arms
that the update to the posterior state will be small. Moreover,
we need to do this across random realizations of the propensity scores.
To do so, we develop uniform rates of convergence for posterior means
of arms in both sets.

We first define some new notation. For $\epsilon >0$, let the set $I_{\epsilon}(\pstate_{t})$ be defined as the set of arms
whose propensity scores (given state $\pstate_{t}$) are bigger than $\epsilon$.
\[
I_{\epsilon}(\pstate_{t}) \defeq \{ a \in [\numarm]: \pi_{t,a}(\pstate_{t}) > \epsilon \}
\]
Let $\mu_{n,t+1}^{I_{\epsilon}}(\pstate_{t})$ denote the vector of posterior means
for arms in $I_{\epsilon}(\pstate_{t})$, and let $\mu_{n,t+1}^{I^{c}_{\epsilon}}$ be the posterior measurement
of arms not in $I_{\epsilon}(\pstate_{t})$. We also use the notation $||\cdot||_{2,I^{c}_{\epsilon}}$ to denote
the $2$-norm only among arms in $I^{c}_{\epsilon}$.

We have the following bound for the difference in $g_n$ and $g$, in terms of bounded Lipschitz distance
between posterior means $\mu_{n,t+1}$ and $\mu_{t+1}$
\[
  \begin{aligned}
    &|\E[g_{n}(\Pstate_{n,0},\ldots,\Pstate_{n,t})]-\mathbb{E}[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})]| \\
    &=|\E[\E\left[f(\pstate_{0:t},\Pstate_{n,t+1})-f(\pstate_{0:t}, \Pstate_{t+1})|\Pstate_{n,0},\ldots \Pstate_{n,t}=\pstate_{0:t}\right]]| \\
    &=|\E[\E\left[f(\pstate_{0:t},\mu_{n,t+1}(\pstate_{t}),\sigma_{t+1}(\pstate_{t}))-f(\pstate_{0:t},\mu_{t+1}(\pstate_{t}),\sigma_{t+1}(\pstate_{t}))
    |\Pstate_{n,0},\ldots \Pstate_{n,t}=\pstate_{0:t}\right]]| \\
    &\leq \E[\E\left[d_{\text{BL}}(\mu_{n,t+1}(\pstate_{t}),\mu_{t+1}(\pstate_{t}))|\Pstate_{n,t}=\pstate_{t}\right]] \\
  \end{aligned}
\]

Note that the only difference between $\mu_{n,t+1}(x_{t})$ and $\mu_{t+1}(x_{t})$ is that
$\mu_{n,t+1}(x_{t})$ is updated using the aggregated rewards $\sqrt{n}\widetilde{R}^{n}_{t}$
while $\mu_{t+1}(x_{t})$ is updated by by a Gaussian $\widetilde{\Sigma}^{1/2}Z$. For arms with a large enough 
propensity score, $\sqrt{n}\widetilde{R}^{n}_{t} \cd \widetilde{\Sigma}^{1/2}Z$ by the CLT. For arms with very
small propensity scores, both $\sqrt{n}\widetilde{R}^{n}_{t}$ and $\widetilde{\Sigma}^{1/2}Z$
will be close to zero.

To show this concretely, we can bound the bounded Lipschitz difference by separating out the difference in posterior means among arms
with propensity scores larger than $\epsilon$, and those with propensity scores less than $\epsilon$:

\begin{equation}
  \label{eqn:bl-props-ge-eps}
  \begin{aligned}
    &\E[\E_{\pstate_{t}} \left[d_{\text{BL}}(\mu_{n,t+1}(\pstate_{t}),\mu_{t+1}(\pstate_{t}))\right]] \\
    &\leq \E[\E_{\pstate_{t}} \left[d_{\text{BL}}(\mu_{n,t+1}^{I_{\epsilon}}(\pstate_{t}),\mu_{n,t+1}^{I_{\epsilon}}(\pstate_{t}))\right]]
    +\E [ \E_{\pstate_{t}} [ \ltwo{ \mu_{n,t+1}^{I_{\epsilon}^{c}}(\pstate_{t}) - \mu_{n,t+1}^{I_{\epsilon}^{c}}(\pstate_{t})) }] ]
    \end{aligned}
\end{equation}

Since for any bounded 1-Lipschitz function $f$ and random vectors $A,A'\in \R^{n},B,B'\in \R^{m}$:
\[
  \begin{aligned}
  |\E f(A,B) - \E f(A',B')| &= |\E f(A,B) - \E f(A',B)| + |\E f(A',B) - \E f(A',B')| \\
                            &\leq d_{\text{BL}}(A,A') + \ltwo{(A',B) - (A',B')} \\
                            & = d_{\text{BL}}(A,A') + \ltwo{B - B'}
  \end{aligned}
\]

To bound the second part of the inequality (\ref{eqn:bl-props-ge-eps}),
we will show that for the arms whose propensity scores are less than $\epsilon$, 
the posterior means in the pre-limit vs 
in the Gaussian sequential experiment will be close, as both will be close to the prior. 
Consider any $\pstate_{t} = (\bar{\mu}_{t}, \bar{\sigma}_{t})$:

\[
  \begin{aligned}
  & \E \left[ \E_{\pstate_{t}} \left[ || \mu_{n,t+1}^{I_{\epsilon}^{c}}(\pstate_{t}) - \mu_{n,t+1}^{I_{\epsilon}^{c}}(\pstate_{t}) ||_{2} \right] \right] \\
  &= \E \left[ \E_{\pstate_{t}} \left[ || \mu_{n,t+1}(\pstate_{t}) - \mu_{n,t+1}(\pstate_{t}) ||_{2, I_{\epsilon}^{c}}  \right] \right] \\
  &= \E \left[ \E_{\pstate_{t}} \left[ ||  \sigma_{t+1}^{2}(\pstate_{t}) s_{t}^{-2} \sqrt{n}\widetilde{R}_{t}^{n} -  \sigma_{t+1}^{2}(\pstate_{t}) s_{t}^{-2}\pi_{t}(\pstate_{t})h -  \sigma_{t+1}^{2}s_{t}^{-2} \widetilde{\Sigma}^{1/2}_{t}(\pstate_{t})Z  ||_{2, I_{\epsilon}^{c}}  \right] \right] \\
  &\leq \E \left[ \E_{\pstate_{t}} \left[ || \sqrt{n}\widetilde{R}_{t}^{n} - \pi_{t}(\pstate_{t})h ||_{2, I_{\epsilon}^{c}} 
       +  || \widetilde{\Sigma}^{1/2}_{t}(\pstate_{t})Z  ||_{2, I_{\epsilon}^{c}}  \right] \right] \\
  &\leq \epsilon^{1/2} \left( \sum_{a} \frac{s_{t,a}^{2} + h_{a}^{2}}{b_{t}} \right)^{1/2} + \epsilon^{1/2} (\max_{a} s_{t,a}) \numarm
\end{aligned}
\]

The second-to-last line uses triangle inequality and the fact that $\sigma_{t+1}^{2}(x_{t}) \leq s_{t}^{2}$ for all $x_{t}$. The last line uses the fact that:

\[
\begin{split}
  &\E \left[ \E_{\pstate_{t}} \left[  || \sqrt{n}\widetilde{R}_{t}^{n} - \pi_{t}(\pstate_{t})h||_{2, I_{\epsilon}^{c}}   \right] \right] \\
  &  \leq \sqrt{n} \E \left[ \E_{\pstate_{t}} \left[ \sum_{a\in I_{\epsilon}^{c}(\pstate_{t})} \left( \frac{1}{b_{t}n} \sum_{j=1}^{b_{t}n} \xi_{a,j}^{t} R_{a,j}^{t} - \pi_{t,a}(\pstate_{t})\frac{h}{\sqrt{n}} \right)^{2}
    \right] \right]^{1/2} \\
  & = \sqrt{n} \E \left[ \E_{\pstate_{t}} \left[  \sum_{a\in I_{\epsilon}^{c}(\pstate_{t})} \text{Var} \left( \frac{1}{b_{t}n} \sum_{j=1}^{b_{t}n} \xi_{a,j}^{t} R_{a,j}^{t} \right)
    \right] \right]^{1/2}\\
  & \leq \sqrt{n} \E \left[ \E_{\pstate_{t}} \left[  \sum_{a\in I_{\epsilon}^{c}(\pstate_{t})} \frac{\pi_{t,a}(\pstate_{t}) (s_{t,a}^{2} + h_{a}^{2})}{b_{t}n} \right] \right]^{1/2} \\
  &\leq \epsilon^{1/2} \left( \sum_{a} \frac{s_{t,a}^{2} + h_{a}^{2}}{b_{t}} \right)^{1/2}
\end{split}
\]
where the first inequality uses Jensen's inequality, and the second inequality uses the fact that $\text{Var}(\xi_{a,j}^{t}R_{a,j}^{t}) = \pi_{t,a}(\pstate_{t}) s_{t,a}^{2} + \pi_{t,a}(\pstate_{t})(1-\pi_{t,a}(\pstate_{t}))h_{a}^{2}$.

It remains then to bound the first part of the inequality (\ref{eqn:bl-props-ge-eps}), which
is the distance between the posterior means for the arms with propensity scores greater than $\epsilon$.
To do so, we use bounds on the rate of convergence for the CLT for the posterior means of arms
with propensity scores larger than $\epsilon$, which hold regardless of the realization of $\pstate_{t}$.

We restrict ourselves to arms $a \in I_{\epsilon}(x_{t})$ and use subscript $\epsilon$ to denote quantities restricted
to those arms. If $I_{\epsilon}(x_{t})$ is empty, then the distance is automatically zero. Moreover,
for $\epsilon < 1/\numarm$ there will always be at least 1 arm in $I_{\epsilon}(x_{t})$, so without loss we assume that
$|I_{\epsilon}(x_{t})| = m > 0$ for some $m$.

We define some new notation. Let $\widetilde{Q}_{n,\epsilon}^{t}(\pstate_{t})$ be the normalized estimator, 
restricted to arms in $I_{\epsilon}(x_{t})$.

\begin{equation*}
  \widetilde{Q}_{n,\epsilon}^{t}(\pstate_{t}) \defeq
  \widetilde{\Sigma}_{n,\epsilon,t}^{-1/2}(\pstate_{t})(\sqrt{n}\widetilde{R}_{\epsilon, t}^{n} - \pi_{t}(\pstate_{t})h)
  = \frac{1}{\sqrt{n}}\sum_{j=1}^{n} \Sigma_{n,\epsilon,t}^{-1/2}(\pstate_{t})
  \left(
    \xi_{a,j}^{t}R_{a,j}^{t} -\frac{\pi_{t,a}(\pstate_{t})h_{a}}{\sqrt{n}}
  \right)_{a\in I_{\epsilon}(\pstate_{t})}.
\end{equation*}
where the conditional covariance $\widetilde{\Sigma}_{n,\epsilon,t}(\pstate_{t})$ is:

\[
  \widetilde{\Sigma}_{n,\epsilon,t}(\pstate_{t}) \defeq \text{Cov}(\xi_{a,j}^{t}R_{a,j}^{t}) = \widetilde{\Sigma}_{\epsilon,t}(\pstate_{t}) + \frac{1}{n}\text{diag}(\pi_{t,a}(\pstate_{t})h_{a}^{2}) - \frac{1}{n}(\pi_{t}(\pstate_{t})h)(\pi_{t}(\pstate_{t})h)^{\top}
\]
with entries restricted to $a\in I_{\epsilon}(\pstate_{t})$.

It is helpful to specify the minimum and eigenvalues of $\widetilde{\Sigma}_{n,\epsilon,t}(\pstate_{t})$, as was done in Lemma \ref{lemma:min-max-eig}.
%{\citet[Section 5]{Golub73}}

\begin{lemma} \label{lemma:bayes-min-max-eig} Suppose that $|I_{\epsilon}(\pstate_{t})|> 0$. Let $\lambda_{\max}(\cdot)$ and $\lambda_{\min}(\cdot)$ denote
  the maximum and minimum eigenvalues respectively. For any realization of $\pstate_{t}$, we have that:
  \[
    \begin{aligned}
    \lambda_{\max} (\widetilde{\Sigma}_{n,\epsilon,t}(\pstate_{t})) &\leq \lambda_{\max}
    \left( \widetilde{\Sigma}_{\epsilon,t}(\pstate_{t})+\frac{1}{n} \text{diag} \left( \pi_{t,a}(\pstate_{t})h_{a}^{2}  \right) \right)
    \leq \max_{a}\left( s_{t,a}^{2} + h_{a}^{2} \right) \\
    \lambda_{\min} (\widetilde{\Sigma}_{n,\epsilon,t}(\pstate_{t})) & \geq \lambda_{\min}(\Sigma_{\epsilon, t}(\pstate_{t})) + \frac{1}{n} \lambda_{\min} \left( \text{diag}(\pi_{t,a}(\pstate_{t})h_{a}^{2}) - (\pi_{t}(\pstate_{t})h)(\pi_{t}(\pstate_{t})h)^{\top} \right)
    \geq \epsilon \left( \min_{a}s_{t,a}^{2}  \right) \\
    \end{aligned}
  \]
\end{lemma}

\begin{proof-of-lemma}
  The first inequality follows since
  $\lambda_{\max}(A + B) \le \lambda_{\max}(A) + \lambda_{\max}(B)$ for
  symmetric matrices $A,B \in \R^{K\times K}$. The second inequality uses
  $\lambda_{\min}(A + B) \geq \lambda_{\min}(A) + \lambda_{\min}(B)$.
  Moreover, for any $b\in \R^{m}$
  \[
  b^{\top}\left( \text{diag}(\pi_{t,a}(\pstate_{t})h_{a}^{2}) - (\pi_{t}(\pstate_{t})h)(\pi_{t}(\pstate_{t})h)^{\top} \right)b
  = \sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})h_{a}^{2}b_{a}^{2} - \left( \sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})h_{a}b_{a} \right)^{2} \geq 0
  \]
  as by Cauchy-Schwartz:
  \[
   \left( \sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})h_{a}b_{a} \right)^{2} \leq \left(\sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t}) \right)
   \left(\sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})h_{a}^{2}b_{a}^{2} \right) \leq \left(\sum_{a\in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})h_{a}^{2}b_{a}^{2} \right)
  \]
  
so the matrix is positive semi-definite
\end{proof-of-lemma}

As in the proof of Theorem \ref{theorem:limit}, we can observe that

\begin{align}
  & \E[\E_{\pstate_{t}}\left[d_{\text{BL}}(\mu_{n,t+1}^{I_{\epsilon}}(\pstate_{t}),\mu_{n,t+1}^{I_{\epsilon}}(\pstate_{t})) \right]] \nonumber \\
  & = \E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\sqrt{n}\widetilde{R}_{\epsilon, t}^{n} - \pi_{t}(\pstate_{t})h, \widetilde{\Sigma}^{1/2}_{\epsilon, t}(\pstate_{t})Z ) \right]] \nonumber \\
  & \leq \E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\sqrt{n}\widetilde{R}_{\epsilon, t}^{n} - \pi_{t}(\pstate_{t})h, \widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z ) \right]] 
    + \E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z, \widetilde{\Sigma}^{1/2}_{\epsilon, t}(\pstate_{t})Z ) \right]]
    \label{eqn:bayes-bl-triangle}
\end{align}

The first part of the preceding inequality \eqref{eqn:bayes-bl-triangle} will vanish as $n\to \infty$ due to the CLT.
The second part contains discrepancies that result from sampling according to random multinomial vectors,
and will also converge to zero as $n\to\infty$.

We begin with bounding the first term in \eqref{eqn:bayes-bl-triangle}. Since for any $1$-Lipschitz function $f$,
the Lipschitz constant of $v \mapsto f(\Sigma_{n,\epsilon,t}^{1/2}(x_{t})v)$ is 
$\lambda_{\max} \left(\Sigma_{n,\epsilon,t}^{1/2}(\pstate_{t}) \right)$,

\[
  \begin{split}
  & \E[\E_{\pstate_{t}} \left[ d_{\text{BL}, \epsilon} (\Pstate_{t+1} - \pi_{t}(\pstate_{0:t})h, \widetilde{\Sigma}^{1/2}_{n,t+1}(\pstate_{0:t})Z ) \right]] \\
  & \leq \max_{a} (s_{t+1,a}^{2} + h_{a}^{2})^{1/2} \cdot \E[\E_{\pstate_{0:t}} \left[ d_{\text{BL}} (\widetilde{Q}_{n,\epsilon}^{t+1}(\pstate_{0:t}), \widetilde{\Sigma}^{1/2}_{n,t+1}(\pstate_{0:t})Z ) \right]]
  \end{split}
\]
using the upper bound for the max eigenvalue in Lemma \ref{lemma:bayes-min-max-eig}.

Conditional on $x_{t}$, $\widetilde{Q}_{n,\epsilon}^{t}(\pstate_{t})$ is a normalized sum of independent random vectors.
We proceed to make use of the quantitative rate of convergence for the CLT provided by Lemma \ref{lemma:clt-rate}.
Using $C_{\numarm, \delta}$ to denote a constant that only depends on
$\numarm$ and $\delta$ (that may differ line by line), use lower bound on the
minimum eigenvalue of $\Sigma_{n,\epsilon, t}$ given in Lemma~\ref{lemma:bayes-min-max-eig}
to get

\begin{equation*}
  \begin{split}
  \widetilde{M}(\pstate_{t})
  & \defeq \sup_{n} \frac{1}{n}\sum_{j=1}^{n} \mathbb{E}
    \ltwo{\widetilde{\Sigma}_{n,\epsilon,t}^{-1/2}(x_{t})
    \left(
      \xi_{a,j}^{t}R_{a,j}^{t} -\frac{\pi_{t,a}(\pstate_{t})h_{a}}{\sqrt{n}}
    \right)_{a\in I_{\epsilon}(\pstate_{t})}}^{3+\delta} \\
  & \leq \left( \epsilon \min_{a} s_{t,a}^{2} \right)^{-\frac{3+\delta}{2}} \sup_{n} \frac{1}{n}\sum_{j=1}^{n} \mathbb{E}
  \ltwo{ \xi_{j}^{t}R_{j}^{t} -\frac{\pi_{t}(\pstate_{t})h}{\sqrt{n}}}^{3+\delta} \\
      &\leq C_{k,\delta} \left( \epsilon \min_{a} s_{t,a}^{2} \right)^{-\frac{3+\delta}{2}}
      \max_{a} \E \left|\xi_{j}^{t+1}R_{j,a} - \frac{h}{\sqrt{n}}\right|^{3+\delta} < \infty\\
  \end{split}
\end{equation*}

Using Assumption~\ref{assumption:reward}\ref{item:moment}, conclude

\[
  \widetilde{M}(\pstate_{t})\leq C_{k,\delta} \left( \epsilon \min_{a} s_{t,a}^{2} \right)^{-\frac{3+\delta}{2}} 
  \left( C + \left(\frac{\max_{a} |h_{a}|}{\sqrt{n}} \right)^{3+\delta} \right) < \infty 
\]
where $C$ is the moment bound in $\epsilon_{a}$ given in Assumption~\ref{assumption:reward}\ref{item:moment}.

Apply Lemma~\ref{lemma:clt-rate} to get

\[
  \begin{split}
  &\E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\sqrt{n}\widetilde{R}_{\epsilon, t}^{n} - \pi_{t}(\pstate_{t})h, \widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z )\right]] \\
  & \leq \max_{a} (s_{t,a}^{2} + h_{a}^{2})^{1/2} \cdot \E[\E_{\pstate_{t}} \left[ A_{m,\delta} \widetilde{M}(\pstate_{t})^{\frac{3+3\delta}{3+\delta}} n^{-1/2}
  + B_{m,\delta} \widetilde{M}(\pstate_{t})^{\frac{3}{3+\delta}} n^{-1/2} \right]]
  \end{split}
\]


Taking expectation over $x_{t}$ and using the preceding bound on $M(\pstate_{t})$, we have that
\[
  \begin{split}
  & \E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\sqrt{n}\widetilde{R}_{\epsilon, t}^{n} - \pi_{t}(\pstate_{t})h, \widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z )|\Pstate_{n,t}=\pstate_{t}\right]] \\
  & \leq \max_{a} (s_{t,a}^{2} + h_{a}^{2})^{1/2} \cdot 
  \E[\E_{\pstate_{t}} \left[ A_{m,\delta} \widetilde{M}(\pstate_{t})^{\frac{3+3\delta}{3+\delta}} n^{-1/2}
  + B_{m,\delta} \widetilde{M}(\pstate_{t})^{\frac{3}{3+\delta}} n^{-1/2}
   |\Pstate_{n,t}=\pstate_{t}\right]] \\
  & \leq n^{-1/2} \cdot C_{k,\delta,s,b_{t}} \epsilon^{-\frac{3+3\delta}{2}} 
  \left( C^{\frac{3+3\delta}{3+\delta}} + \frac{\max_{a} \{|h_{a}|^{4+3\delta} + |h_{a}|^{3+3\delta} \}}{n^{\frac{3+3\delta}{2}}} \right) \\
  &+n^{-1/2} \cdot B_{k,\delta,s,b_{t}} \epsilon^{-\frac{3}{2}}
  \left( C^{\frac{3}{3+\delta}} + \frac{3}{(3+\delta)C^{\frac{\delta}{3+\delta}}}\frac{\max_{a} \{|h_{a}|^{4 + \delta} + |h_{a}|^{3 + \delta} \}}{n^{\frac{3+\delta}{2}}} \right)
  \end{split}
\]
where $C_{k,\delta,s,b_{t}}, B_{k,\delta,s,b_{t}}$ are constants that only depend on $K,\delta$, measurement noise $s^{2}$,
and batch scale $b_{t}$. Note that this bound holds regardless of the realization of $\pstate_t$.

Finally, we find an upper bound for the second term in the inequality \eqref{eqn:bayes-bl-triangle}, which characterizes 
the distance between $\widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z$ 
and $\widetilde{\Sigma}^{1/2}_{\epsilon, t}(\pstate_{t})Z$. We show that this goes to zero
through a bound on the KL-divergence. We defer the proof to section \ref{section:proof-bayes-kl-cov}.

\begin{lemma}\label{lemma:bayes-kl-cov} The KL-divergence between $N(0, \Sigma_{n,\epsilon, t}(\pstate_{t}))$ and
  $N(0, \Sigma_{\epsilon, t}(\pstate_{t}))$
  is bounded above as follows:
\[
 \dkl{N(0, \Sigma_{n,\epsilon, t}(\pstate_{t})}{N(0, \Sigma_{\epsilon, t}(\pstate_{t}))}
  \leq \frac{1}{n} \left[\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right]
\]
\end{lemma}

This guarantees that:
\[
  \begin{split}
  &\E[\E_{\pstate_{t}} \left[ d_{\text{BL}} (\widetilde{\Sigma}^{1/2}_{n,\epsilon, t}(\pstate_{t})Z, \widetilde{\Sigma}^{1/2}_{\epsilon, t}(\pstate_{t})Z ) \right]] \\
  &\leq n^{-1/2} \sqrt{2}\left(\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})}+\sum_{a}\left(\frac{h_{a}^{2}}{s_{t+1,a}^{2}}\right)\right)^{1/2}
  \end{split}
\]

Altogether, we have shown that
\[
  |\E[g_{n}(\Pstate_{n,0},\ldots,\Pstate_{n,t})]-\mathbb{E}[g(\Pstate_{n,0},\ldots,\Pstate_{n,t})]|
  \leq A\epsilon^{1/2} + B\epsilon^{-\frac{3+3\delta}{2}}n^{-1/2} + C\epsilon^{-\frac{3}{2}}n^{-1/2} + Dn^{-1/2}
\]
where $A,B,C,D$ are constants that do not depend on $\epsilon$ or $n$. Since the choice of threshold $\epsilon$ was arbitrary,
we can set $\epsilon = n^{-\frac{1}{4+3\delta}}$, we can get a rate of convergence of $n^{-\frac{1}{8 + 6\delta}}$.

Thus, this shows that $\E[f(X_{n,0},\ldots,X_{n,t+1})] \to \E[f(X_{0},\ldots,X_{t+1})]$ as $n\to \infty$ 
for any bounded Lipschitz function $f$, which implies the desired weak convergence.


\subsubsection{Proof of Lemma~\ref{lemma:bayes-kl-cov} \label{section:proof-bayes-kl-cov}}

We use the expression for the KL-divergence between two multivariate normal distributions:

\[
  \begin{aligned}
	& \dkl{N(0, \Sigma_{n,\epsilon, t}(\pstate_{t})}{N(0, \Sigma_{\epsilon, t}(\pstate_{t}))} \\
	&=\text{tr}\left(\Sigma_{\epsilon, t}(\pstate_{t})^{-1} \Sigma_{n,\epsilon, t}(\pstate_{t})\right)-k+\log\frac{\det\Sigma_{\epsilon, t}(\pstate_{t})}{\det\Sigma_{n,\epsilon, t}(\pstate_{t})} \\
  &=\sum_{a \in I_{\epsilon}(\pstate_{t})} \left( s_{t,a}^{2}\pi_{t,a}(\pstate_{t}) \right)^{-1} 
  \left(s_{t,a}^{2}\pi_{t,a}(\pstate_{t}) + \pi_{t,a}(\pstate_{t}) (1 - \pi_{t,a}(\pstate_{t})) \frac{h_{a}^{2}}{n} \right)-k \\
  &\qquad +\log\det\Sigma_{\epsilon, t}(x_{t})-\log\det\Sigma_{n,\epsilon, t+1}(\pstate_{t}) \\
	&\leq \sum_{a \in I_{\epsilon}(\pstate_{t})} \frac{1}{n} \frac{\left(1-\pi_{t+1,a}(\pstate_{t})\right)h_{a}^{2}}{s_{t, a}^{2}}
  +\sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left( s_{t,a}^{2}\pi_{t,a}(\pstate_{t}) \right) \\
  & \qquad-\sum_{a \in I_{\epsilon}(\pstate_{t})}\log\left(s_{t,a}^{2}\pi_{t,a}(\pstate_{t})+\frac{1}{n}h_{a}^{2}\pi_{t,a}(\pstate_{t})\right) 
  + \left(\frac{1}{n}\frac{\max_{a} h_{a}^{2}/s_{t+1,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t+1,a}^{2}+h_{a}^{2})} \right) \\
	&\leq\frac{1}{n}\left[\sum_{a}\left(\frac{h_{a}^{2}}{s_{t,a}^{2}}\right) + \frac{\max_{a} h_{a}^{2}/s_{t,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t,a}^{2}+h_{a}^{2})}\right]
\end{aligned}
\]

We obtain $\det{\Sigma_{n,t}(\pstate_{t})}$ using the fact that $\Sigma_{n,t}(\pstate_{t})$ is a rank-one perturbation of a diagonal matrix:

\[
  \begin{aligned}
  \log\det\Sigma_{n,\epsilon,t}(\pstate_{t})	&=\log\det\left(\Sigma_{\epsilon,t}(\pstate_{t})+\frac{1}{n}\text{diag}\left(\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)\right) \\
  &\qquad +\log\det\left(I+\left(\Sigma_{\epsilon,t}(\pstate_{t})+\frac{1}{n}\text{diag}\left(\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)\right)^{-1}
  \left(-\frac{1}{n}(\pi_{t}(\pstate_{t})h)(\pi_{t}(\pstate_{t})h)^{\top}\right)\right) \\
	&=\sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left(s_{t,a}^{2}\pi_{t,a}(\pstate_{t})+\frac{1}{n}h_{a}^{2}\pi_{t,a}(\pstate_{t})\right)  \\
  &\qquad+\log\det\left(I-\frac{1}{n}(\pi_{t}(\pstate_{t})h)^{\top}\left(\Sigma_{\epsilon, t}(\pstate_{t})+\frac{1}{n}\text{diag}\left(\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)\right)^{-1}(\pi_{t}(\pstate_{t})h)\right) \\
	&=\sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left(\pi_{t,a}(\pstate_{t})s_{t,a}^{2}+\frac{1}{n}\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)
  +\log\left(1-\frac{1}{n} \sum_{a \in I_{\epsilon}(\pstate_{t})} \pi_{t,a}(\pstate_{t})\frac{h_{a}^{2}}{s_{t,a}^{2}+(1/n)h_{a}^{2}}\right) \\
  &\geq \sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left(\pi_{t,a}(\pstate_{t})s_{t,a}^{2}+\frac{1}{n}\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)
   + \log\left(1- \frac{1}{n}\max_{a} \frac{h_{a}^{2}}{s_{t,a}^{2}+(1/n)h_{a}^{2}}\right)
  \end{aligned}
\]

Finally, we use the bound $\log(1-x)\geq \frac{-x}{1-x}$ to obtain

\[
  \begin{aligned}
    \log\det\Sigma_{n,\epsilon,t}(\pstate_{t})&\geq \sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left(\pi_{t,a}(\pstate_{t})s_{t,a}^{2}+\frac{1}{n}\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)
    -  \frac{1}{n}\frac{\max_{a} \frac{h_{a}^{2}}{s_{t,a}^{2}+(1/n)h_{a}^{2}}}{1 - \max_{a} \frac{h_{a}^{2}}{ns_{t,a}^{2}+h_{a}^{2}}} \\
  &\geq \sum_{a \in I_{\epsilon}(\pstate_{t})} \log\left(\pi_{t,a}(\pstate_{t})s_{t,a}^{2}+\frac{1}{n}\pi_{t,a}(\pstate_{t})h_{a}^{2}\right)
   -  \frac{1}{n}\frac{\max_{a} h_{a}^{2}/s_{t,a}^{2}}{1 - \max_{a} h_{a}^{2}/(s_{t,a}^{2}+h_{a}^{2})} \\
  \end{aligned}
\]




% We denote the importance sampling estimator at time $t+1$ conditional on previous estimates as 
% $\bar{R}^{n}_{t+1}(y) \equiv \bar{R}^{n}_{t+1} | \sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t} =y$ \hn{This notation is ill-defined; you can define a RV that has the same conditional law as the RHS}
%   and 
% and and so we can rewrite the expectation of $g$ as: 
% \[ \E[f(\sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t+1})]	= \E [g_{n}(\sqrt{n}\bar{R}^{n}_{0},\ldots,\sqrt{n} \bar{R}^{n}_{t})]\]
% \hn{Let's introduce and start using the notation $\E_y[\cdot] \defeq \E[\cdot \mid \sqrt{n} \{\bar{R}^n_s\}_{s=0}^t = y]$ here.}

% For any fixed $y$ such that $\frac{1}{\pi_{t+1,a}(y)}<\infty,\forall a$,
% \hn{The below display has many problems. $\E$ should be $\E_y$ and the second equality seems wrong? It's unclear why you're stating this in the first place.}
% \[ 
%   \begin{aligned}
%     \sup_{n}\mathbb{E}  \left|\left| \frac{\xi^{t+1}_{j}R_{j}^{t+1}}{\pi_{t+1}} \right|\right|^{2}
%     & =\sup_{n}\sum_{a}\mathbb{E} \left[ \left(\frac{\xi^{t+1}_{a,j}R_{a,j}^{t+1}}{\pi_{t+1,a}}\right)^{2} \right] \\
%     &=\sup_{n}\sum_{a}\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\left(\frac{1}{\pi_{t+1,a}(y)}-1\right)\frac{h_{a}^{2}}{n}+h_{a}^{2} \\
%     &\leq\sum_{a}\frac{s_{a}^{2}+h_{a}^{2}}{\pi_{t+1,a}(y)}+h_{a}^{2} < \infty 
%   \end{aligned}    
% \]


% Moreover, $\E\left[\sqrt{n}\bar{R}_{t+1}^{n}\right]=h$ and $\Sigma_{t+1}^{n}(y)\equiv\text{Cov}(R_{j}^{t+1}) = 
% \Sigma_{t+1}(y)+\frac{1}{n} \text{diag} \left( \frac{h_{a}^2}{\pi_{t-1,a}(y)} \right)- \frac{1}{n}hh^{\top} $ \hn{$\pi$ indices are off here. And $\frac{1}{n} hh^\top$ seems wrong as it assumes components of $\xi^{t+1}_{j}$ are independent. The off-diagonal terms should contain $\cov(\xi^{t+1}_{j, a}, \xi^{t+1}_{j, a'})$ related terms.} and $\Sigma_{t+1}^n(y) \to \Sigma_{t+1}(y)$ as $n\to \infty$. So by Lindeberg CLT~\hn{CITE},
% \[ \sqrt{n}\bar{R}_{t+1}^{n}(y) \cd N(h,\Sigma_{t+1}(y)) \]
% \hn{Perhaps it's clearer to write this by explicitly saying the convergence is conditional on the history}
% Thus, for any $y$ such that $\frac{1}{\pi_{t+1,a}(y)}<\infty,\forall a$, by Portmanteau theorem~\hn{CITE}, this implies pointwise convergence of $g_{n}(y) \to g(y) \equiv \E[f(y, \Sigma^{1/2}_{t+1}(y)Z + h)]$ as $n\to \infty$, where $Z \sim N(0, I)$.

% By the Portmanteau theorem and the induction hypothesis, $|\mathbb{E}[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t+1}^{n})]-\mathbb{E}[g(G_{1},...,G_{t})]| \to 0$ converges to zero as $n\to\infty$.

% Let $\sqrt{n}\widehat{R}_{t+1}^{n}\equiv\sqrt{n}\bar{R}_{t+1}^{n}-h$ be the demeaned estimator \hn{This notation is only used a couple times. Let's not introduce unnecessary notation.} and define 
% \[Q_{n}^{t+1}(y)\equiv\sqrt{n}\Sigma_{n,t+1}^{-1/2}(y)\widehat{R}_{t+1}^{n}=\frac{1}{\sqrt{n}}\sum_{j=1}^{n}\Sigma_{n,t+1}^{-1/2}(y)\left(\frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(y)}-h\right)\]
% The terms in the sum are iid across $j$ with mean zero and identity covariance and by the moment assumption we have $m_{3+\delta}(y)=\sup_{n}\frac{1}{n}\sum_{j=1}^{n}\mathbb{E}\left\Vert \Sigma_{n,t+1}^{-1/2}(y)\left(\frac{\xi_{j}^{t+1}R_{j}^{t+1}}{\pi_{t+1}(y)}-h\right)\right\Vert ^{3+\delta}<\infty$ 
% for some $\delta>0$. Let $d_\text{BL}$ denote the bounded Lipschitz distance defined as:
% \[d_{\text{BL}}(\mu,\nu)=\sup\left\{ |\mathbb{E}_{\mu}[f]-\mathbb{E}_{\nu}[f]|:f\in\text{Lip}(\mathbb{R}^{k}),\sup_{x,y\in\mathbb{R}^{k}}|f(x)-f(y)|\leq1\right\} \] 
% It is well-known that $d_\text{BL}$ metrizes weak convergence and $d_\text{BL}(\mu,\nu)\leq2d_{TV}(\mu,\nu)$. B
% For any 1-Lipschitz function $f$, the Lipschitz constant of $f(\Sigma_{n,t+1}^{1/2}(y)\cdot)$ is $\lambda_{1}(\Sigma_{n,t+1}^{1/2}(y)) 
% =\lambda_{1}(\Sigma_{n,t+1}(y))^{1/2}\leq\max_{a}\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\frac{2h_{a}^{2}}{\pi_{t+1,a}(y)}\right)^{1/2}$. \hn{Can you first define $\lambda_1$, and double check these eigenvalue calculations?}

% \[
%   \begin{aligned}
%     d_{\text{BL}}(\sqrt{n}\widehat{R}_{t+1}^{n},\Sigma_{t+1}^{1/2}(y)Z)	&\leq d_{\text{BL}}(\Sigma_{n,t+1}^{1/2}(y)Q_{n}^{t+1}(y),\Sigma_{n,t+1}^{1/2}(y)Z)+d_{\text{BL}}(\Sigma_{n,t+1}^{1/2}(y)Z,\Sigma_{t+1}^{1/2}(y)Z) \\
% 	 &=\left[\max_{a}\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\frac{2h_{a}^{2}}{\pi_{t+1,a}(y)}\right)^{1/2}\right]d_{\text{BL}}(Q_{n}^{t+1}(y),Z)+2d_{\text{TV}}(\Sigma_{n,t+1}^{1/2}(y)Z,\Sigma_{t+1}^{1/2}(y)Z)\\
%    &\leq n^{-1/2}\frac{\max_{a}(s_{a}^{2}+2h_{a}^{2})^{1/2}}{\min_{a}\pi_{t+1,a}(y)^{1/2}}A_{K,\delta}m_{3+\delta}^{\frac{3(1+\delta)}{3+\delta}}(y)+2n^{-1/2}\sqrt{\left[\left(\frac{\max_{a}h_{a}^{2}/s_{a}^{2}}{2(1-\max_{a}h_{a}^{2}/s_{a}^{2})}\right)+\sum_{a}\left(\frac{h_{a}^{2}}{2s_{a}^{2}}\right)\right]}
%   \end{aligned}
% \]

% The bound for the second term is obtained by Pinsker's inequality:

% \[
%   \begin{aligned}
% 	&d_{\text{TV}}(N(0,\Sigma_{n,t+1}(y)),N(0,\Sigma_{t+1}(y))) \\
% 	&\leq\sqrt{\frac{1}{2}KL(N(0,\Sigma_{n,t+1}(y)),N(0,\Sigma_{t+1}(y)))} \\
% 	&=\sqrt{\frac{1}{2}\left[\text{tr}\left(\Sigma_{t+1}(y)^{-1}\Sigma_{n,t+1}(y)\right)-k+\log\frac{\det\Sigma_{t+1}(y)}{\det\Sigma_{n,t+1}(y)}\right]} \\
% 	&=\sqrt{\frac{1}{2}\left[\sum_{a}\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}\right)^{-1}\left(\frac{s_{t}^{2}}{\pi_{t+1,a}(y)}+\left(\frac{1}{\pi_{t+1,a}(y)}-1\right)\frac{h_{a}^{2}}{n}\right)-k+\log\det\Sigma_{t+1}(y)-\log\det\Sigma_{n,t+1}(y)\right]} \\
% 	&=\sqrt{\frac{1}{2}\left[\sum_{a}\frac{\left(1-\pi_{t+1,a}(y)\right)}{s_{a}^{2}}\frac{h_{a}^{2}}{n}+\sum_{a}\log\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}\right)-\sum_{a}\log\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(y)}\right)-\left(\frac{\max_{a}\frac{h_{a}^{2}}{ns_{a}^{2}+h_{a}^{2}}}{(1-\max_{a}\frac{h_{a}^{2}}{ns_{a}^{2}+h_{a}^{2}})}\right)\right]} \\
% 	&\leq\sqrt{\frac{1}{2n}\left[\left(\frac{\max_{a}\frac{h_{a}^{2}}{ns_{a}^{2}+h_{a}^{2}}}{(1-\max_{a}\frac{h_{a}^{2}}{ns_{a}^{2}+h_{a}^{2}})}\right)+\sum_{a}\left(\frac{h_{a}^{2}}{s_{a}^{2}}\right)\right]}
% \end{aligned}
% \]

% as $\Sigma_{n,t+1}=\Sigma_{t+1}+\frac{1}{n}\text{diag}\left(\frac{h^{2}}{\pi_{t+1}(y)}\right)-\frac{1}{n}hh^{\top}$ and

% \[
%   \begin{aligned}
%   \log\det\Sigma_{n,t+1}(y)	&=\log\det\left(\Sigma_{t+1}(y)+\frac{1}{n}\text{diag}\left(h^{2}/\pi_{t+1}(y)\right)\right) \\
%   &+\log\det\left(I+\left(\Sigma_{t+1}(y)+\frac{1}{n}\text{diag}\left(h^{2}/\pi_{t+1}(y)\right)\right)^{-1}\left(-\frac{1}{n}hh^{\top}\right)\right) \\
% 	&=\sum_{a}\log\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(y)}\right)+\log\det\left(I-\frac{1}{n}h^{\top}\left(\Sigma_{t+1}(y)+\frac{1}{n}\text{diag}\left(h^{2}/\pi_{t+1}(y)\right)\right)^{-1}h\right) \\
% 	&=\sum_{a}\log\left(\frac{s_{a}^{2}}{\pi_{t+1,a}(y)}+\frac{1}{n}\frac{h_{a}^{2}}{\pi_{t+1,a}(y)}\right)+\log\left(1-\sum_{a}\pi_{t+1,a}(y)\frac{h_{a}^{2}}{ns_{a}^{2}+h_{a}^{2}}\right)
%   \end{aligned}
% \]

% Since $f$ is bounded and Lipschitz continuous, we have that 

% \[
%   \begin{aligned}
%     &|\mathbb{E}[g_{n}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]-\mathbb{E}[g(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})]| \\
%     &=\mathbb{E}[\mathbb{E}[\left[f(y,\sqrt{n}\bar{R}_{t+1}^{n})-f(y,\Sigma_{t+1}^{1/2}(y)Z+h)|\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n}=y\right]]] \\
%     &\leq n^{-1/2}\mathbb{E}\left[\frac{\max_{a}(s_{a}^{2}+2h_{a}^{2})^{1/2}}{\min_{a}\pi_{t+1,a}(y)^{1/2}}A_{K,\delta}m_{3+\delta}^{\frac{3(1+\delta)}{3+\delta}}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})\right] \\
%     &+n^{-1/2}\sqrt{\left[\left(\frac{1}{2(1-\max_{a}h_{a}^{2}/(h_{a}^{2}+s_{a}^{2}))}\right)+\sum_{a}\left(\frac{h_{a}^{2}}{2s_{a}^{2}}\right)\right]} \\
%     &\leq n^{-1/2}A_{K,\delta}B_{K,\delta}\mathbb{E}\left[\left(R_{a,j}^{t+1}\right)^{3+\delta}\right]^{\frac{3+3\delta}{3+\delta}}\mathbb{E}\left[\left(\min_{a}\pi_{t+1,a}(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t}^{n})\right)^{-3(1+\delta)-\frac{1}{2}}\right] \\
%     &+n^{-1/2}\sqrt{\left[\left(\frac{1}{2(1-\max_{a}h_{a}^{2}/(h_{a}^{2}+s_{a}^{2}))}\right)+\sum_{a}\left(\frac{h_{a}^{2}}{2s_{a}^{2}}\right)\right]} \\
%     &\leq n^{-1/2}CA_{K,\delta}B_{K,\delta}C_{t+1}\sum_{a}\mathbb{E}\left[\left(R_{a,j}^{t+1}\right)^{3+\delta}\right]^{\frac{3+3\delta}{3+\delta}}+n^{-1/2}\sqrt{\left[\left(\frac{1}{2(1-\max_{a}h_{a}^{2}/(h_{a}^{2}+s_{a}^{2}))}\right)+\sum_{a}\left(\frac{h_{a}^{2}}{2s_{a}^{2}}\right)\right]} \\
%   \end{aligned}
% \]

% where $B_{k,\delta}$ is a constant depending on $k$ and lower-order moments of $R_{a,j}^{t+1}$ and $\min_{a}\pi_{t+1,a}(\sqrt{n}\bar{R}_{0}^{n},\dots,\sqrt{n}\bar{R}_{t}^{n})$.

% Thus, we have shown that for any bounded Lipschitz function $f$, $\mathbb{E}[f(\sqrt{n}\bar{R}_{0}^{n},...,\sqrt{n}\bar{R}_{t+1}^{n})] \to \mathbb{E}[f(G_{1},...,G_{t+1})]$,
% where $G_{t+1}|G_{t},...,G_{1}\sim N(h,\Sigma_{t+1}(G_{t},...,G_{1}))$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

